Codescent and bicolimits of pseudo-algebras

We categorify cocompleteness results of monad theory, in the context of pseudomonads. We first prove a general result establishing that, in any 2-category, weighted bicolimits can be constructed from oplax bicolimits and bicoequalizers of codescent objects. After prerequisites on pseudomonads and their pseudo-algebras, we give a 2-dimensional Linton theorem reducing bicocompleteness of 2-categories of pseudo-algebras to existence of bicoequalizers of codescent objects. Finally we prove this condition to be fulfilled in the case of a bifinitary pseudomonad, ensuring bicocompleteness.

==> Complicated_proof_of_lemma_3.12.tex <==
Moreover, though the forgetfull functor $ U_T$ may not preserve bicoequalizers of codescent diagrams of pseudo-algebras, the arrow $ p : T \oplaxbicolim_I A_i \rightarrow C$ together with its $\xi$ still pseudocoequalizes $U_T \mathscr{X}_\mathbb{A}$. This latter condition gives in particular the lower and higher coherence 
% https://q.uiver.app/?q=WzAsNixbMSwxLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzEsMiwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsxLDMsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDMsIkMiXSxbMCwwLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMCwxLCJUcyJdLFsxLDIsIlxcbXVfQSJdLFswLDMsIlRhIiwyXSxbMyw0LCJwIl0sWzIsNCwicCIsMl0sWzUsMCwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgXFxldGFfe0FfaX0iLDFdLFs1LDMsIiIsMCx7ImN1cnZlIjotMiwibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSwyLCIiLDIseyJvZmZzZXQiOjEsImN1cnZlIjo1LCJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs1LDEsIiIsMSx7ImN1cnZlIjozfV0sWzYsNCwiXFx4aSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDEyLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBcXGFscGhhXnNfaSBcXGF0b3AgXFxzaW1lcSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMTQsIlRcXHNpZ21hIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE0LDEzLCJcXHpldGFfQSBcXGF0b3AgXFxzaW1lcSIsMCx7ImxhYmVsX3Bvc2l0aW9uIjo2MCwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{T\underset{I}\oplaxbicolim \; A_i} \\
	& {T\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; A_i} \\
	& {TT\underset{I}\oplaxbicolim \; A_i} \\
	& {T\underset{I}\oplaxbicolim \; A_i} && C
	\arrow[""{name=0, anchor=center, inner sep=0}, "Ts", from=2-2, to=3-2]
	\arrow["{\mu_A}", from=3-2, to=4-2]
	\arrow["Ta"', from=2-2, to=2-4]
	\arrow["p", from=2-4, to=4-4]
	\arrow["p"', from=4-2, to=4-4]
	\arrow["{T\underset{I}\oplaxbicolim \; \eta_{A_i}}"{description}, from=1-1, to=2-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, curve={height=-12pt}, Rightarrow, no head, from=1-1, to=2-4]
	\arrow[""{name=2, anchor=center, inner sep=0}, shift right=1, curve={height=30pt}, Rightarrow, no head, from=1-1, to=4-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, curve={height=18pt}, from=1-1, to=3-2]
	\arrow["{\xi \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=4-4]
	\arrow["{T\underset{I}\oplaxbicolim \; \alpha^s_i \atop \simeq}"{description, pos=0.4}, Rightarrow, draw=none, from=2-2, to=1]
	\arrow["{T\sigma \atop \simeq}"{description}, Rightarrow, draw=none, from=2-2, to=3]
	\arrow["{\zeta_A \atop \simeq}"{pos=0.6}, Rightarrow, draw=none, from=3, to=2]
\end{tikzcd} = 1_p \]


% https://q.uiver.app/?q=WzAsMTEsWzIsMSwiVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMiwzLCJUIFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsMSwiVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDMsIkMiXSxbMiwyLCJUVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDAsIlQgXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzAsMywiVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMCwwLCJUIFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVFRBX2kiXSxbMSwzLCJUIFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDIsIlRUIFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFsxLDIsIlRUVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDIsIlRhIiwyXSxbMiwxLCJcXHhpIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsMywicCIsMl0sWzIsMywicCIsMV0sWzQsMSwiXFxtdV9BIl0sWzAsNCwiVHMiXSxbNSwyLCJUYSJdLFs3LDUsIlQgXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUYV9pIl0sWzYsOF0sWzgsMSwiXFxtdV9BIiwyXSxbNyw5LCJUdCIsMl0sWzksMTAsIlRUcyJdLFsxMCw4LCJUIFxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pfSIsMV0sWzEwLDQsIlxcbXVfe1RBfSJdLFsxMCwxLCJcXHJob197XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzcsMCwiVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFxcbXVfe0FfaX0iLDFdLFs5LDYsIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaX0iLDJdLFsyNiwxMCwiVFxcdGF1IFxcYXRvcCBcXHNpbWVxIiwxLHsibGV2ZWwiOjEsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyNiwxNywiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgXFxhbHBoYV5zX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTksMjIsIlxcbXVfcyBcXGF0b3AgXFxzaW1lcSIsMSx7ImxldmVsIjoxLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}
	{T \underset{I}\oplaxbicolim \; TTA_i} &&& {T \underset{I}\oplaxbicolim \; TA_i} \\
	&& {T \underset{I}\oplaxbicolim \; TA_i} & {T \underset{I}\oplaxbicolim \; A_i} \\
	{TT \underset{I}\oplaxbicolim \; TA_i} & {TTT \underset{I}\oplaxbicolim \; A_i} & {TT \underset{I}\oplaxbicolim \; A_i} \\
	{T \underset{I}\oplaxbicolim \; TA_i} & {T T\underset{I}\oplaxbicolim \; A_i} & {T \underset{I}\oplaxbicolim \; A_i} & C
	\arrow["Ta"', from=2-3, to=2-4]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=2-4, to=4-3]
	\arrow["p"', from=4-3, to=4-4]
	\arrow["p"{description}, from=2-4, to=4-4]
	\arrow["{\mu_A}", from=3-3, to=4-3]
	\arrow["Ts", from=2-3, to=3-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "Ta", from=1-4, to=2-4]
	\arrow["{T \underset{I}\oplaxbicolim \; Ta_i}", from=1-1, to=1-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, from=4-1, to=4-2]
	\arrow["{\mu_A}"', from=4-2, to=4-3]
	\arrow["Tt"', from=1-1, to=3-1]
	\arrow[""{name=2, anchor=center, inner sep=0}, "TTs", from=3-1, to=3-2]
	\arrow["{T \mu_{\underset{I}\oplaxbicolim \; A_i}}"{description}, from=3-2, to=4-2]
	\arrow["{\mu_{TA}}", from=3-2, to=3-3]
	\arrow["{\rho_{\underset{I}\oplaxbicolim \; A_i} \atop \simeq}"{description}, draw=none, from=3-2, to=4-3]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{T \underset{I}\oplaxbicolim \; \mu_{A_i}}"{description}, from=1-1, to=2-3]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"', from=3-1, to=4-1]
	\arrow["{T\tau \atop \simeq}"{description}, draw=none, from=3, to=3-2]
	\arrow["{T\underset{I}\oplaxbicolim \; \alpha^s_i \atop \simeq}"{description}, Rightarrow, draw=none, from=3, to=0]
	\arrow["{\mu_s \atop \simeq}"{description}, draw=none, from=1, to=2]
\end{tikzcd}\]
% https://q.uiver.app/?q=WzAsMTAsWzAsNCwiVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDAsIlQgXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMyw0LCJDIl0sWzIsMCwiVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMCwyLCJUIFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFswLDAsIlQgXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUVEFfaSJdLFswLDMsIlQgVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzAsMSwiVFQgXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzIsMiwiVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsyLDEsIlQgVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzAsMiwicCIsMl0sWzEsMiwicCIsMV0sWzMsMSwiVGEiXSxbNSwzLCJUIFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVGFfaSJdLFs0LDYsIlRzIiwyXSxbNiwwLCJcXG11X0EiLDJdLFs1LDcsIlR0IiwyXSxbNyw0LCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2l9IiwyXSxbOCwyLCJwIiwxXSxbMyw5LCJUcyIsMl0sWzksOCwiXFxtdV9BIiwyXSxbNCw4LCJUYSIsMV0sWzcsOSwiVFRhIiwxXSxbOSwxMSwiXFx4aSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxOCw2LCJcXHhpIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEzLDIyLCJUXFx0aGV0YSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyMiwyMSwiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBhX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[=\begin{tikzcd}
	{T \underset{I}\oplaxbicolim \; TTA_i} && {T \underset{I}\oplaxbicolim \; TA_i} & {T \underset{I}\oplaxbicolim \; A_i} \\
	{TT \underset{I}\oplaxbicolim \; TA_i} && {T T\underset{I}\oplaxbicolim \; A_i} \\
	{T \underset{I}\oplaxbicolim \; TA_i} && {T \underset{I}\oplaxbicolim \; A_i} \\
	{T T\underset{I}\oplaxbicolim \; A_i} \\
	{T \underset{I}\oplaxbicolim \; A_i} &&& C
	\arrow["p"', from=5-1, to=5-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "p"{description}, from=1-4, to=5-4]
	\arrow["Ta", from=1-3, to=1-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{T \underset{I}\oplaxbicolim \; Ta_i}", from=1-1, to=1-3]
	\arrow["Ts"', from=3-1, to=4-1]
	\arrow["{\mu_A}"', from=4-1, to=5-1]
	\arrow["Tt"', from=1-1, to=2-1]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"', from=2-1, to=3-1]
	\arrow[""{name=2, anchor=center, inner sep=0}, "p"{description}, from=3-3, to=5-4]
	\arrow["Ts"', from=1-3, to=2-3]
	\arrow["{\mu_A}"', from=2-3, to=3-3]
	\arrow[""{name=3, anchor=center, inner sep=0}, "Ta"{description}, from=3-1, to=3-3]
	\arrow[""{name=4, anchor=center, inner sep=0}, "TTa"{description}, from=2-1, to=2-3]
	\arrow["{\xi \atop \simeq}"{description}, Rightarrow, draw=none, from=2-3, to=0]
	\arrow["{\xi \atop \simeq}"{description}, Rightarrow, draw=none, from=2, to=4-1]
	\arrow["{T\theta \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=4]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; a_i} \atop \simeq}"{description}, Rightarrow, draw=none, from=4, to=3]
\end{tikzcd}\]




\begin{division}[Free pseudomorphism at inclusions]
Then we can construct a canonical oplax cocone of pseudomorphisms of pseudo-algebras from $\mathbb{A}$ to $ (C,c, (\gamma^t, \gamma^s))$ as the following. First observe that at each $i \in I$ we can consider the free pseudomorphism over the inclusion $ q_i$
% https://q.uiver.app/?q=WzAsNCxbMCwxLCJUKEFfaSkiXSxbMSwxLCJUKFxcdW5kZXJzZXR7SX17XFxvcGxheGJpY29saW19IFxcOyBBX2kpIl0sWzEsMCwiVFQoXFx1bmRlcnNldHtJfXtcXG9wbGF4Ymljb2xpbX0gXFw7IEFfaSkiXSxbMCwwLCJUVChBX2kpIl0sWzAsMSwiVChxX2kpIiwyXSxbMiwxLCJcXG11X3tcXHVuZGVyc2V0e0l9e1xcb3BsYXhiaWNvbGltfSBcXDsgQV9pfSJdLFszLDAsIlxcbXVfe0FfaX0iLDJdLFszLDIsIlRUKHFfaSkiXSxbNyw0LCJcXG11X3txX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{TT(A_i)} & {TT(\underset{I}{\oplaxbicolim} \; A_i)} \\
	{T(A_i)} & {T(\underset{I}{\oplaxbicolim} \; A_i)}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{T(q_i)}"', from=2-1, to=2-2]
	\arrow["{\mu_{\underset{I}{\oplaxbicolim} \; A_i}}", from=1-2, to=2-2]
	\arrow["{\mu_{A_i}}"', from=1-1, to=2-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{TT(q_i)}", from=1-1, to=1-2]
	\arrow["{\mu_{q_i} \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=0]
\end{tikzcd}\]
which produces a pseudomorphism of pseudo-algebras
% https://q.uiver.app/?q=WzAsMixbMCwwLCIoVChBX2kpLFxcbXVfe0FfaX0sIChcXHhpX3tBX2l9LCBcXHJob197QV9pfSkgKSJdLFsyLDAsIihUKFxcdW5kZXJzZXR7SX17XFxvcGxheGJpY29saW19IFxcOyBBX2kpLCBcXG11X3tcXHVuZGVyc2V0e0l9e1xcb3BsYXhiaWNvbGltfSBcXDsgQV9pfSwgKFxceGlfe1xcdW5kZXJzZXR7SX17XFxvcGxheGJpY29saW19IFxcOyBBX2l9LCBcXHJob197XFx1bmRlcnNldHtJfXtcXG9wbGF4Ymljb2xpbX0gXFw7IEFfaX0pIl0sWzAsMSwiKFQocV9pKSwgXFxtdV97cV9pfSkiXV0=
\[\begin{tikzcd}
	{(T(A_i),\mu_{A_i}, (\xi_{A_i}, \rho_{A_i}) )} && {(T(\underset{I}{\oplaxbicolim} \; A_i), \mu_{A}, (\xi_{A}, \rho_{A}))}
	\arrow["{(T(q_i), \mu_{q_i})}", from=1-1, to=1-3]
\end{tikzcd}\]

\end{division}

In order to incude an oplax cocone from $\mathbb{A}$ to $(C,c, \gamma^t, \gamma^s))$, we must now establish that the composite above pseudocoequalizes the Barr construction at each individual pseudo-algebras $(A_i,a_i,(\alpha_i^s, \alpha_i^t)) $ and then use the bicoequalizing property of the pseudo-algebra. We must then establish the following technical lemma, whose proof, which is very long and tedious, can be omitted at a first reading:

\begin{lemma}\label{hard lemma}
For each $i \in I$, the composite pseudomorphism $(p,\pi)(T(q_i), \mu_{q_i})$ pseudocoequalizes the codescent object $ \mathscr{X}_{(A_i,a_i,(\alpha_i^s, \alpha_i^t))}$ of \cref{codescent object at an algebra}.
\end{lemma}

\begin{proof}
We first insert an underlying invertible 2-cell between the underlying maps as follows: 
% https://q.uiver.app/?q=WzAsOCxbMCwwLCJUVEFfaSJdLFsyLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMSwyLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzEsMywiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsMywiQyJdLFsyLDAsIlRBX2kiXSxbMCwyLCJUQV9pIl0sWzAsMSwiVHFeVF9pIiwxXSxbMSwyLCJUcyIsMV0sWzIsMywiXFxtdV9BIl0sWzEsNCwiVGEiLDJdLFs0LDUsInAiXSxbMyw1LCJwIiwyXSxbMCw2LCJUYV9pIl0sWzYsNCwiVHFfaSJdLFswLDcsIlxcbXVfe0FfaX0iLDJdLFs3LDMsIlRxX2kiLDJdLFswLDIsIlRUcV9pIiwxXSxbNiwxLCJUXFx0aGV0YV9pIFxcYXRvcFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOSw1LCJcXGNoaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxOCw3LCJcXG11X3txX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsMiwiVFxcc2lnbWFfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	{TTA_i} && {TA_i} \\
	&& {T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	{TA_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	& {T\underset{I}\oplaxbicolim \; A_i} && C
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Tq^T_i}"{description}, from=1-1, to=2-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Ts"{description}, from=2-3, to=3-2]
	\arrow["{\mu_A}", from=3-2, to=4-2]
	\arrow["Ta"', from=2-3, to=2-4]
	\arrow["p", from=2-4, to=4-4]
	\arrow["p"', from=4-2, to=4-4]
	\arrow["{Ta_i}", from=1-1, to=1-3]
	\arrow["{Tq_i}", from=1-3, to=2-4]
	\arrow["{\mu_{A_i}}"', from=1-1, to=3-1]
	\arrow["{Tq_i}"', from=3-1, to=4-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{TTq_i}"{description}, from=1-1, to=3-2]
	\arrow["{T\theta_i \atop\simeq}"{description}, draw=none, from=1-3, to=2-3]
	\arrow["{\xi \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=4-4]
	\arrow["{\mu_{q_i} \atop \simeq}"{description}, Rightarrow, draw=none, from=2, to=3-1]
	\arrow["{T\sigma_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=3-2]
\end{tikzcd}\]
It is routine, yet tedious to check this defines a transformation of pseudomorphisms, using successively pseudonaturality of the multiplication over the left triangle and the fact that $\xi$ is a transformation of pseudomorphisms. \\
% https://q.uiver.app/?q=WzAsMTIsWzAsMiwiVFRBX2kiXSxbMiwzLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzEsNCwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsxLDUsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDMsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbNCw1LCJDIl0sWzIsMiwiVEFfaSJdLFswLDQsIlRBX2kiXSxbMCwwLCJUVFRBX2kiXSxbMiwwLCJUVEFfaSJdLFszLDEsIlRUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsMywiVEMiXSxbMCwxLCJUcV5UX2kiLDFdLFsxLDIsIlRzIiwxXSxbMiwzLCJcXG11X0EiLDFdLFsxLDQsIlRhIiwxXSxbNCw1LCJwIiwxXSxbMyw1LCJwIiwyXSxbMCw2LCJUYV9pIiwxXSxbNiw0LCJUcV9pIiwxXSxbMCw3LCJcXG11X3tBX2l9IiwyXSxbNywzLCJUcV9pIiwyXSxbMCwyLCJUVHFfaSIsMV0sWzYsMSwiVFxcdGhldGFfaSBcXGF0b3BcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsMCwiXFxtdV97VEFfaX0iLDJdLFs4LDksIlRUYV9pIl0sWzksNiwiXFxtdV97QV9pfSIsMV0sWzksMTAsIlRUcV9pIl0sWzEwLDQsIlxcbXVfe1QgXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9IiwxXSxbMTAsMTEsIlRwIl0sWzExLDUsImMiXSxbMTMsNSwiXFxjaGkgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMjIsNywiXFxtdV97cV9pfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMiwyLCJUXFxzaWdtYV9pIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzI1LDE4LCJcXG11X3thX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzI3LDE5LCJcXG11X3txX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE2LDExLCJcXHBpIFxcYXRvcCBcXHNpbWVxIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d






% https://q.uiver.app/?q=WzAsMTEsWzIsMSwiVFRBX2kiXSxbNCwyLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzMsMywiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDQsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFs1LDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFs1LDQsIkMiXSxbNCwxLCJUQV9pIl0sWzIsMywiVEFfaSJdLFszLDAsIlRUQV9pIl0sWzAsMCwiVFRUQV9pIl0sWzAsMiwiVFRBX2kiXSxbMCwxLCJUcV5UX2kiLDFdLFsxLDIsIlRzIiwxXSxbMiwzLCJcXG11X0EiXSxbMSw0LCJUYSIsMl0sWzQsNSwicCJdLFszLDUsInAiLDJdLFswLDYsIlRhX2kiLDFdLFs2LDQsIlRxX2kiXSxbMCw3LCJcXG11X3tBX2l9IiwxXSxbNywzLCJUcV9pIiwyXSxbMCwyLCJUVHFfaSIsMV0sWzYsMSwiVFxcdGhldGFfaSBcXGF0b3BcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsNiwiVGFfaSJdLFs5LDAsIlRcXG11X3tBX2l9IiwxXSxbOSwxMCwiXFxtdV97VEFfaX0iLDJdLFsxMCw3LCJcXG11X3tBX2l9IiwyXSxbOSw4LCJUVGFfaSJdLFs4LDAsIlRcXGFscGhhX2ledCBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMCwwLCJcXG11X3tcXG11X3tBX2l9fSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMiw1LCJcXGNoaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyMSw3LCJcXG11X3txX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzExLDIsIlRcXHNpZ21hX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
% https://q.uiver.app/?q=WzAsMTEsWzEsMSwiVFRBX2kiXSxbMiwxLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzEsMiwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsxLDMsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDMsIkMiXSxbMywwLCJUQV9pIl0sWzAsMywiVEFfaSJdLFsxLDAsIlRUQV9pIl0sWzAsMCwiVFRUQV9pIl0sWzAsMSwiVFRBX2kiXSxbMCwxLCJUcV5UX2kiLDFdLFsxLDIsIlRzIiwxXSxbMiwzLCJcXG11X0EiXSxbMSw0LCJUYSIsMl0sWzQsNSwicCJdLFszLDUsInAiLDJdLFswLDYsIlRhX2kiLDFdLFs2LDQsIlRxX2kiXSxbMCw3LCJcXG11X3tBX2l9IiwxLHsibGFiZWxfcG9zaXRpb24iOjcwfV0sWzcsMywiVHFfaSIsMl0sWzAsMiwiVFRxX2kiLDFdLFs2LDEsIlRcXHRoZXRhX2kgXFxhdG9wXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDYsIlRhX2kiXSxbOSwwLCJUXFxtdV97QV9pfSIsMV0sWzksMTAsIlxcbXVfe1RBX2l9IiwyXSxbMTAsNywiXFxtdV97QV9pfSIsMl0sWzksOCwiVFRhX2kiXSxbOCwwLCJUXFxhbHBoYV9pXnQgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTAsMCwiXFxtdV97XFxtdV97QV9pfX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTIsNSwiXFxjaGkgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMjEsNywiXFxtdV97cV9pfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMSwyLCJUXFxzaWdtYV9pIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d



More challenging is to show that the composite invertible transformation of pseudomorphisms we inserted above satisfy the coherence conditions relative to the codescent data of $ \mathscr{X}_{(A_i, a_i, (\alpha^t_i, \alpha^s_i))}$. We first show that the underlying 2-cell $ \xi$ satisfy the coherences conditions relative to the underlying codescent diagram $ U_T \mathscr{X}_{(A_i, a_i, (\alpha^t_i, \alpha^s_i))}$.\\

For the lower condition, consider the following pasting, where the 2-cells $ T\alpha^T_i$ and $ \zeta_{A_i}$ for the invertible 2-cells in the codescent data in the Barr construction at $A_i$ - see \cref{codescent object at an algebra}. 
% https://q.uiver.app/?q=WzAsOSxbMSwxLCJUVEFfaSJdLFszLDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMiwzLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzIsNCwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsNCwiQyJdLFszLDEsIlRBX2kiXSxbMSwzLCJUQV9pIl0sWzAsMCwiVEFfaSJdLFswLDEsIlRxXlRfaSIsMV0sWzEsMiwiVHMiLDFdLFsyLDMsIlxcbXVfQSJdLFsxLDQsIlRhIiwyXSxbNCw1LCJwIl0sWzMsNSwicCIsMl0sWzYsNCwiVHFfaSJdLFswLDcsIlxcbXVfe0FfaX0iLDFdLFs3LDMsIlRxX2kiLDJdLFswLDIsIlRUcV9pIiwxXSxbNiwxLCJUXFx0aGV0YV9pIFxcYXRvcFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCwwLCJUXFxldGFfe0FfaX0iLDFdLFs4LDYsIiIsMCx7ImN1cnZlIjotMiwibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCw3LCIiLDEseyJjdXJ2ZSI6MiwibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCw2LCJUYV9pIiwxXSxbMTAsNSwiXFxjaGkgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTgsNywiXFxtdV97cV9pfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs5LDIsIlRcXHNpZ21hX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCwyMiwiXFx6ZXRhX3tBX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMjEsIlRcXGFscGhhXnRfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	{TA_i} \\
	& {TTA_i} && {TA_i} \\
	&&& {T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	& {TA_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	&& {T\underset{I}\oplaxbicolim \; A_i} && C
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Tq^T_i}"{description}, from=2-2, to=3-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Ts"{description}, from=3-4, to=4-3]
	\arrow["{\mu_A}", from=4-3, to=5-3]
	\arrow["Ta"', from=3-4, to=3-5]
	\arrow["p", from=3-5, to=5-5]
	\arrow["p"', from=5-3, to=5-5]
	\arrow["{Tq_i}", from=2-4, to=3-5]
	\arrow["{\mu_{A_i}}"{description}, from=2-2, to=4-2]
	\arrow["{Tq_i}"', from=4-2, to=5-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{TTq_i}"{description}, from=2-2, to=4-3]
	\arrow["{T\theta_i \atop\simeq}"{description}, draw=none, from=2-4, to=3-4]
	\arrow["{T\eta_{A_i}}"{description}, from=1-1, to=2-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, curve={height=-12pt}, Rightarrow, no head, from=1-1, to=2-4]
	\arrow[""{name=4, anchor=center, inner sep=0}, curve={height=12pt}, Rightarrow, no head, from=1-1, to=4-2]
	\arrow["{Ta_i}"{description}, from=2-2, to=2-4]
	\arrow["{\xi \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=5-5]
	\arrow["{\mu_{q_i} \atop \simeq}"{description}, Rightarrow, draw=none, from=2, to=4-2]
	\arrow["{T\sigma_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=4-3]
	\arrow["{\zeta_{A_i} \atop \simeq}"{description}, Rightarrow, draw=none, from=2-2, to=4]
	\arrow["{T\alpha^t_i \atop \simeq}"{description}, Rightarrow, draw=none, from=2-2, to=3]
\end{tikzcd}\]

Then in the lower left part of the diagram above we detect part of the pseudonaturality prism of $ \zeta$ at the oplax bicolimit inclusions: we can then do the following substitution - where, we recall, all occurence of $A$ stand for $ \oplaxbicolim_I A_i$:



% https://q.uiver.app/?q=WzAsOSxbMSwxLCJUVEFfaSJdLFszLDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMSwzLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzEsNCwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsNCwiQyJdLFszLDEsIlRBX2kiXSxbMCwwLCJUQV9pIl0sWzAsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzAsMSwiVHFeVF9pIiwxXSxbMSwyLCJUcyIsMV0sWzIsMywiXFxtdV9BIl0sWzEsNCwiVGEiLDJdLFs0LDUsInAiXSxbMyw1LCJwIiwyXSxbNiw0LCJUcV9pIl0sWzAsMiwiVFRxX2kiLDFdLFs2LDEsIlRcXHRoZXRhX2kgXFxhdG9wXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs3LDAsIlRcXGV0YV97QV9pfSIsMV0sWzcsNiwiIiwwLHsiY3VydmUiOi0yLCJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDYsIlRhX2kiLDFdLFs3LDgsIlRxX2kiLDJdLFs4LDIsIlRcXGV0YV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9IiwxXSxbMCw4LCJUXFxldGFfe3FfaX0gXFxhdG9wIFxcc2ltZXEiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCwzLCIiLDIseyJjdXJ2ZSI6MywibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTAsNSwiXFx4aVxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzksMiwiVFxcc2lnbWFfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDE5LCJUXFxhbHBoYV50X2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMjQsMjIsIlxcemV0YV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9IFxcYXRvcCBcXHNpbWVxIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{TA_i} \\
	& {TTA_i} && {TA_i} \\
	{T\underset{I}\oplaxbicolim \; A_i} &&& {T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	& {TT\underset{I}\oplaxbicolim \; A_i} \\
	& {T\underset{I}\oplaxbicolim \; A_i} &&& C
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Tq^T_i}"{description}, from=2-2, to=3-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Ts"{description}, from=3-4, to=4-2]
	\arrow["{\mu_A}", from=4-2, to=5-2]
	\arrow["Ta"', from=3-4, to=3-5]
	\arrow["p", from=3-5, to=5-5]
	\arrow["p"', from=5-2, to=5-5]
	\arrow["{Tq_i}", from=2-4, to=3-5]
	\arrow["{TTq_i}"{description}, from=2-2, to=4-2]
	\arrow["{T\theta_i \atop\simeq}"{description}, draw=none, from=2-4, to=3-4]
	\arrow["{T\eta_{A_i}}"{description}, from=1-1, to=2-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, curve={height=-12pt}, Rightarrow, no head, from=1-1, to=2-4]
	\arrow["{Ta_i}"{description}, from=2-2, to=2-4]
	\arrow["{Tq_i}"', from=1-1, to=3-1]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{T\eta_{A}}"{description}, from=3-1, to=4-2]
	\arrow["{T\eta_{q_i} \atop \simeq}"', draw=none, from=2-2, to=3-1]
	\arrow[""{name=4, anchor=center, inner sep=0}, curve={height=18pt}, Rightarrow, no head, from=3-1, to=5-2]
	\arrow["{\xi\atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=5-5]
	\arrow["{T\sigma_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=4-2]
	\arrow["{T\alpha^t_i \atop \simeq}"{description}, Rightarrow, draw=none, from=2-2, to=2]
	\arrow["{\zeta_{A} \atop \simeq}"', Rightarrow, draw=none, from=4, to=3]
\end{tikzcd}\]

But now the middle left prism recomposes as in the following diagram, where $ \sigma$ was defined in the second part of the proof of \cref{coherence data oplax bicolim : lower data}

% https://q.uiver.app/?q=WzAsOSxbMiwxLCJUVEFfaSJdLFszLDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMSwzLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzEsNCwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsNCwiQyJdLFszLDEsIlRBX2kiXSxbMCwwLCJUQV9pIl0sWzAsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzAsMSwiVHFeVF9pIiwxXSxbMSwyLCJUcyIsMV0sWzIsMywiXFxtdV9BIl0sWzEsNCwiVGEiLDJdLFs0LDUsInAiXSxbMyw1LCJwIiwyXSxbNiw0LCJUcV9pIl0sWzYsMSwiVFxcdGhldGFfaSBcXGF0b3BcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzcsMCwiVFxcZXRhX3tBX2l9IiwxXSxbNyw2LCIiLDAseyJjdXJ2ZSI6LTIsImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsNiwiVGFfaSIsMV0sWzcsOCwiVHFfaSIsMl0sWzgsMiwiVFxcZXRhX3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaX0iLDFdLFswLDgsIlRcXHRoZXRhJ19pIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsMywiIiwyLHsiY3VydmUiOjMsImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSIsMV0sWzEwLDUsIlxceGlcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDE4LCJUXFxhbHBoYV50X2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMjMsMjEsIlxcemV0YV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9IFxcYXRvcCBcXHNpbWVxIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzI0LDIsIlRcXHNpZ21hIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{TA_i} \\
	{T\underset{I}\oplaxbicolim \; A_i} && {TTA_i} & {TA_i} \\
	&&& {T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	& {TT\underset{I}\oplaxbicolim \; A_i} \\
	& {T\underset{I}\oplaxbicolim \; A_i} &&& C
	\arrow["{Tq^T_i}"{description}, from=2-3, to=3-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "Ts"{description}, from=3-4, to=4-2]
	\arrow["{\mu_A}", from=4-2, to=5-2]
	\arrow["Ta"', from=3-4, to=3-5]
	\arrow["p", from=3-5, to=5-5]
	\arrow["p"', from=5-2, to=5-5]
	\arrow["{Tq_i}", from=2-4, to=3-5]
	\arrow["{T\theta_i \atop\simeq}"{description}, draw=none, from=2-4, to=3-4]
	\arrow["{T\eta_{A_i}}"{description}, from=1-1, to=2-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, curve={height=-12pt}, Rightarrow, no head, from=1-1, to=2-4]
	\arrow["{Ta_i}"{description}, from=2-3, to=2-4]
	\arrow["{Tq_i}"', from=1-1, to=2-1]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{T\eta_{A}}"{description}, from=2-1, to=4-2]
	\arrow["{T\theta'_i \atop \simeq}"{description}, draw=none, from=2-3, to=2-1]
	\arrow[""{name=3, anchor=center, inner sep=0}, curve={height=18pt}, Rightarrow, no head, from=2-1, to=5-2]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{T\underset{I}\oplaxbicolim \; TA_i}"{description}, from=2-1, to=3-4]
	\arrow["{\xi\atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=5-5]
	\arrow["{T\alpha^t_i \atop \simeq}"{description}, Rightarrow, draw=none, from=2-3, to=1]
	\arrow["{\zeta_{A} \atop \simeq}"', Rightarrow, draw=none, from=3, to=2]
	\arrow["{T\sigma \atop \simeq}"{description}, Rightarrow, draw=none, from=4, to=4-2]
\end{tikzcd}\]

Then we recognize the pseudonaturality prism of $T \overline{\alpha}$ we also considered in the first part of the proof of \cref{Codescent object at oplax bicolimit: lower data}: its outer part is an equality face since it relate pseudosections:

% https://q.uiver.app/?q=WzAsOCxbMywyLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzEsMywiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsxLDQsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFs0LDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFs0LDQsIkMiXSxbNCwxLCJUQV9pIl0sWzAsMCwiVEFfaSJdLFswLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDEsIlRzIiwxXSxbMSwyLCJcXG11X0EiXSxbMCwzLCJUYSIsMl0sWzMsNCwicCJdLFsyLDQsInAiLDJdLFs1LDMsIlRxX2kiXSxbNiw1LCIiLDAseyJjdXJ2ZSI6LTIsImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsNywiVHFfaSIsMl0sWzcsMSwiVFxcZXRhX3tBfSIsMV0sWzcsMiwiIiwyLHsiY3VydmUiOjMsImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzcsMCwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSIsMV0sWzcsMywiIiwwLHsiY3VydmUiOi0yLCJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDQsIlxceGlcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxNywxNiwiXFx6ZXRhX3tBfSBcXGF0b3AgXFxzaW1lcSIsMix7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxOCwxLCJUXFxzaWdtYSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxNCwxOSwiPSIsMCx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxOSwwLCJUXFxvdmVybGluZXtcXGFscGhhfV5zIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{TA_i} \\
	{T\underset{I}\oplaxbicolim \; A_i} &&&& {TA_i} \\
	&&& {T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	& {TT\underset{I}\oplaxbicolim \; A_i} \\
	& {T\underset{I}\oplaxbicolim \; A_i} &&& C
	\arrow[""{name=0, anchor=center, inner sep=0}, "Ts"{description}, from=3-4, to=4-2]
	\arrow["{\mu_A}", from=4-2, to=5-2]
	\arrow["Ta"', from=3-4, to=3-5]
	\arrow["p", from=3-5, to=5-5]
	\arrow["p"', from=5-2, to=5-5]
	\arrow["{Tq_i}", from=2-5, to=3-5]
	\arrow[""{name=1, anchor=center, inner sep=0}, curve={height=-12pt}, Rightarrow, no head, from=1-1, to=2-5]
	\arrow["{Tq_i}"', from=1-1, to=2-1]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{T\eta_{A}}"{description}, from=2-1, to=4-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, curve={height=18pt}, Rightarrow, no head, from=2-1, to=5-2]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{T\underset{I}\oplaxbicolim \; TA_i}"{description}, from=2-1, to=3-4]
	\arrow[""{name=5, anchor=center, inner sep=0}, curve={height=-12pt}, Rightarrow, no head, from=2-1, to=3-5]
	\arrow["{\xi\atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=5-5]
	\arrow["{\zeta_{A} \atop \simeq}"', Rightarrow, draw=none, from=3, to=2]
	\arrow["{T\sigma \atop \simeq}"{description}, Rightarrow, draw=none, from=4, to=4-2]
	\arrow["{=}", Rightarrow, draw=none, from=1, to=5]
	\arrow["{T\overline{\alpha}^s}"{description}, Rightarrow, draw=none, from=5, to=3-4]
\end{tikzcd}\]

But we saw that $ p$ satisfy the lower coherence condition from its pseudocoequalizing property of $ U_T\mathscr{X}_{\mathbb{A}}$. Hence the inner surface reduces onto the identity $p$, and the overall diagram reduces onto the identity of $pTq_i$. This ensures the lower coherence condition.\\ 


Now we prove the higher coherence condition. Consider the following pasting - we paste two copies of the inserted 2-cell against the lower projections in the intermediate higher codescent 2-cell:
% https://q.uiver.app/?q=WzAsMTQsWzIsNSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsNSwiQyJdLFszLDAsIlRBX2kiXSxbMCw1LCJUQV9pIl0sWzEsMCwiVFRBX2kiXSxbMCwwLCJUVFRBX2kiXSxbMCwyLCJUVEFfaSJdLFsyLDMsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwyLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzIsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFsxLDQsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMSwzLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzEsMiwiVEFfaSJdLFsxLDIsInAiXSxbMCwyLCJwIiwyXSxbMywxLCJUcV9pIl0sWzQsMCwiVHFfaSIsMl0sWzUsMywiVGFfaSJdLFs2LDcsIlxcbXVfe1RBX2l9IiwyXSxbNyw0LCJcXG11X3tBX2l9IiwyXSxbNiw1LCJUVGFfaSJdLFs1LDEwLCJUcV5UX2kiLDAseyJsYWJlbF9wb3NpdGlvbiI6NzB9XSxbMTAsOSwiVHMiXSxbOSw4LCJcXG11X0EiXSxbMTAsMSwiVGEiLDFdLFs3LDExLCJUVHFfaSIsMl0sWzEyLDExLCJUcyJdLFsxMiw4LCJUYSIsMl0sWzExLDAsIlxcbXVfQSIsMV0sWzcsMTIsIlRxXlRfaSIsMCx7ImxhYmVsX3Bvc2l0aW9uIjo4MH1dLFsxMSw0LCJcXG11X3txX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsMiwicCIsMV0sWzUsOSwiVFRxX2kiLDJdLFs1LDEzLCJcXG11X3tBX2l9IiwxXSxbNywxMywiVGFfaSIsMV0sWzEzLDgsIlRxX2kiLDFdLFsxMiwxMywiVFxcdGhldGFfaSBcXGF0b3BcXHNpbWVxIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsMTMsIlxcbXVfe2FfaSB9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMsMjUsIlRcXHRoZXRhX2kgXFxhdG9wXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMSwzMiwiXFx4aSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMCwzMiwiXFx4aSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyNiwzMCwiVFxcc2lnbWFfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyMiwzMywiVFxcc2lnbWFfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszMywxMywiXFxtdV97cV9pfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}[sep=large]
	{TTTA_i} & {TTA_i} && {TA_i} \\
	&& {T\underset{I}\oplaxbicolim \; TA_i} \\
	{TTA_i} & {TA_i} & {TT\underset{I}\oplaxbicolim \; A_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	& {TT\underset{I}\oplaxbicolim \; A_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	& {T\underset{I}\oplaxbicolim \; TA_i} \\
	{TA_i} && {T\underset{I}\oplaxbicolim \; A_i} & C
	\arrow["p", from=3-4, to=6-4]
	\arrow["p"', from=6-3, to=6-4]
	\arrow["{Tq_i}", from=1-4, to=3-4]
	\arrow["{Tq_i}"', from=6-1, to=6-3]
	\arrow["{Ta_i}", from=1-2, to=1-4]
	\arrow["{\mu_{TA_i}}"', from=1-1, to=3-1]
	\arrow["{\mu_{A_i}}"', from=3-1, to=6-1]
	\arrow["{TTa_i}", from=1-1, to=1-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Tq^T_i}"{pos=0.7}, from=1-2, to=2-3]
	\arrow["Ts", from=2-3, to=3-3]
	\arrow["{\mu_A}", from=3-3, to=4-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Ta"{description}, from=2-3, to=3-4]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{TTq_i}"', from=3-1, to=5-2]
	\arrow["Ts", from=4-2, to=5-2]
	\arrow["Ta"', from=4-2, to=4-3]
	\arrow["{\mu_A}"{description}, from=5-2, to=6-3]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{Tq^T_i}"{pos=0.8}, from=3-1, to=4-2]
	\arrow["{\mu_{q_i} \atop \simeq}"{description}, draw=none, from=5-2, to=6-1]
	\arrow[""{name=4, anchor=center, inner sep=0}, "p"{description}, from=4-3, to=6-4]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{TTq_i}"', from=1-2, to=3-3]
	\arrow["{\mu_{A_i}}"{description}, from=1-2, to=3-2]
	\arrow["{Ta_i}"{description}, from=3-1, to=3-2]
	\arrow["{Tq_i}"{description}, from=3-2, to=4-3]
	\arrow["{T\theta_i \atop\simeq}", draw=none, from=4-2, to=3-2]
	\arrow["{\mu_{a_i } \atop \simeq}"{description}, draw=none, from=1-1, to=3-2]
	\arrow["{T\theta_i \atop\simeq}"{description}, Rightarrow, draw=none, from=1-4, to=1]
	\arrow["{\xi \atop \simeq}"{description}, Rightarrow, draw=none, from=5-2, to=4]
	\arrow["{\xi \atop \simeq}"{description}, Rightarrow, draw=none, from=2-3, to=4]
	\arrow["{T\sigma_i \atop \simeq}"{description}, Rightarrow, draw=none, from=2, to=3]
	\arrow["{T\sigma_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=5]
	\arrow["{\mu_{q_i} \atop \simeq}"{description}, Rightarrow, draw=none, from=5, to=3-2]
\end{tikzcd}\]

We can fill the upper left cube in this diagram thanks to the first codescent condition of the diagram $\mathscr{X}_\mathbb{A}$ of \cref{underlying codescent object} which appears here as the central composite square:
% https://q.uiver.app/?q=WzAsMTUsWzIsNSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsNSwiQyJdLFszLDAsIlRBX2kiXSxbMCw1LCJUQV9pIl0sWzEsMCwiVFRBX2kiXSxbMCwwLCJUVFRBX2kiXSxbMCwyLCJUVEFfaSJdLFsyLDMsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwyLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzIsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFsxLDQsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMSwzLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzEsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVFRBX2kiXSxbMSwyLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFsxLDIsInAiXSxbMCwyLCJwIiwyXSxbMywxLCJUcV9pIl0sWzQsMCwiVHFfaSIsMl0sWzUsMywiVGFfaSJdLFs2LDcsIlxcbXVfe1RBX2l9IiwyXSxbNyw0LCJcXG11X3tBX2l9IiwyXSxbNiw1LCJUVGFfaSJdLFs1LDEwLCJUcV5UX2kiLDAseyJsYWJlbF9wb3NpdGlvbiI6NzB9XSxbMTAsOSwiVHMiXSxbOSw4LCJcXG11X0EiXSxbMTAsMSwiVGEiLDFdLFs3LDExLCJUVHFfaSIsMSx7ImN1cnZlIjoyfV0sWzEyLDExLCJUcyJdLFsxMiw4LCJUYSIsMl0sWzExLDAsIlxcbXVfQSIsMV0sWzcsMTIsIlRxXlRfaSIsMV0sWzExLDQsIlxcbXVfe3FfaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCwyLCJwIiwxXSxbNiwxMywiVHFee1RUfV9pIiwxXSxbMTMsMTAsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRhX2kiLDJdLFsxMywxNCwiVHQiLDJdLFsxNCwxMiwiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pfSIsMV0sWzE0LDksIlRUYSIsMl0sWzYsMTQsIlRUcV5UX2kiLDEseyJjdXJ2ZSI6Mn1dLFs1LDEzLCJUXFx0aGV0YV5UX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsOSwiVFxcdGhldGEgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTQsOCwiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBhX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMsMjYsIlRcXHRoZXRhX2kgXFxhdG9wXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMSwzMywiXFx4aSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMCwzMywiXFx4aSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyNywzMSwiVFxcc2lnbWFfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszNiwzOSwiVFxcdGF1X2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}[sep=large]
	{TTTA_i} & {TTA_i} && {TA_i} \\
	& {T\underset{I}\oplaxbicolim \; TTA_i} & {T\underset{I}\oplaxbicolim \; TA_i} \\
	{TTA_i} & {TT\underset{I}\oplaxbicolim \; TA_i} & {TT\underset{I}\oplaxbicolim \; A_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	& {T\underset{I}\oplaxbicolim \; TA_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	& {TT\underset{I}\oplaxbicolim \; A_i} \\
	{TA_i} && {T\underset{I}\oplaxbicolim \; A_i} & C
	\arrow["p", from=3-4, to=6-4]
	\arrow["p"', from=6-3, to=6-4]
	\arrow["{Tq_i}", from=1-4, to=3-4]
	\arrow["{Tq_i}"', from=6-1, to=6-3]
	\arrow["{Ta_i}", from=1-2, to=1-4]
	\arrow["{\mu_{TA_i}}"', from=1-1, to=3-1]
	\arrow["{\mu_{A_i}}"', from=3-1, to=6-1]
	\arrow["{TTa_i}", from=1-1, to=1-2]
	\arrow["{Tq^T_i}"{pos=0.7}, from=1-2, to=2-3]
	\arrow["Ts", from=2-3, to=3-3]
	\arrow["{\mu_A}", from=3-3, to=4-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "Ta"{description}, from=2-3, to=3-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{TTq_i}"{description}, curve={height=12pt}, from=3-1, to=5-2]
	\arrow["Ts", from=4-2, to=5-2]
	\arrow["Ta"', from=4-2, to=4-3]
	\arrow["{\mu_A}"{description}, from=5-2, to=6-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{Tq^T_i}"{description}, from=3-1, to=4-2]
	\arrow["{\mu_{q_i} \atop \simeq}"{description}, draw=none, from=5-2, to=6-1]
	\arrow[""{name=3, anchor=center, inner sep=0}, "p"{description}, from=4-3, to=6-4]
	\arrow["{Tq^{TT}_i}"{description}, from=1-1, to=2-2]
	\arrow["{T\underset{I}\oplaxbicolim \; Ta_i}"', from=2-2, to=2-3]
	\arrow[""{name=4, anchor=center, inner sep=0}, "Tt"', from=2-2, to=3-2]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"{description}, from=3-2, to=4-2]
	\arrow["TTa"', from=3-2, to=3-3]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{TTq^T_i}"{description}, curve={height=12pt}, from=1-1, to=3-2]
	\arrow["{T\theta^T_i \atop \simeq}"{description}, draw=none, from=1-2, to=2-2]
	\arrow["{T\theta \atop \simeq}"{description}, draw=none, from=2-2, to=3-3]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; a_i} \atop \simeq}"{description}, draw=none, from=3-2, to=4-3]
	\arrow["{T\theta_i \atop\simeq}"{description}, Rightarrow, draw=none, from=1-4, to=0]
	\arrow["{\xi \atop \simeq}"{description}, Rightarrow, draw=none, from=5-2, to=3]
	\arrow["{\xi \atop \simeq}"{description}, Rightarrow, draw=none, from=2-3, to=3]
	\arrow["{T\sigma_i \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=2]
	\arrow["{T\tau_i \atop \simeq}"{description}, Rightarrow, draw=none, from=4, to=5]
\end{tikzcd}\]

But now we can use the fact that $ p : T \oplaxbicolim_I A_i \rightarrow C$ together with $\xi$ pseudocoequalizes $U_T\mathscr{X}_\mathbb{A}$: the higher coherence condition of $\xi$ ensures then that the lower hexagon in the diagram above decomposes as below:


% https://q.uiver.app/?q=WzAsMTYsWzMsNSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsNSwiQyJdLFs0LDAsIlRBX2kiXSxbMCw1LCJUQV9pIl0sWzIsMCwiVFRBX2kiXSxbMCwwLCJUVFRBX2kiXSxbMCwzLCJUVEFfaSJdLFszLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMiw0LCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzEsMywiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFsxLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRUQV9pIl0sWzEsMiwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMyw0LCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsMywiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFsyLDMsIlRUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzEsMiwicCJdLFswLDIsInAiLDJdLFszLDEsIlRxX2kiXSxbNCwwLCJUcV9pIiwyXSxbNSwzLCJUYV9pIl0sWzYsNywiXFxtdV97VEFfaX0iLDJdLFs3LDQsIlxcbXVfe0FfaX0iLDJdLFs2LDUsIlRUYV9pIl0sWzUsOCwiVHFeVF9pIiwwLHsibGFiZWxfcG9zaXRpb24iOjcwfV0sWzgsMSwiVGEiLDFdLFs3LDksIlRUcV9pIiwxLHsiY3VydmUiOjJ9XSxbMTAsOSwiVHMiLDFdLFs5LDAsIlxcbXVfQSIsMV0sWzcsMTAsIlRxXlRfaSJdLFs5LDQsIlxcbXVfe3FfaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiwxMSwiVHFee1RUfV9pIiwxXSxbMTEsOCwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVGFfaSIsMl0sWzExLDEyLCJUdCIsMl0sWzEyLDEwLCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2l9IiwyXSxbNiwxMiwiVFRxXlRfaSIsMSx7ImN1cnZlIjoyfV0sWzUsMTEsIlRcXHRoZXRhXlRfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMywwLCJcXG11X0EiXSxbMTQsMSwiVGEiLDJdLFsxNCwyLCJcXHhpIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE0LDEzLCJUcyJdLFsxMSwxNCwiXFxzbWFsbHtUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBcXG11X3tBX2l9fSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo2MH1dLFs4LDE0LCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBcXGFscGhhXnNfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxNSwxMywiVFxcbXVfQSIsMV0sWzEyLDE1LCJUVHMiLDFdLFsxNSw5LCJcXG11X3tUQX0iXSxbMywyNSwiVFxcdGhldGFfaSBcXGF0b3BcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMzLDM1LCJUXFx0YXVfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyNiwyNywiVFxcc2lnbWFfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0NCwyNywiXFxtdV9zIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzQzLDI4LCJcXHJob19BIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE1LDQxLCJUXFx0YXUgXFxhdG9wIFxcc2ltZXEiLDAseyJsYWJlbF9wb3NpdGlvbiI6NDAsInNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	{TTTA_i} && {TTA_i} && {TA_i} \\
	& {T\underset{I}\oplaxbicolim \; TTA_i} && {T\underset{I}\oplaxbicolim \; TA_i} \\
	& {TT\underset{I}\oplaxbicolim \; TA_i} &&& {T\underset{I}\oplaxbicolim \; A_i} \\
	{TTA_i} & {T\underset{I}\oplaxbicolim \; TA_i} & {TTT\underset{I}\oplaxbicolim \; A_i} & {T\underset{I}\oplaxbicolim \; TA_i} \\
	&& {TT\underset{I}\oplaxbicolim \; A_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	{TA_i} &&& {T\underset{I}\oplaxbicolim \; A_i} & C
	\arrow["p", from=3-5, to=6-5]
	\arrow["p"', from=6-4, to=6-5]
	\arrow["{Tq_i}", from=1-5, to=3-5]
	\arrow["{Tq_i}"', from=6-1, to=6-4]
	\arrow["{Ta_i}", from=1-3, to=1-5]
	\arrow["{\mu_{TA_i}}"', from=1-1, to=4-1]
	\arrow["{\mu_{A_i}}"', from=4-1, to=6-1]
	\arrow["{TTa_i}", from=1-1, to=1-3]
	\arrow["{Tq^T_i}"{pos=0.7}, from=1-3, to=2-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "Ta"{description}, from=2-4, to=3-5]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{TTq_i}"{description}, curve={height=12pt}, from=4-1, to=5-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "Ts"{description}, from=4-2, to=5-3]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\mu_A}"{description}, from=5-3, to=6-4]
	\arrow["{Tq^T_i}", from=4-1, to=4-2]
	\arrow["{\mu_{q_i} \atop \simeq}"{description}, draw=none, from=5-3, to=6-1]
	\arrow["{Tq^{TT}_i}"{description}, from=1-1, to=2-2]
	\arrow["{T\underset{I}\oplaxbicolim \; Ta_i}"', from=2-2, to=2-4]
	\arrow[""{name=4, anchor=center, inner sep=0}, "Tt"', from=2-2, to=3-2]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"', from=3-2, to=4-2]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{TTq^T_i}"{description}, curve={height=12pt}, from=1-1, to=3-2]
	\arrow["{T\theta^T_i \atop \simeq}"{description}, draw=none, from=1-3, to=2-2]
	\arrow["{\mu_A}", from=5-4, to=6-4]
	\arrow["Ta"', from=4-4, to=3-5]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=4-4, to=6-5]
	\arrow["Ts", from=4-4, to=5-4]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\small{T\underset{I}\oplaxbicolim \; \mu_{A_i}}}"{description, pos=0.6}, from=2-2, to=4-4]
	\arrow["{T\underset{I}\oplaxbicolim \; \alpha^s_i \atop \simeq}"{description}, draw=none, from=2-4, to=4-4]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{T\mu_A}"{description}, from=4-3, to=5-4]
	\arrow[""{name=8, anchor=center, inner sep=0}, "TTs"{description}, from=3-2, to=4-3]
	\arrow["{\mu_{TA}}", from=4-3, to=5-3]
	\arrow["{T\theta_i \atop\simeq}"{description}, Rightarrow, draw=none, from=1-5, to=0]
	\arrow["{T\tau_i \atop \simeq}"{description}, Rightarrow, draw=none, from=4, to=5]
	\arrow["{T\sigma_i \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=2]
	\arrow["{\mu_s \atop \simeq}"{description}, Rightarrow, draw=none, from=8, to=2]
	\arrow["{\rho_A \atop \simeq}"{description}, Rightarrow, draw=none, from=7, to=3]
	\arrow["{T\tau \atop \simeq}"{pos=0.4}, Rightarrow, draw=none, from=4-3, to=6]
\end{tikzcd}\]

Now we must force the middle higher codescent projection $ T\mu_{A_i}$ appear in the diagram. This is possible by recognizing in the diagram above the front faces of the following cube the bicolimit projections defines over the associated codescent 2-cells, in the upper right part of the diagram above:



% https://q.uiver.app/?q=WzAsNyxbMSwzLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwyLCJUQV9pIl0sWzIsMCwiVFRBX2kiXSxbMSwwLCJUVFRBX2kiXSxbMSwxLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzAsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVFRBX2kiXSxbMCwzLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzEsMCwiVHFfaSJdLFsyLDEsIlRhX2kiXSxbMywyLCJUVGFfaSJdLFsyLDQsIlRxXlRfaSIsMCx7ImxhYmVsX3Bvc2l0aW9uIjo3MH1dLFs0LDAsIlRhIiwxXSxbMyw1LCJUcV57VFR9X2kiLDFdLFs1LDQsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRhX2kiLDJdLFsyLDUsIlRcXHRoZXRhXlRfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs2LDAsIlRhIiwyXSxbNSw2LCJcXHNtYWxse1RcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFxcbXVfe0FfaX19IiwxLHsibGFiZWxfcG9zaXRpb24iOjYwfV0sWzQsNiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgXFxhbHBoYV5zX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCwxMSwiVFxcdGhldGFfaSBcXGF0b3BcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	& {TTTA_i} & {TTA_i} \\
	{T\underset{I}\oplaxbicolim \; TTA_i} & {T\underset{I}\oplaxbicolim \; TA_i} \\
	&& {TA_i} \\
	{T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i}
	\arrow["{Tq_i}", from=3-3, to=4-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Ta_i}", from=1-3, to=3-3]
	\arrow["{TTa_i}", from=1-2, to=1-3]
	\arrow["{Tq^T_i}"{pos=0.7}, from=1-3, to=2-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Ta"{description}, from=2-2, to=4-2]
	\arrow["{Tq^{TT}_i}"', from=1-2, to=2-1]
	\arrow["{T\underset{I}\oplaxbicolim \; Ta_i}"', from=2-1, to=2-2]
	\arrow["{T\theta^T_i \atop \simeq}"{description}, draw=none, from=1-3, to=2-1]
	\arrow["Ta"', from=4-1, to=4-2]
	\arrow["{\small{T\underset{I}\oplaxbicolim \; \mu_{A_i}}}"{description, pos=0.6}, from=2-1, to=4-1]
	\arrow["{T\underset{I}\oplaxbicolim \; \alpha^s_i \atop \simeq}"{description}, draw=none, from=2-2, to=4-1]
	\arrow["{T\theta_i \atop\simeq}"{description}, Rightarrow, draw=none, from=0, to=1]
\end{tikzcd}\]
% https://q.uiver.app/?q=WzAsNyxbMSwzLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwyLCJUQV9pIl0sWzIsMCwiVFRBX2kiXSxbMSwwLCJUVFRBX2kiXSxbMCwxLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUVEFfaSJdLFswLDMsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMSwyLCJUVEEiXSxbMSwwLCJUcV9pIl0sWzIsMSwiVGFfaSJdLFszLDIsIlRUYV9pIl0sWzMsNCwiVHFee1RUfV9pIiwyXSxbNSwwLCJUYSIsMl0sWzQsNSwiXFxzbWFsbHtUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBcXG11X3tBX2l9fSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo2MH1dLFszLDYsIlRcXG11X3tBX2l9IiwxXSxbNiw1LCJUcV5UX2kiLDFdLFs2LDEsIlRhX2kiLDFdLFs2LDIsIlRcXGFscGhhXnNfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDYsIlRcXG11X3txX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[=\begin{tikzcd}
	& {TTTA_i} & {TTA_i} \\
	{T\underset{I}\oplaxbicolim \; TTA_i} \\
	& TTA & {TA_i} \\
	{T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i}
	\arrow["{Tq_i}", from=3-3, to=4-2]
	\arrow["{Ta_i}", from=1-3, to=3-3]
	\arrow["{TTa_i}", from=1-2, to=1-3]
	\arrow["{Tq^{TT}_i}"', from=1-2, to=2-1]
	\arrow["Ta"', from=4-1, to=4-2]
	\arrow["{\small{T\underset{I}\oplaxbicolim \; \mu_{A_i}}}"{description, pos=0.6}, from=2-1, to=4-1]
	\arrow["{T\mu_{A_i}}"{description}, from=1-2, to=3-2]
	\arrow["{Tq^T_i}"{description}, from=3-2, to=4-1]
	\arrow["{Ta_i}"{description}, from=3-2, to=3-3]
	\arrow["{T\alpha^s_i \atop \simeq}"{description}, draw=none, from=3-2, to=1-3]
	\arrow["{T\mu_{q_i} \atop \simeq}"{description}, draw=none, from=2-1, to=3-2]
\end{tikzcd}\]
Then one can substitute the three front faces with their corresponding three opposite back faces as in the diagram below:

% % https://q.uiver.app/?q=WzAsMTYsWzMsNSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsNSwiQyJdLFs0LDAsIlRBX2kiXSxbMCw1LCJUQV9pIl0sWzMsMCwiVFRBX2kiXSxbMCwwLCJUVFRBX2kiXSxbMCwzLCJUVEFfaSJdLFsyLDQsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMSwzLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzEsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVFRBX2kiXSxbMSwyLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFszLDQsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMywzLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzIsMywiVFRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMywxLCJUVEFfaSJdLFsxLDIsInAiXSxbMCwyLCJwIiwyXSxbMywxLCJUcV9pIl0sWzQsMCwiVHFfaSIsMl0sWzUsMywiVGFfaSJdLFs2LDcsIlxcbXVfe1RBX2l9IiwyXSxbNyw0LCJcXG11X3tBX2l9IiwyXSxbNiw1LCJUVGFfaSJdLFs3LDgsIlRUcV9pIiwxLHsiY3VydmUiOjJ9XSxbOSw4LCJUcyIsMV0sWzgsMCwiXFxtdV9BIiwxXSxbNyw5LCJUcV5UX2kiXSxbOCw0LCJcXG11X3txX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsMTAsIlRxXntUVH1faSIsMV0sWzEwLDExLCJUdCIsMl0sWzExLDksIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaX0iLDJdLFs2LDExLCJUVHFeVF9pIiwxLHsiY3VydmUiOjJ9XSxbNSwxMCwiVFxcdGhldGFeVF9pIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEyLDAsIlxcbXVfQSJdLFsxMywxLCJUYSIsMl0sWzEzLDIsIlxceGkgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMTIsIlRzIl0sWzEwLDEzLCJcXHNtYWxse1RcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFxcbXVfe0FfaX19IiwxLHsibGFiZWxfcG9zaXRpb24iOjYwfV0sWzE0LDEyLCJUXFxtdV9BIiwxXSxbMTEsMTQsIlRUcyIsMV0sWzE0LDgsIlxcbXVfe1RBfSJdLFs2LDE1LCJUXFxtdV97QV9pfSIsMV0sWzE1LDEzLCJUcV5UX2kiLDFdLFsxNSwzLCJUYV9pIiwxXSxbMTUsMSwiVFxcdGhldGFfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszMCwzMiwiVFxcdGF1X2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMjQsMjUsIlRcXHNpZ21hX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNDAsMjUsIlxcbXVfcyBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszOSwyNiwiXFxyaG9fQSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxNCwzOCwiVFxcdGF1IFxcYXRvcCBcXHNpbWVxIiwwLHsibGFiZWxfcG9zaXRpb24iOjQwLCJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMzgsMTUsIlRcXG11X3txX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{TTTA_i} &&& {TTA_i} & {TA_i} \\
	& {T\underset{I}\oplaxbicolim \; TTA_i} && {TTA_i} \\
	& {TT\underset{I}\oplaxbicolim \; TA_i} &&& {T\underset{I}\oplaxbicolim \; A_i} \\
	{TTA_i} & {T\underset{I}\oplaxbicolim \; TA_i} & {TTT\underset{I}\oplaxbicolim \; A_i} & {T\underset{I}\oplaxbicolim \; TA_i} \\
	&& {TT\underset{I}\oplaxbicolim \; A_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	{TA_i} &&& {T\underset{I}\oplaxbicolim \; A_i} & C
	\arrow["p", from=3-5, to=6-5]
	\arrow["p"', from=6-4, to=6-5]
	\arrow["{Tq_i}", from=1-5, to=3-5]
	\arrow["{Tq_i}"', from=6-1, to=6-4]
	\arrow["{Ta_i}", from=1-4, to=1-5]
	\arrow["{\mu_{TA_i}}"', from=1-1, to=4-1]
	\arrow["{\mu_{A_i}}"', from=4-1, to=6-1]
	\arrow["{TTa_i}", from=1-1, to=1-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{TTq_i}"{description}, curve={height=12pt}, from=4-1, to=5-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Ts"{description}, from=4-2, to=5-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\mu_A}"{description}, from=5-3, to=6-4]
	\arrow["{Tq^T_i}", from=4-1, to=4-2]
	\arrow["{\mu_{q_i} \atop \simeq}"{description}, draw=none, from=5-3, to=6-1]
	\arrow["{Tq^{TT}_i}"{description}, from=1-1, to=2-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, "Tt"', from=2-2, to=3-2]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"', from=3-2, to=4-2]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{TTq^T_i}"{description}, curve={height=12pt}, from=1-1, to=3-2]
	\arrow["{T\theta^T_i \atop \simeq}"{description}, draw=none, from=1-4, to=2-2]
	\arrow["{\mu_A}", from=5-4, to=6-4]
	\arrow["Ta"', from=4-4, to=3-5]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=4-4, to=6-5]
	\arrow["Ts", from=4-4, to=5-4]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{\small{T\underset{I}\oplaxbicolim \; \mu_{A_i}}}"{description, pos=0.6}, from=2-2, to=4-4]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{T\mu_A}"{description}, from=4-3, to=5-4]
	\arrow[""{name=7, anchor=center, inner sep=0}, "TTs"{description}, from=3-2, to=4-3]
	\arrow["{\mu_{TA}}", from=4-3, to=5-3]
	\arrow["{T\mu_{A_i}}"{description}, from=1-1, to=2-4]
	\arrow["{Tq^T_i}"{description}, from=2-4, to=4-4]
	\arrow["{Ta_i}"{description}, from=2-4, to=1-5]
	\arrow["{T\theta_i \atop \simeq}"{description}, draw=none, from=2-4, to=3-5]
	\arrow["{T\tau_i \atop \simeq}"{description}, Rightarrow, draw=none, from=3, to=4]
	\arrow["{T\sigma_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=1]
	\arrow["{\mu_s \atop \simeq}"{description}, Rightarrow, draw=none, from=7, to=1]
	\arrow["{\rho_A \atop \simeq}"{description}, Rightarrow, draw=none, from=6, to=2]
	\arrow["{T\tau \atop \simeq}"{pos=0.4}, Rightarrow, draw=none, from=4-3, to=5]
	\arrow["{T\mu_{q_i} \atop \simeq}"{description}, Rightarrow, draw=none, from=5, to=2-4]
\end{tikzcd}\]


Now recognize the presence in the diagram above of the back three faces of the following prism in the middle left part:
% https://q.uiver.app/?q=WzAsNixbMCwwLCJUVFRBX2kiXSxbMCwxLCJUVEFfaSJdLFsyLDIsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMSwxLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzEsMCwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMiwxLCJUVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDEsIlxcbXVfe1RBX2l9IiwyXSxbMSwyLCJUVHFfaSIsMix7ImN1cnZlIjozfV0sWzMsMiwiVHMiLDFdLFsxLDMsIlRxXlRfaSJdLFs0LDMsIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaX0iLDJdLFs0LDUsIlRUcyIsMV0sWzUsMiwiXFxtdV97VEF9Il0sWzAsNCwiVFRxXlRfaSJdLFs3LDgsIlRcXHNpZ21hX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTEsOCwiXFxtdV9zIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{TTTA_i} & {TT\underset{I}\oplaxbicolim \; TA_i} \\
	{TTA_i} & {T\underset{I}\oplaxbicolim \; TA_i} & {TTT\underset{I}\oplaxbicolim \; A_i} \\
	&& {TT\underset{I}\oplaxbicolim \; A_i}
	\arrow["{\mu_{TA_i}}"', from=1-1, to=2-1]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{TTq_i}"', curve={height=18pt}, from=2-1, to=3-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Ts"{description}, from=2-2, to=3-3]
	\arrow["{Tq^T_i}", from=2-1, to=2-2]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"', from=1-2, to=2-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, "TTs"{description}, from=1-2, to=2-3]
	\arrow["{\mu_{TA}}", from=2-3, to=3-3]
	\arrow["{TTq^T_i}", from=1-1, to=1-2]
	\arrow["{T\sigma_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=1]
	\arrow["{\mu_s \atop \simeq}"{description}, Rightarrow, draw=none, from=2, to=1]
\end{tikzcd}\]
% https://q.uiver.app/?q=WzAsNSxbMCwwLCJUVEFfaSJdLFswLDEsIlRBX2kiXSxbMywyLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwwLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzMsMSwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDEsIlxcbXVfe0FfaX0iLDJdLFswLDMsIlRxXlRfaSIsMV0sWzEsMiwiVHFfaSIsMix7ImN1cnZlIjozfV0sWzQsMiwiXFxtdV97QX0iXSxbMyw0LCJUcyJdLFswLDQsIlRUcV9pIiwxLHsibGFiZWxfcG9zaXRpb24iOjQwLCJjdXJ2ZSI6M31dLFsxMCw3LCJcXG11X3txX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsibGFiZWxfcG9zaXRpb24iOjQwLCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTAsOSwiVFxcc2lnbWFfaSBcXGF0b3AgXFxzaW1lcSIsMCx7ImxhYmVsX3Bvc2l0aW9uIjozMCwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[=\begin{tikzcd}
	{TTA_i} && {T\underset{I}\oplaxbicolim \; TA_i} \\
	{TA_i} &&& {TT\underset{I}\oplaxbicolim \; A_i} \\
	&&& {T\underset{I}\oplaxbicolim \; A_i}
	\arrow["{\mu_{A_i}}"', from=1-1, to=2-1]
	\arrow["{Tq^T_i}"{description}, from=1-1, to=1-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Tq_i}"', curve={height=18pt}, from=2-1, to=3-4]
	\arrow["{\mu_{A}}", from=2-4, to=3-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Ts", from=1-3, to=2-4]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{TTq_i}"{description, pos=0.4}, curve={height=18pt}, from=1-1, to=2-4]
	\arrow["{\mu_{q_i} \atop \simeq}"{description, pos=0.4}, Rightarrow, draw=none, from=2, to=0]
	\arrow["{TT\sigma_i \atop \simeq}"{pos=0.3}, Rightarrow, draw=none, from=2, to=1]
\end{tikzcd}\]

and substitute them with the front three faces as in the following diagram
% https://q.uiver.app/?q=WzAsMTUsWzMsNSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsNSwiQyJdLFs0LDAsIlRBX2kiXSxbMCw1LCJUQV9pIl0sWzMsMCwiVFRBX2kiXSxbMCwwLCJUVFRBX2kiXSxbMCwzLCJUVEFfaSJdLFsyLDQsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwxLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUVEFfaSJdLFsyLDIsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzMsNCwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMiwzLCJUVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDEsIlRUQV9pIl0sWzEsMiwicCJdLFswLDIsInAiLDJdLFszLDEsIlRxX2kiXSxbNCwwLCJUcV9pIiwyXSxbNSwzLCJUYV9pIl0sWzYsNywiXFxtdV97VEFfaX0iLDJdLFs3LDQsIlxcbXVfe0FfaX0iLDJdLFs2LDUsIlRUYV9pIl0sWzgsMCwiXFxtdV9BIiwxXSxbOCw0LCJcXG11X3txX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsOSwiVHFee1RUfV9pIiwxXSxbOSwxMCwiVHQiLDJdLFs2LDEwLCJUVHFeVF9pIiwxLHsiY3VydmUiOjJ9XSxbNSw5LCJUXFx0aGV0YV5UX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTEsMCwiXFxtdV9BIl0sWzEyLDEsIlRhIiwyXSxbMTIsMiwiXFx4aSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMiwxMSwiVHMiXSxbOSwxMiwiXFxzbWFsbHtUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBcXG11X3tBX2l9fSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjozMCwiY3VydmUiOi0xfV0sWzEzLDExLCJUXFxtdV9BIiwxXSxbMTAsMTMsIlRUcyIsMl0sWzEzLDgsIlxcbXVfe1RBfSJdLFs2LDE0LCJUXFxtdV97QV9pfSIsMSx7ImN1cnZlIjotMX1dLFsxNCwxMiwiVHFeVF9pIiwxXSxbMTQsMywiVGFfaSIsMV0sWzE0LDEsIlRcXHRoZXRhX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiwxMywiVFRUcV9pIiwxLHsibGFiZWxfcG9zaXRpb24iOjgwLCJjdXJ2ZSI6M31dLFsxMyw3LCJcXG11X3tUcV9pfSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs3LDgsIlRUcV9pIiwxLHsiY3VydmUiOjJ9XSxbMjYsMjcsIlRcXHRhdV9pIFxcYXRvcCBcXHNpbWVxIiwxLHsibGFiZWxfcG9zaXRpb24iOjQwLCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMzQsMjMsIlxccmhvX0EgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMzMsIlRcXHRhdSBcXGF0b3AgXFxzaW1lcSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMzLDE0LCJUXFxtdV97cV9pfSBcXGF0b3AgXFxzaW1lcSIsMCx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMCw0MSwiVFRcXHNpZ21hX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJsYWJlbF9wb3NpdGlvbiI6NDAsInNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	{TTTA_i} &&& {TTA_i} & {TA_i} \\
	&& {T\underset{I}\oplaxbicolim \; TTA_i} & {TTA_i} \\
	&& {TT\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	{TTA_i} && {TTT\underset{I}\oplaxbicolim \; A_i} \\
	&& {TT\underset{I}\oplaxbicolim \; A_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	{TA_i} &&& {T\underset{I}\oplaxbicolim \; A_i} & C
	\arrow["p", from=3-5, to=6-5]
	\arrow["p"', from=6-4, to=6-5]
	\arrow["{Tq_i}", from=1-5, to=3-5]
	\arrow["{Tq_i}"', from=6-1, to=6-4]
	\arrow["{Ta_i}", from=1-4, to=1-5]
	\arrow["{\mu_{TA_i}}"', from=1-1, to=4-1]
	\arrow["{\mu_{A_i}}"', from=4-1, to=6-1]
	\arrow["{TTa_i}", from=1-1, to=1-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\mu_A}"{description}, from=5-3, to=6-4]
	\arrow["{\mu_{q_i} \atop \simeq}"{description}, draw=none, from=5-3, to=6-1]
	\arrow["{Tq^{TT}_i}"{description}, from=1-1, to=2-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Tt"', from=2-3, to=3-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{TTq^T_i}"{description}, curve={height=12pt}, from=1-1, to=3-3]
	\arrow["{T\theta^T_i \atop \simeq}"{description}, draw=none, from=1-4, to=2-3]
	\arrow["{\mu_A}", from=5-4, to=6-4]
	\arrow["Ta"', from=3-4, to=3-5]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=3-4, to=6-5]
	\arrow["Ts", from=3-4, to=5-4]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\small{T\underset{I}\oplaxbicolim \; \mu_{A_i}}}"{description, pos=0.3}, curve={height=-6pt}, from=2-3, to=3-4]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{T\mu_A}"{description}, from=4-3, to=5-4]
	\arrow["TTs"', from=3-3, to=4-3]
	\arrow["{\mu_{TA}}", from=4-3, to=5-3]
	\arrow["{T\mu_{A_i}}"{description}, curve={height=-6pt}, from=1-1, to=2-4]
	\arrow["{Tq^T_i}"{description}, from=2-4, to=3-4]
	\arrow["{Ta_i}"{description}, from=2-4, to=1-5]
	\arrow["{T\theta_i \atop \simeq}"{description}, draw=none, from=2-4, to=3-5]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{TTTq_i}"{description, pos=0.8}, curve={height=18pt}, from=1-1, to=4-3]
	\arrow["{\mu_{Tq_i} \atop \simeq}"{description}, draw=none, from=4-3, to=4-1]
	\arrow["{TTq_i}"{description}, curve={height=12pt}, from=4-1, to=5-3]
	\arrow["{T\tau_i \atop \simeq}"{description, pos=0.4}, Rightarrow, draw=none, from=1, to=2]
	\arrow["{\rho_A \atop \simeq}"{description}, Rightarrow, draw=none, from=4, to=0]
	\arrow["{T\tau \atop \simeq}"{description, pos=0.4}, Rightarrow, draw=none, from=4-3, to=3]
	\arrow["{T\mu_{q_i} \atop \simeq}", Rightarrow, draw=none, from=3, to=2-4]
	\arrow["{TT\sigma_i \atop \simeq}"{description, pos=0.4}, Rightarrow, draw=none, from=3-3, to=5]
\end{tikzcd}\]

It is possible now to recognize the three back faces of the following cube associated to the multiplication part:

% https://q.uiver.app/?q=WzAsNyxbMCwwLCJUVFRBX2kiXSxbMCwxLCJUVEFfaSJdLFsxLDIsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMSwwLCJUVEFfaSJdLFsyLDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsyLDEsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMSwxLCJUVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDEsIlxcbXVfe1RBX2l9IiwyXSxbMSwyLCJUVHFfaSIsMl0sWzAsMywiVFxcbXVfe1RBX2l9Il0sWzIsNCwiXFxtdV97QX0iLDJdLFs1LDQsIlxcbXVfe0F9Il0sWzMsNSwiVFRxX2kiLDAseyJsYWJlbF9wb3NpdGlvbiI6NDB9XSxbNiwyLCJcXG11X3tUQX0iXSxbNiw1LCJUXFxtdV9BIiwyXSxbMCw2LCJUVFRxX2kiLDFdLFs2LDQsIlxccmhvX0EgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMSw2LCJcXG11X1RxX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMyw2LCJUXFxtdV97cV9pfSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	{TTTA_i} & {TTA_i} \\
	{TTA_i} & {TTT\underset{I}\oplaxbicolim \; A_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	& {TT\underset{I}\oplaxbicolim \; A_i} & {T\underset{I}\oplaxbicolim \; A_i}
	\arrow["{\mu_{TA_i}}"', from=1-1, to=2-1]
	\arrow["{TTq_i}"', from=2-1, to=3-2]
	\arrow["{T\mu_{TA_i}}", from=1-1, to=1-2]
	\arrow["{\mu_{A}}"', from=3-2, to=3-3]
	\arrow["{\mu_{A}}", from=2-3, to=3-3]
	\arrow["{TTq_i}"{pos=0.4}, from=1-2, to=2-3]
	\arrow["{\mu_{TA}}", from=2-2, to=3-2]
	\arrow["{T\mu_A}"', from=2-2, to=2-3]
	\arrow["{TTTq_i}"{description}, from=1-1, to=2-2]
	\arrow["{\rho_A \atop \simeq}"{description}, draw=none, from=2-2, to=3-3]
	\arrow["{\mu_{Tq_i} \atop \simeq}"{description}, draw=none, from=2-1, to=2-2]
	\arrow["{T\mu_{q_i} \atop \simeq}"{description}, draw=none, from=1-2, to=2-2]
\end{tikzcd}\]
% https://q.uiver.app/?q=WzAsNyxbMCwwLCJUVFRBX2kiXSxbMCwxLCJUVEFfaSJdLFsxLDIsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMSwwLCJUVEFfaSJdLFsxLDEsIlRBX2kiXSxbMiwyLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwxLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzAsMSwiXFxtdV97VEFfaX0iLDJdLFsxLDIsIlRUcV9pIiwyXSxbMCwzLCJUXFxtdV97VEFfaX0iXSxbMyw0LCJcXG11X3tBX2l9IiwyXSxbMSw0LCJcXG11X3tBX2l9IiwxXSxbNCw1LCJUcV9pIiwxLHsibGFiZWxfcG9zaXRpb24iOjIwfV0sWzIsNSwiXFxtdV97QX0iLDJdLFs2LDUsIlxcbXVfe0F9Il0sWzMsNiwiVFRxX2kiLDAseyJsYWJlbF9wb3NpdGlvbiI6NDB9XSxbNCw3LCJcXHJob197e0FfaX19IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIsMTEsIlxcbXVfe3FfaX0gXFxhdG9wIFxcc2ltZXEiLDIseyJsYWJlbF9wb3NpdGlvbiI6MzAsInNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxNSwxMiwiXFxtdV97cV9pfSBcXGF0b3AgXFxzaW1lcSIsMix7ImxhYmVsX3Bvc2l0aW9uIjo0MCwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[=\begin{tikzcd}
	{TTTA_i} & {TTA_i} \\
	{TTA_i} & {TA_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	& {TT\underset{I}\oplaxbicolim \; A_i} & {T\underset{I}\oplaxbicolim \; A_i}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\mu_{TA_i}}"', from=1-1, to=2-1]
	\arrow["{TTq_i}"', from=2-1, to=3-2]
	\arrow["{T\mu_{TA_i}}", from=1-1, to=1-2]
	\arrow["{\mu_{A_i}}"', from=1-2, to=2-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\mu_{A_i}}"{description}, from=2-1, to=2-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{Tq_i}"{description, pos=0.2}, from=2-2, to=3-3]
	\arrow["{\mu_{A}}"', from=3-2, to=3-3]
	\arrow["{\mu_{A}}", from=2-3, to=3-3]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{TTq_i}"{pos=0.4}, from=1-2, to=2-3]
	\arrow["{\rho_{{A_i}} \atop \simeq}"{description}, Rightarrow, draw=none, from=2-2, to=1-1]
	\arrow["{\mu_{q_i} \atop \simeq}"'{pos=0.3}, Rightarrow, draw=none, from=3-2, to=1]
	\arrow["{\mu_{q_i} \atop \simeq}"'{pos=0.4}, Rightarrow, draw=none, from=3, to=2]
\end{tikzcd}\]


Then we can subsitute them with their opposite front faces as in the diagram below
% https://q.uiver.app/?q=WzAsMTUsWzMsNSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsNSwiQyJdLFs0LDAsIlRBX2kiXSxbMCw1LCJUQV9pIl0sWzMsMCwiVFRBX2kiXSxbMCwwLCJUVFRBX2kiXSxbMCwzLCJUVEFfaSJdLFsyLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRUQV9pIl0sWzIsMiwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMyw0LCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFsyLDMsIlRUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsMSwiVFRBX2kiXSxbMiw0LCJUVEFfaSJdLFsxLDIsInAiXSxbMCwyLCJwIiwyXSxbMywxLCJUcV9pIl0sWzQsMCwiVHFfaSIsMl0sWzUsMywiVGFfaSJdLFs2LDcsIlxcbXVfe1RBX2l9IiwyXSxbNyw0LCJcXG11X3tBX2l9IiwyXSxbNiw1LCJUVGFfaSJdLFs2LDgsIlRxXntUVH1faSIsMV0sWzgsOSwiVHQiLDJdLFs2LDksIlRUcV5UX2kiLDEseyJjdXJ2ZSI6MX1dLFs1LDgsIlRcXHRoZXRhXlRfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMCwwLCJcXG11X0EiXSxbMTEsMSwiVGEiLDJdLFsxMSwyLCJcXHhpIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzExLDEwLCJUcyJdLFs4LDExLCJcXHNtYWxse1RcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFxcbXVfe0FfaX19IiwxLHsibGFiZWxfcG9zaXRpb24iOjMwfV0sWzEyLDEwLCJUXFxtdV9BIiwxXSxbOSwxMiwiVFRzIiwyXSxbNiwxMywiVFxcbXVfe0FfaX0iLDEseyJjdXJ2ZSI6LTF9XSxbMTMsMTEsIlRxXlRfaSJdLFsxMywzLCJUYV9pIiwxXSxbMTMsMSwiVFxcdGhldGFfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs2LDEyLCJUVFRxX2kiLDEseyJsYWJlbF9wb3NpdGlvbiI6ODAsImN1cnZlIjoyfV0sWzYsMTQsIlRcXG11X3tBX2l9IiwxLHsiY3VydmUiOjN9XSxbMTQsNCwiXFxtdV97QV9pfSIsMV0sWzE0LDEwLCJUVHFfaSIsMV0sWzE0LDEyLCJUXFxtdV97cV9pfVxcYXRvcCBcXHNpbWVxIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE0LDAsIlxcbXVfe1RxX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzI0LDI1LCJUXFx0YXVfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMiwzMSwiVFxcdGF1IFxcYXRvcCBcXHNpbWVxIiwxLHsibGFiZWxfcG9zaXRpb24iOjQwLCJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMzEsMTMsIlRcXG11X3txX2l9IFxcYXRvcCBcXHNpbWVxIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzksMzgsIlRUXFxzaWdtYV9pIFxcYXRvcCBcXHNpbWVxIiwxLHsibGFiZWxfcG9zaXRpb24iOjQwLCJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNDAsNywiXFxyaG9fe0FfaX0gXFxhdG9wIFxcc2ltZXEiLDIseyJsZXZlbCI6MSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{TTTA_i} &&& {TTA_i} & {TA_i} \\
	&& {T\underset{I}\oplaxbicolim \; TTA_i} & {TTA_i} \\
	&& {TT\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	{TTA_i} && {TTT\underset{I}\oplaxbicolim \; A_i} \\
	&& {TTA_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	{TA_i} &&& {T\underset{I}\oplaxbicolim \; A_i} & C
	\arrow["p", from=3-5, to=6-5]
	\arrow["p"', from=6-4, to=6-5]
	\arrow["{Tq_i}", from=1-5, to=3-5]
	\arrow["{Tq_i}"', from=6-1, to=6-4]
	\arrow["{Ta_i}", from=1-4, to=1-5]
	\arrow["{\mu_{TA_i}}"', from=1-1, to=4-1]
	\arrow["{\mu_{A_i}}"', from=4-1, to=6-1]
	\arrow["{TTa_i}", from=1-1, to=1-4]
	\arrow["{Tq^{TT}_i}"{description}, from=1-1, to=2-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "Tt"', from=2-3, to=3-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{TTq^T_i}"{description}, curve={height=6pt}, from=1-1, to=3-3]
	\arrow["{T\theta^T_i \atop \simeq}"{description}, draw=none, from=1-4, to=2-3]
	\arrow["{\mu_A}", from=5-4, to=6-4]
	\arrow["Ta"', from=3-4, to=3-5]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=3-4, to=6-5]
	\arrow["Ts", from=3-4, to=5-4]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\small{T\underset{I}\oplaxbicolim \; \mu_{A_i}}}"{description, pos=0.3}, from=2-3, to=3-4]
	\arrow["{T\mu_A}"{description}, from=4-3, to=5-4]
	\arrow["TTs"', from=3-3, to=4-3]
	\arrow["{T\mu_{A_i}}"{description}, curve={height=-6pt}, from=1-1, to=2-4]
	\arrow["{Tq^T_i}", from=2-4, to=3-4]
	\arrow["{Ta_i}"{description}, from=2-4, to=1-5]
	\arrow["{T\theta_i \atop \simeq}"{description}, draw=none, from=2-4, to=3-5]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{TTTq_i}"{description, pos=0.8}, curve={height=12pt}, from=1-1, to=4-3]
	\arrow["{T\mu_{A_i}}"{description}, curve={height=18pt}, from=1-1, to=5-3]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{\mu_{A_i}}"{description}, from=5-3, to=6-1]
	\arrow["{TTq_i}"{description}, from=5-3, to=5-4]
	\arrow["{T\mu_{q_i}\atop \simeq}"', draw=none, from=5-3, to=4-3]
	\arrow["{\mu_{Tq_i} \atop \simeq}"{description}, draw=none, from=5-3, to=6-4]
	\arrow["{T\tau_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=1]
	\arrow["{T\tau \atop \simeq}"{description, pos=0.4}, Rightarrow, draw=none, from=4-3, to=2]
	\arrow["{T\mu_{q_i} \atop \simeq}", Rightarrow, draw=none, from=2, to=2-4]
	\arrow["{TT\sigma_i \atop \simeq}"{description, pos=0.4}, Rightarrow, draw=none, from=3-3, to=3]
	\arrow["{\rho_{A_i} \atop \simeq}"', draw=none, from=4, to=4-1]
\end{tikzcd}\]


But now recall that $Ts Tq^T_i \simeq TTq_i$ in each $i$: then one can glue the two copies of $T\mu_{A_i}$ in the diagram above to get rid of the complicated part in the middle: only remain the following diagram, and this ensures the coherence condition:









\begin{comment}
% https://q.uiver.app/?q=WzAsNyxbMiwwLCJUVEFfaSJdLFswLDAsIlRUVEFfaSJdLFswLDEsIlRUQV9pIl0sWzIsMSwiVEFfaSJdLFszLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMywyLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMSwyLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzEsMCwiVFRhX2kiXSxbMSwyLCJUXFxtdV97VEFfaX0iLDFdLFsyLDMsIlRhX2kiLDFdLFswLDMsIlRhX2kiLDJdLFswLDQsIlRxXlRfaSIsMV0sWzMsNSwiVHFfaSIsMV0sWzQsNSwiVGEiLDFdLFsyLDYsIlRxXlRfaSIsMV0sWzYsNSwiVGEiLDJdLFszLDYsIlRcXHRoZXRhX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNyw5LCJUXFxhbHBoYV5zX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTAsNCwiVFxcdGhldGFfaSBcXGF0b3AgXFxzaW1lcSIsMSx7ImxldmVsIjoxLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}
	{TTTA_i} && {TTA_i} \\
	{TTA_i} && {TA_i} & {T\underset{I}\oplaxbicolim \; TA_i} \\
	& {T\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; A_i}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{TTa_i}", from=1-1, to=1-3]
	\arrow["{T\mu_{TA_i}}"', from=1-1, to=2-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{Ta_i}"{description}, from=2-1, to=2-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{Ta_i}"', from=1-3, to=2-3]
	\arrow["{Tq^T_i}"{description}, from=1-3, to=2-4]
	\arrow["{Tq_i}"{description}, from=2-3, to=3-4]
	\arrow["Ta", from=2-4, to=3-4]
	\arrow["{Tq^T_i}"{description}, from=2-1, to=3-2]
	\arrow["Ta"', from=3-2, to=3-4]
	\arrow["{T\theta_i \atop \simeq}"{description}, draw=none, from=2-3, to=3-2]
	\arrow["{T\alpha^s_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=1]
	\arrow["{T\theta_i \atop \simeq}"{description}, draw=none, from=2, to=2-4]
\end{tikzcd}\]

% https://q.uiver.app/?q=WzAsNyxbMywyLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwwLCJUVEFfaSJdLFswLDAsIlRUVEFfaSJdLFszLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMSwxLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUVEFfaSJdLFsxLDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMCwxLCJUVEFfaSJdLFsyLDEsIlRUYV9pIl0sWzEsMywiVHFeVF9pIiwwLHsibGFiZWxfcG9zaXRpb24iOjcwfV0sWzMsMCwiVGEiLDFdLFsyLDQsIlRxXntUVH1faSIsMV0sWzQsMywiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVGFfaSIsMl0sWzEsNCwiVFxcdGhldGFeVF9pIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzUsMCwiVGEiLDJdLFs0LDUsIlxcc21hbGx7VFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgXFxtdV97QV9pfX0iLDEseyJsYWJlbF9wb3NpdGlvbiI6NjB9XSxbMyw1LCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBcXGFscGhhXnNfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyLDYsIlRcXG11X3tBX2l9IiwyXSxbNiw1LCJUcV5UX2kiLDJdLFsxNywxMCwiVFxcbXVfaSBcXGF0b3AgXFxzaW1lcSIsMCx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[=\begin{tikzcd}
	{TTTA_i} && {TTA_i} \\
	{TTA_i} & {T\underset{I}\oplaxbicolim \; TTA_i} && {T\underset{I}\oplaxbicolim \; TA_i} \\
	& {T\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; A_i}
	\arrow["{TTa_i}", from=1-1, to=1-3]
	\arrow["{Tq^T_i}"{pos=0.7}, from=1-3, to=2-4]
	\arrow["Ta", from=2-4, to=3-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Tq^{TT}_i}"{description}, from=1-1, to=2-2]
	\arrow["{T\underset{I}\oplaxbicolim \; Ta_i}"', from=2-2, to=2-4]
	\arrow["{T\theta^T_i \atop \simeq}"{description}, draw=none, from=1-3, to=2-2]
	\arrow["Ta"', from=3-2, to=3-4]
	\arrow["{\small{T\underset{I}\oplaxbicolim \; \mu_{A_i}}}"{description, pos=0.6}, from=2-2, to=3-2]
	\arrow["{T\underset{I}\oplaxbicolim \; \alpha^s_i \atop \simeq}"{description}, draw=none, from=2-4, to=3-2]
	\arrow["{T\mu_{A_i}}"', from=1-1, to=2-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{Tq^T_i}"', from=2-1, to=3-2]
	\arrow["{T\mu_i \atop \simeq}", Rightarrow, draw=none, from=1, to=0]
\end{tikzcd}\]









% https://q.uiver.app/?q=WzAsMTUsWzIsMCwiVFRBX2kiXSxbMCwwLCJUVFRBX2kiXSxbMCwyLCJUVEFfaSJdLFsxLDMsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMSwxLCJUVEFfaSJdLFsyLDEsIlRBX2kiXSxbMSwyLCJUQV9pIl0sWzIsNCwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFs0LDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsyLDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMiwzLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzAsNCwiVEFfaSJdLFs0LDAsIlRBX2kiXSxbNCw0LCJDIl0sWzEsMiwiXFxtdV97VEFfaX0iLDJdLFsxLDAsIlRUYV9pIl0sWzIsMywiVFRxX2kiLDFdLFsxLDQsIlRcXG11X3tUQV9pfSIsMV0sWzQsNSwiVGFfaSIsMV0sWzQsNiwiXFxtdV97QV9pfSIsMl0sWzAsNSwiVGFfaSIsMl0sWzIsNiwiXFxtdV97QV9pfSIsMV0sWzAsOCwiVHFeVF9pIiwxXSxbNSw5LCJUcV9pIiwxXSxbOCw5LCJUYSIsMV0sWzQsMTAsIlRxXlRfaSIsMV0sWzEwLDksIlRhIiwyXSxbNiw3LCJUcV9pIiwxLHsibGFiZWxfcG9zaXRpb24iOjIwfV0sWzUsMTAsIlRcXHRoZXRhX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMyw3LCJcXG11X3tBfSIsMV0sWzExLDcsIlxcbXVfe0F9Il0sWzEwLDExLCJUcyJdLFs0LDExLCJUVHFfaSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MH1dLFsyLDEyLCJcXG11X3tBX2l9IiwyXSxbMywxMiwiXFxtdV97cV9pfSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDEzLCJUYV9pIl0sWzksMTQsInAiXSxbNywxNCwicCIsMl0sWzE0LDEwLCJcXHhpIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEzLDksIlRxX2kiXSxbMTIsNywiVHFfaSIsMl0sWzE2LDE5LCJUXFxhbHBoYV5zX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiwxNSwiXFxyaG9fe3tBX2l9fSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDM2LCJUXFx0aGV0YV9pIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIxLDgsIlRcXHRoZXRhX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJsZXZlbCI6MSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMsMjIsIlxcbXVfe3FfaX0gXFxhdG9wIFxcc2ltZXEiLDIseyJsYWJlbF9wb3NpdGlvbiI6MzAsInNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszMywyOCwiXFxtdV97cV9pfSBcXGF0b3AgXFxzaW1lcSIsMix7ImxhYmVsX3Bvc2l0aW9uIjo0MCwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMzLDMyLCJUXFxzaWdtYV9pIFxcYXRvcCBcXHNpbWVxIiwxLHsibGFiZWxfcG9zaXRpb24iOjYwLCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}
	{TTTA_i} && {TTA_i} && {TA_i} \\
	& {TTA_i} & {TA_i} & {T\underset{I}\oplaxbicolim \; TA_i} \\
	{TTA_i} & {TA_i} & {T\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; A_i} \\
	& {TT\underset{I}\oplaxbicolim \; A_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	{TA_i} && {T\underset{I}\oplaxbicolim \; A_i} && C
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\mu_{TA_i}}"', from=1-1, to=3-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{TTa_i}", from=1-1, to=1-3]
	\arrow["{TTq_i}"{description}, from=3-1, to=4-2]
	\arrow["{T\mu_{TA_i}}"{description}, from=1-1, to=2-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{Ta_i}"{description}, from=2-2, to=2-3]
	\arrow["{\mu_{A_i}}"', from=2-2, to=3-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{Ta_i}"', from=1-3, to=2-3]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{\mu_{A_i}}"{description}, from=3-1, to=3-2]
	\arrow["{Tq^T_i}"{description}, from=1-3, to=2-4]
	\arrow["{Tq_i}"{description}, from=2-3, to=3-5]
	\arrow["Ta"{description}, from=2-4, to=3-5]
	\arrow["{Tq^T_i}"{description}, from=2-2, to=3-3]
	\arrow["Ta"', from=3-3, to=3-5]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{Tq_i}"{description, pos=0.2}, from=3-2, to=5-3]
	\arrow["{T\theta_i \atop \simeq}"{description}, draw=none, from=2-3, to=3-3]
	\arrow["{\mu_{A}}"{description}, from=4-2, to=5-3]
	\arrow["{\mu_{A}}", from=4-3, to=5-3]
	\arrow[""{name=6, anchor=center, inner sep=0}, "Ts", from=3-3, to=4-3]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{TTq_i}"{description, pos=0.4}, from=2-2, to=4-3]
	\arrow["{\mu_{A_i}}"', from=3-1, to=5-1]
	\arrow["{\mu_{q_i} \atop \simeq}"{description}, draw=none, from=4-2, to=5-1]
	\arrow[""{name=8, anchor=center, inner sep=0}, "{Ta_i}", from=1-3, to=1-5]
	\arrow["p", from=3-5, to=5-5]
	\arrow["p"', from=5-3, to=5-5]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=5-5, to=3-3]
	\arrow["{Tq_i}", from=1-5, to=3-5]
	\arrow["{Tq_i}"', from=5-1, to=5-3]
	\arrow["{T\alpha^s_i \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=2]
	\arrow["{\rho_{{A_i}} \atop \simeq}"{description}, Rightarrow, draw=none, from=3-2, to=0]
	\arrow["{T\theta_i \atop \simeq}"{description}, Rightarrow, draw=none, from=2-4, to=8]
	\arrow["{T\theta_i \atop \simeq}"{description}, draw=none, from=3, to=2-4]
	\arrow["{\mu_{q_i} \atop \simeq}"'{pos=0.3}, Rightarrow, draw=none, from=4-2, to=4]
	\arrow["{\mu_{q_i} \atop \simeq}"'{pos=0.4}, Rightarrow, draw=none, from=7, to=5]
	\arrow["{T\sigma_i \atop \simeq}"{description, pos=0.6}, Rightarrow, draw=none, from=7, to=6]
\end{tikzcd}\]

\end{comment}

% https://q.uiver.app/?q=WzAsMTEsWzEsMSwiVFRBX2kiXSxbMiwyLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzIsMywiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsyLDQsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDQsIkMiXSxbMywwLCJUQV9pIl0sWzAsNCwiVEFfaSJdLFsxLDAsIlRUQV9pIl0sWzAsMCwiVFRUQV9pIl0sWzAsMiwiVFRBX2kiXSxbMCwxLCJUcV5UX2kiLDFdLFsxLDIsIlRzIiwxXSxbMiwzLCJcXG11X0EiXSxbMSw0LCJUYSIsMl0sWzQsNSwicCJdLFszLDUsInAiLDJdLFswLDYsIlRhX2kiLDFdLFs2LDQsIlRxX2kiXSxbMCw3LCJcXG11X3tBX2l9IiwxLHsibGFiZWxfcG9zaXRpb24iOjcwfV0sWzcsMywiVHFfaSIsMl0sWzAsMiwiVFRxX2kiLDEseyJjdXJ2ZSI6Mn1dLFs2LDEsIlRcXHRoZXRhX2kgXFxhdG9wXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDYsIlRhX2kiXSxbOSwwLCJUXFxtdV97QV9pfSIsMV0sWzksMTAsIlxcbXVfe1RBX2l9IiwyXSxbMTAsNywiXFxtdV97QV9pfSIsMl0sWzksOCwiVFRhX2kiXSxbOCwwLCJUXFxhbHBoYV9pXnQgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTAsMCwiXFxtdV97XFxtdV97QV9pfX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTIsNSwiXFxjaGkgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMjEsNywiXFxtdV97cV9pfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMSwyLCJUXFxzaWdtYV9pIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}[sep=large]
	{TTTA_i} & {TTA_i} && {TA_i} \\
	& {TTA_i} \\
	{TTA_i} && {T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	&& {TT\underset{I}\oplaxbicolim \; A_i} \\
	{TA_i} && {T\underset{I}\oplaxbicolim \; A_i} & C
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Tq^T_i}"{description}, from=2-2, to=3-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Ts"{description}, from=3-3, to=4-3]
	\arrow["{\mu_A}", from=4-3, to=5-3]
	\arrow["Ta"', from=3-3, to=3-4]
	\arrow["p", from=3-4, to=5-4]
	\arrow["p"', from=5-3, to=5-4]
	\arrow["{Ta_i}"{description}, from=2-2, to=1-4]
	\arrow["{Tq_i}", from=1-4, to=3-4]
	\arrow["{\mu_{A_i}}"{description, pos=0.7}, from=2-2, to=5-1]
	\arrow["{Tq_i}"', from=5-1, to=5-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{TTq_i}"{description}, curve={height=12pt}, from=2-2, to=4-3]
	\arrow["{T\theta_i \atop\simeq}"{description}, draw=none, from=1-4, to=3-3]
	\arrow["{Ta_i}", from=1-2, to=1-4]
	\arrow["{T\mu_{A_i}}"{description}, from=1-1, to=2-2]
	\arrow["{\mu_{TA_i}}"', from=1-1, to=3-1]
	\arrow["{\mu_{A_i}}"', from=3-1, to=5-1]
	\arrow["{TTa_i}", from=1-1, to=1-2]
	\arrow["{T\alpha_i^t \atop \simeq}"{description}, draw=none, from=1-2, to=2-2]
	\arrow["{\mu_{\mu_{A_i}} \atop \simeq}"{description}, draw=none, from=3-1, to=2-2]
	\arrow["{\xi \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=5-4]
	\arrow["{\mu_{q_i} \atop \simeq}"{description}, Rightarrow, draw=none, from=2, to=5-1]
	\arrow["{T\sigma_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=4-3]
\end{tikzcd}\]

This achieves to prove that each $ pTq_i$ pseudocoequalizes the codescent diagram $U_T\mathscr{X}_{(A_i, a_i, (\alpha^t_i, \alpha_i^s))}$. \\

We must now prove that this property lifts to the overlying pseudo-algebraic structure: but this is a consequence of the fact that all the 2-cells involved above are transformations of pseudomorphisms between underlying 1-cells of pseudomorphisms, either by definition or by pseudonaturality. We left to careful reader the task to check this property.
\end{proof}




























This pseudomorphisms inserts in particular by the universal property of bicoequalizers an invertible transformation of pseudomorphisms $\xi$ as below
% https://q.uiver.app/?q=WzAsNyxbMCwxLCJUVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMSwyLCJUVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsyLDEsIlRDIl0sWzAsMiwiVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMSwwLCJUVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsxLDMsIlQgXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwyLCJDIl0sWzAsMSwiVFxcbXVfQVQocykiLDFdLFsxLDIsIlRwIiwxXSxbMCwzLCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2l9IiwyXSxbMCw0LCJUKGEpIl0sWzQsMiwiVHAiXSxbMyw1LCJcXG11X0FUKHMpIiwyXSxbNSw2LCJwIiwyXSxbMiw2LCJjIl0sWzEsNSwiXFxtdV9BIiwyXSxbNCwxLCJcXGNoaSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxLDMsIlxccmhvX0FcXG11X3MgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMSw2LCJcXHBpIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	& {TT \underset{I}\oplaxbicolim \; A_i} \\
	{TT \underset{I}\oplaxbicolim \; TA_i} && TC \\
	{T \underset{I}\oplaxbicolim \; TA_i} & {TT \underset{I}\oplaxbicolim \; A_i} & C \\
	& {T \underset{I}\oplaxbicolim \; A_i}
	\arrow["{T\mu_ATTs}"{description}, from=2-1, to=3-2]
	\arrow["Tp"{description}, from=3-2, to=2-3]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"', from=2-1, to=3-1]
	\arrow["{TT\underset{I}\oplaxbicolim \; a_i}", from=2-1, to=1-2]
	\arrow["Tp", from=1-2, to=2-3]
	\arrow["{\mu_ATs}"', from=3-1, to=4-2]
	\arrow["p"', from=4-2, to=3-3]
	\arrow["c", from=2-3, to=3-3]
	\arrow["{\mu_A}"', from=3-2, to=4-2]
	\arrow["{T\xi \atop \simeq}"{description}, draw=none, from=1-2, to=3-2]
	\arrow["{\rho_A\mu_s \atop \simeq}"{description}, draw=none, from=3-2, to=3-1]
	\arrow["{\pi \atop \simeq}"{description}, draw=none, from=3-2, to=3-3]
\end{tikzcd}\]% https://q.uiver.app/?q=WzAsNyxbMCwxLCJUVCBcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMiwxLCJUQyJdLFswLDIsIlQgXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzEsMCwiVFQgXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMSwzLCJUIFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzIsMiwiQyJdLFsxLDEsIlQgXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMCwyLCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2l9IiwyXSxbMCwzLCJUVChhKSJdLFszLDEsIlRwIl0sWzIsNCwiXFxtdV9BVChzKSIsMl0sWzQsNSwicCIsMl0sWzEsNSwiYyJdLFsyLDYsIlQoYSkiLDFdLFs2LDUsInAiLDFdLFszLDYsIlxcbXVfQSIsMV0sWzYsNCwiXFxjaGkgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOSwxNCwiXFxwaSBcXGF0b3AgXFxzaW1lcSIsMCx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDEzLCJcXG11X2EgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[=\begin{tikzcd}
	& {TT \underset{I}\oplaxbicolim \; A_i} \\
	{TT \underset{I}\oplaxbicolim \; TA_i} & {T \underset{I}\oplaxbicolim \; A_i} & TC \\
	{T \underset{I}\oplaxbicolim \; TA_i} && C \\
	& {T \underset{I}\oplaxbicolim \; A_i}
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"', from=2-1, to=3-1]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{TT\underset{I}\oplaxbicolim \; a_i}", from=2-1, to=1-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Tp", from=1-2, to=2-3]
	\arrow["{\mu_ATs}"', from=3-1, to=4-2]
	\arrow["p"', from=4-2, to=3-3]
	\arrow["c", from=2-3, to=3-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{T\underset{I}\oplaxbicolim \; a_i}"{description}, from=3-1, to=2-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, "p"{description}, from=2-2, to=3-3]
	\arrow["{\mu_A}"{description}, from=1-2, to=2-2]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=2-2, to=4-2]
	\arrow["{\pi \atop \simeq}", Rightarrow, draw=none, from=1, to=3]
	\arrow["{\mu_a \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=2]
\end{tikzcd}\]





==> cut.tex <==
Now we turn to the higher coherence data. We claim they are obtained as the following:\begin{itemize}
    \item the multiplication % https://q.uiver.app/?q=WzAsMixbMCwwLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IFRBX2kiXSxbMiwwLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgVEFfaSJdLFswLDEsIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IFRBX2l9Il1d
\[\begin{tikzcd}
	{TT\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; TA_i}
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}", from=1-1, to=1-3]
\end{tikzcd}\]
%which we will denote as  as if $A$ denoted $ \oplaxbicolim_I A_i$ for concision;
\item the composite 
% https://q.uiver.app/?q=WzAsNCxbMiwwLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaSJdLFsyLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGNvbGltIFxcOyBBX2kiXSxbMCwwLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IFRBX2kiXSxbNCwxLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgVEFfaSJdLFswLDEsIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaX0iLDJdLFsyLDAsIlRUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IGFfaSkiXSxbMSwzLCJUKFxcZXRhX3tcXHVuZGVyc2V0e2l9e1xcb3BsYXhiaWNvbGltfSBBX2l9KSJdXQ==
\[\begin{tikzcd}
	{TT\underset{I}\oplaxbicolim \; TA_i} && {TT\underset{I}\oplaxbicolim \; A_i} \\
	&& {T\underset{I}\oplaxbicolim \; A_i} && {T\underset{I}\oplaxbicolim \; TA_i}
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; A_i}}"', from=1-3, to=2-3]
	\arrow["{TT(\underset{I}\oplaxbicolim \; a_i)}", from=1-1, to=1-3]
	\arrow["{T(\underset{i}{\oplaxbicolim} \;\eta_{ A_i})}", from=2-3, to=2-5]
\end{tikzcd}\]
We will denote in an abbreviated way this map as $T(H) \mu_A TT(a)$ for concision, as if $ a$ denoted $ \oplaxbicolim_I a_i$ and $ H$ denoted $ \oplaxbicolim_I \eta_{A_i}$;
\item and for the last 1-cell, observe that the natural modification $\rho$ provided in the data of the pseudomonad gives at $\oplaxbicolim_I A_i$ an invertible 2-cell
% https://q.uiver.app/?q=WzAsNCxbMiwwLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaSJdLFsyLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGNvbGltIFxcOyBBX2kiXSxbMCwwLCJUVFRcXHVuZGVyc2V0e0l9XFxvcGxheGNvbGltIFxcOyBBX2kiXSxbMCwxLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaSJdLFswLDEsIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaX0iXSxbMiwwLCJcXG11X3tUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaSl9Il0sWzIsMywiVFxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaX0iLDJdLFszLDEsIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaX0iLDJdLFsyLDEsIlxccmhvX3tcXHVuZGVyc2V0e0l9XFxvcGxheGNvbGltIFxcOyBBX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{TTT\underset{I}\oplaxbicolim \; A_i} && {TT\underset{I}\oplaxbicolim \; A_i} \\
	{TT\underset{I}\oplaxbicolim \; A_i} && {T\underset{I}\oplaxbicolim \; A_i}
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; A_i}}", from=1-3, to=2-3]
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; A_i)}}", from=1-1, to=1-3]
	\arrow["{T\mu_{\underset{I}\oplaxbicolim \; A_i}}"', from=1-1, to=2-1]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; A_i}}"', from=2-1, to=2-3]
	\arrow["{\rho_{\underset{I}\oplaxbicolim \; A_i} \atop \simeq}"{description}, draw=none, from=1-1, to=2-3]
\end{tikzcd}\]
Then one can take either one or the other side of the following whiskering
% https://q.uiver.app/?q=WzAsNixbMiwxLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaSJdLFsyLDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGNvbGltIFxcOyBBX2kiXSxbMCwxLCJUVFRcXHVuZGVyc2V0e0l9XFxvcGxheGNvbGltIFxcOyBBX2kiXSxbMCwyLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaSJdLFswLDAsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgVEFfaSJdLFsyLDMsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGNvbGltIFxcOyBUQV9pIl0sWzAsMSwiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgQV9pfSJdLFsyLDAsIlxcbXVfe1QoXFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgQV9pKX0iXSxbMiwzLCJUXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgQV9pfSIsMl0sWzMsMSwiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgQV9pfSIsMl0sWzIsMSwiXFxyaG9fe1xcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCwyLCJUVChzKSIsMl0sWzEsNSwiVChcXGV0YV97XFx1bmRlcnNldHtpfXtcXG9wbGF4Ymljb2xpbX0gQV9pfSkiXV0=
\[\begin{tikzcd}
	{TT\underset{I}\oplaxbicolim \; TA_i} \\
	{TTT\underset{I}\oplaxbicolim \; A_i} && {TT\underset{I}\oplaxbicolim \; A_i} \\
	{TT\underset{I}\oplaxbicolim \; A_i} && {T\underset{I}\oplaxbicolim \; A_i} \\
	&& {T\underset{I}\oplaxbicolim \; TA_i}
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; A_i}}", from=2-3, to=3-3]
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; A_i)}}", from=2-1, to=2-3]
	\arrow["{T\mu_{\underset{I}\oplaxbicolim \; A_i}}"', from=2-1, to=3-1]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; A_i}}"', from=3-1, to=3-3]
	\arrow["{\rho_{\underset{I}\oplaxbicolim \; A_i} \atop \simeq}"{description}, draw=none, from=2-1, to=3-3]
	\arrow["{TT(s)}"', from=1-1, to=2-1]
	\arrow["{T(\underset{i}{\oplaxbicolim}\; \eta_{ A_i})}", from=3-3, to=4-3]
\end{tikzcd}\]
which we will denote as $T(H) \mu_A \mu_{T(A)} TT(s)$
\end{itemize}

\textcolor{red}{$\oplaxbicolim a_i $ and $s$  nor their $T$-power are comparable: $\oplaxbicolim a_i $ is constructed from the pseudo-algebras structures while $s$ depends on the $q_i$ and hence from the underlying oplax cocone made of the $A_i $ and the transition morphisms with are not dependant on the $a_i$ - though related by the $\phi_d$, but those data are merged in the oplax bicolimit. }




% https://q.uiver.app/?q=WzAsMyxbMCwwLCJUVChcXHVuZGVyc2V0e0l9XFxvcGxheGNvbGltIFxcOyBUQV9pKSJdLFszLDAsIlQoXFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgVEFfaSkiXSxbNSwwLCJUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaSkiXSxbMCwxLCJcXHRpbnl7XFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgQV9pfSBUKFxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IFRBX2l9KSBUVChzKX0iXSxbMCwxLCJUVChcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IGFfaSkiLDAseyJvZmZzZXQiOi0zLCJjdXJ2ZSI6LTN9XSxbMCwxLCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGNvbGltIFxcOyBUQV9pfSIsMix7Im9mZnNldCI6MywiY3VydmUiOjN9XSxbMiwxLCJcXHNtYWxse1QoXFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgXFxldGFfe0FfaX0pfSIsMl0sWzEsMiwiXFxzbWFsbHtUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IGFfe2l9KX0iLDAseyJvZmZzZXQiOi0yLCJjdXJ2ZSI6LTN9XSxbMSwyLCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGNvbGltIFxcOyBBX2l9VChzKSIsMix7Im9mZnNldCI6MiwiY3VydmUiOjN9XV0=
% https://q.uiver.app/?q=WzAsMyxbMCwwLCJUVChcXHVuZGVyc2V0e0l9XFxvcGxheGNvbGltIFxcOyBUQV9pKSJdLFszLDAsIlQoXFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgVEFfaSkiXSxbNSwwLCJUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Y29saW0gXFw7IEFfaSkiXSxbMCwxLCJUKFxcdW5kZXJzZXR7aX17XFxvcGxheGJpY29saW19IFxcO1xcZXRhX3sgQV9pfSkgXFxtdV9BIFRUKGEpIiwxXSxbMCwxLCJUKFxcdW5kZXJzZXR7aX17XFxvcGxheGJpY29saW19IFxcO1xcZXRhX3sgQV9pfSkgXFxtdV9BIFRcXG11X0EgVFQocykiLDAseyJvZmZzZXQiOi01fV0sWzAsMSwiXFxtdV97QX0iLDIseyJvZmZzZXQiOjV9XSxbMiwxLCJcXHNtYWxse1QoXFx1bmRlcnNldHtJfVxcb3BsYXhjb2xpbSBcXDsgXFxldGFfe0FfaX0pfSIsMV0sWzEsMiwiVChhKSIsMCx7Im9mZnNldCI6LTV9XSxbMSwyLCJcXG11X3tBfVQocykiLDIseyJvZmZzZXQiOjV9XV0=

\[\begin{tikzcd}
	{TT(\underset{I}\oplaxbicolim \; TA_i)} &&& {T(\underset{I}\oplaxbicolim \; TA_i)} && {T(\underset{I}\oplaxbicolim \; A_i)}
	\arrow["{T(H) \mu_A TT(a)}"{description}, from=1-1, to=1-4]
	\arrow["{T(H) \mu_A \mu_{T(A)} TT(s)}", shift left=5, from=1-1, to=1-4]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"', shift right=5, from=1-1, to=1-4]
	\arrow["{\small{T(H)}}"{description}, from=1-6, to=1-4]
	\arrow["{T(a)}", shift left=5, from=1-4, to=1-6]
	\arrow["{\mu_{A}T(s)}"', shift right=5, from=1-4, to=1-6]
\end{tikzcd}\]
\textcolor{red}{At least one of the higher data is false !}\\

\textcolor{red}{Also : ending a higher data with $T(H)$ should not work because $T(H)$ is already the identity of the codescent diagra, so those arrows above are killing the higher data contained in the third object by forming identities over one of their object. }




We already showed that the right data satisfied the pseudo-sections conditions of the lower data of a codescent object at \cref{coherence data oplax bicolim : lower data}. It remains to show the higher conditions, which amount to inserting invertible 2-cells with the successive composite of the lower and higher data. \\

A first such cell can be obtained as the following pasting:
% https://q.uiver.app/?q=WzAsNyxbMCwwLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFswLDEsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwwLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzAsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzAsMywiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFsxLDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsyLDMsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDEsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBhX2kiLDJdLFswLDIsIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaX0iXSxbMSwzLCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaX0iLDJdLFszLDQsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFxcZXRhX3tBX2l9IiwyXSxbMSw1LCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaX0iXSxbMiw1LCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBhX2kiLDFdLFsyLDYsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBhX2kiXSxbNSw2LCIiLDEseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDYsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBhX2kiLDJdLFszLDYsIiIsMCx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE2LDQsIlRcXG92ZXJsaW5le1xcYWxwaGFec30gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTQsMTYsIj0iLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMTQsIj0iLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCwxMSwiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBhX2kgXFxhdG9wIFxcc2ltZXF9IiwxLHsibGV2ZWwiOjEsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}[row sep=large]
	{TT\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; TA_i} \\
	{TT\underset{I}\oplaxbicolim \; A_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	{T\underset{I}\oplaxbicolim \; A_i} \\
	{T\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; A_i}
	\arrow["{TT\underset{I}\oplaxbicolim \; a_i}"', from=1-1, to=2-1]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\mu_{\underset{I}\oplaxbicolim \; TA_i}}", from=1-1, to=1-3]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; A_i}}"', from=2-1, to=3-1]
	\arrow["{T\underset{I}\oplaxbicolim \; \eta_{A_i}}"', from=3-1, to=4-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\mu_{\underset{I}\oplaxbicolim \; A_i}}", from=2-1, to=2-2]
	\arrow["{T\underset{I}\oplaxbicolim \; a_i}"{description}, from=1-3, to=2-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{T\underset{I}\oplaxbicolim \; a_i}", from=1-3, to=4-3]
	\arrow[""{name=3, anchor=center, inner sep=0}, Rightarrow, no head, from=2-2, to=4-3]
	\arrow["{T\underset{I}\oplaxbicolim \; a_i}"', from=4-1, to=4-3]
	\arrow[""{name=4, anchor=center, inner sep=0}, Rightarrow, no head, from=3-1, to=4-3]
	\arrow["{T\overline{\alpha^s} \atop \simeq}"{description}, Rightarrow, draw=none, from=4, to=4-1]
	\arrow["{=}"{description}, Rightarrow, draw=none, from=3, to=4]
	\arrow["{=}"{description}, Rightarrow, draw=none, from=2, to=3]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; a_i \atop \simeq}}"{description}, draw=none, from=0, to=1]
\end{tikzcd}\]

Then consider following pasting:
% https://q.uiver.app/?q=WzAsOCxbMCwwLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFs0LDAsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMCwyLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzQsMiwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzIsMCwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFszLDAsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsxLDAsIlRUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzIsMiwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsxLDMsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IGFfaSJdLFs0LDUsIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pfSJdLFs2LDQsIlRcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaX0iXSxbMCw2LCJUVHMiXSxbNSwxLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBcXGV0YV97QV9pfSJdLFs3LDMsIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pfSIsMl0sWzIsNywiVHMiLDJdLFs1LDMsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMiwiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9IiwyXSxbNCw3LCIiLDEseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxLDE1LCJUXFxvdmVybGluZXtcXGFscGhhfV5zIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzUsMTMsIj0iLDIseyJsZXZlbCI6MSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsMTQsIlxcbXVfcyBcXGF0b3AgXFxzaW1lcSIsMix7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
% https://q.uiver.app/?q=WzAsOCxbMCwwLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFswLDQsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMSwwLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzEsNCwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzAsMiwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDMsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDEsIlRUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzEsMiwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsxLDMsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IGFfaSIsMl0sWzQsNSwiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9IiwyXSxbNiw0LCJUXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9IiwyXSxbMCw2LCJUVHMiLDJdLFs1LDEsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFxcZXRhX3tBX2l9IiwyXSxbNywzLCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaX0iXSxbMiw3LCJUcyJdLFs1LDMsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMiwiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pfSJdLFs0LDcsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzUsMTMsIj0iLDIseyJsZXZlbCI6MSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsMTQsIlxcbXVfcyBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDUsIlRcXG92ZXJsaW5le1xcYWxwaGF9XnMgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}
	{TT\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; TA_i} \\
	{TTT\underset{I}\oplaxbicolim \; A_i} \\
	{TT\underset{I}\oplaxbicolim \; A_i} & {TT\underset{I}\oplaxbicolim \; A_i} \\
	{T\underset{I}\oplaxbicolim \; A_i} \\
	{T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{T\underset{I}\oplaxbicolim \; a_i}"', from=5-1, to=5-2]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; A_i}}"', from=3-1, to=4-1]
	\arrow["{T\mu_{\underset{I}\oplaxbicolim \; A_i}}"', from=2-1, to=3-1]
	\arrow["TTs"', from=1-1, to=2-1]
	\arrow["{T\underset{I}\oplaxbicolim \; \eta_{A_i}}"', from=4-1, to=5-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\mu_{\underset{I}\oplaxbicolim \; A_i}}", from=3-2, to=5-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, "Ts", from=1-2, to=3-2]
	\arrow[Rightarrow, no head, from=4-1, to=5-2]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}", from=1-1, to=1-2]
	\arrow[Rightarrow, no head, from=3-1, to=3-2]
	\arrow["{=}"', draw=none, from=4-1, to=1]
	\arrow["{\mu_s \atop \simeq}"{description}, Rightarrow, draw=none, from=2-1, to=2]
	\arrow["{T\overline{\alpha}^s \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=4-1]
\end{tikzcd}\]
\textcolor{red}{There is a problem !}


% https://q.uiver.app/?q=WzAsMTAsWzAsMCwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMCwxLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsMCwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFswLDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDMsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbNCwzLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwwLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzMsMCwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzEsMCwiVFRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwzLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzAsMSwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IGFfaSIsMl0sWzEsMywiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9IiwyXSxbMyw0LCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBcXGV0YV97QV9pfSIsMl0sWzIsNSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgYV9pIl0sWzYsNywiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9Il0sWzgsNiwiVFxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pfSJdLFswLDgsIlRUcyJdLFs3LDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFxcZXRhX3tBX2l9Il0sWzksNSwiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9IiwyXSxbNCw5LCJUcyIsMl0sWzMsOSwiVFxcZXRhX3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaX0iLDFdLFs3LDUsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMsNSwiIiwxLHsiY3VydmUiOi0yLCJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszLDcsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIwLDQsIlxcbGFuZ2xlIFxcZXRhX3txX2l9XFxzaWdtYV9pIFxccmFuZ2xlX3tpIFxcaW4gSX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiwyMSwiVFxcb3ZlcmxpbmV7XFxhbHBoYX1ecyBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs5LDIyLCJUXFxvdmVybGluZXtcXHpldGF9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIyLDcsIj0iLDIseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=




Now the codescent object above can be lifted to a codescent object in the 2-category of pseudo-algebras: we can guess already that its 0-cells will be the free pseudo-algebra structure on the underlying object; similarly its 1-cells can be equipped with a structure of pseudomorphism by pasting sequences of naturality squares associated to the multiplication:\begin{itemize}

    \item for the multiplication $ \mu_A$, just take the naturality 2-cell of the natural modification $\rho$:
    % https://q.uiver.app/?q=WzAsNCxbMCwwLCJUVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMCwxLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFsyLDAsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzIsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFswLDEsIlxcbXVfe1QoXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pKX0iLDJdLFswLDIsIlQoXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pfSkiXSxbMiwzLCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2l9Il0sWzEsMywiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pfSIsMl0sWzUsNywiXFxyaG9fIHtcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2l9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{TTT\underset{I}\oplaxbicolim \; TA_i} && {TT\underset{I}\oplaxbicolim \; TA_i} \\
	{TT\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; TA_i}
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; TA_i)}}"', from=1-1, to=2-1]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{T(\mu_{\underset{I}\oplaxbicolim \; TA_i})}", from=1-1, to=1-3]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}", from=1-3, to=2-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"', from=2-1, to=2-3]
	\arrow["{\rho_ {\underset{I}\oplaxbicolim \; TA_i} \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=1]
\end{tikzcd}\]
\item for $ T(H)\mu_ATT(a)$ take the pasting we will denote as $ \mu_{T(H)}\rho_a \mu_{T(a)}$:
% https://q.uiver.app/?q=WzAsOCxbMCwwLCJUVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMCwxLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFs2LDAsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzYsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFsyLDAsIlRUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzQsMCwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsyLDEsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbNCwxLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMCwxLCJcXG11X3tUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSl9IiwyXSxbMiwzLCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2l9Il0sWzAsNCwiVFRUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgYV9pKSJdLFs0LDUsIlQoXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9KSJdLFs1LDIsIlRUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgXFxldGFfe0FfaX0pIl0sWzEsNiwiVFQoXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBhX2kpIiwyXSxbNiw3LCJcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaX0iLDJdLFs3LDMsIlQoXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBcXGV0YV97QV9pfSkiLDJdLFs1LDcsIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pfSIsMV0sWzQsNiwiXFxtdV97VChcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSl9IiwxXSxbMTIsMTUsIlxcbXVfe1QoXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBcXGV0YV97QV9pfSl9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEwLDEzLCJcXG11X3tUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgYV9pKX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTEsMTQsIlxccmhvX3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
% https://q.uiver.app/?q=WzAsOCxbMCwwLCJUVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMiwwLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFswLDMsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzIsMywiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFswLDEsIlRUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzAsMiwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsyLDEsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwyLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMCwxLCJcXG11X3tUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSl9Il0sWzIsMywiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pfSIsMl0sWzAsNCwiVFRUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgYV9pKSIsMl0sWzQsNSwiVChcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaX0pIiwyXSxbNSwyLCJUVChcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFxcZXRhX3tBX2l9KSIsMl0sWzEsNiwiVFQoXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBhX2kpIl0sWzYsNywiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9Il0sWzcsMywiVChcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFxcZXRhX3tBX2l9KSJdLFs1LDcsIlxcbXVfe1xcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pfSIsMV0sWzQsNiwiXFxtdV97VChcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSl9IiwxXSxbMTIsMTUsIlxcbXVfe1QoXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBcXGV0YV97QV9pfSl9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEwLDEzLCJcXG11X3tUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgYV9pKX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTEsMTQsIlxccmhvX3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}[column sep=large]
	{TTT\underset{I}\oplaxbicolim \; TA_i} && {TT\underset{I}\oplaxbicolim \; TA_i} \\
	{TTT\underset{I}\oplaxbicolim \; A_i} && {TT\underset{I}\oplaxbicolim \; A_i} \\
	{TT\underset{I}\oplaxbicolim \; A_i} && {T\underset{I}\oplaxbicolim \; A_i} \\
	{TT\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; TA_i}
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; TA_i)}}", from=1-1, to=1-3]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"', from=4-1, to=4-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{TTT(\underset{I}\oplaxbicolim \; a_i)}"', from=1-1, to=2-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{T(\mu_{\underset{I}\oplaxbicolim \; A_i})}"', from=2-1, to=3-1]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{TT(\underset{I}\oplaxbicolim \; \eta_{A_i})}"', from=3-1, to=4-1]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{TT(\underset{I}\oplaxbicolim \; a_i)}", from=1-3, to=2-3]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{\mu_{\underset{I}\oplaxbicolim \; A_i}}", from=2-3, to=3-3]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{T(\underset{I}\oplaxbicolim \; \eta_{A_i})}", from=3-3, to=4-3]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; A_i}}"{description}, from=3-1, to=3-3]
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; A_i)}}"{description}, from=2-1, to=2-3]
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; \eta_{A_i})} \atop \simeq}"{description}, Rightarrow, draw=none, from=2, to=5]
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; a_i)} \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=3]
	\arrow["{\rho_{\underset{I}\oplaxbicolim \; A_i} \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=4]
\end{tikzcd}\]
\item for $T(H)\mu_A \mu_T(A)TT(s)$ take the following pasting we will denote as $ \mu_{T(H)}\rho_a \rho_{T(a)} \mu_{T(a)}$
% https://q.uiver.app/?q=WzAsMTAsWzAsMCwiVFRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzIsMCwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMCw0LCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSJdLFsyLDQsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMCwxLCJUVFRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMCwzLCJUVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzIsMSwiVFRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMiwzLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMCwyLCJUVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsyLDIsIlRUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kiXSxbMCwxLCJcXG11X3tUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgVEFfaSl9Il0sWzIsMywiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pfSIsMl0sWzAsNCwiVFRUKHMpIiwyXSxbNSwyLCJUVChcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFxcZXRhX3tBX2l9KSIsMl0sWzEsNiwiVFQocykiXSxbNywzLCJUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgXFxldGFfe0FfaX0pIl0sWzUsNywiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9IiwxXSxbNCw2LCJcXG11X3tUVChcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSl9IiwxXSxbMCw2LCJcXG11X3tUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgYV9pKX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzQsOCwiVChcXG11X3tUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pKX0pIiwyXSxbNiw5LCJcXG11X3tUKFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pKX0iXSxbNCw5LCJcXHJob197VChcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSl9IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwibGV2ZWwiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDksIlxcbXVfe1QoXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2kpfSIsMV0sWzksNywiXFxtdV97XFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBBX2l9Il0sWzgsNSwiVChcXG11X3tcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSl9KSIsMV0sWzgsNywiXFxyaG9fe1xcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pfSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMywxNSwiXFxtdV97VChcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFxcZXRhX3tBX2l9KX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}[column sep=huge]
	{TTT\underset{I}\oplaxbicolim \; TA_i} && {TT\underset{I}\oplaxbicolim \; TA_i} \\
	{TTTT\underset{I}\oplaxbicolim \; A_i} && {TTT\underset{I}\oplaxbicolim \; A_i} \\
	{TTT\underset{I}\oplaxbicolim \; A_i} && {TT\underset{I}\oplaxbicolim \; A_i} \\
	{TT\underset{I}\oplaxbicolim \; A_i} && {T\underset{I}\oplaxbicolim \; A_i} \\
	{TT\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; TA_i}
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; TA_i)}}", from=1-1, to=1-3]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; TA_i}}"', from=5-1, to=5-3]
	\arrow["{TTT(s)}"', from=1-1, to=2-1]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{TT(\underset{I}\oplaxbicolim \; \eta_{A_i})}"', from=4-1, to=5-1]
	\arrow["{TT(s)}", from=1-3, to=2-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{T(\underset{I}\oplaxbicolim \; \eta_{A_i})}", from=4-3, to=5-3]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; A_i}}"{description}, from=4-1, to=4-3]
	\arrow["{\mu_{TT(\underset{I}\oplaxbicolim \; A_i)}}"{description}, from=2-1, to=2-3]
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; a_i)} \atop \simeq}"{description}, Rightarrow, draw=none, from=1-1, to=2-3]
	\arrow["{T(\mu_{T(\underset{I}\oplaxbicolim \; A_i)})}"', from=2-1, to=3-1]
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; A_i)}}", from=2-3, to=3-3]
	\arrow["{\rho_{T(\underset{I}\oplaxbicolim \; A_i)} \atop \simeq}"{description}, Rightarrow, draw=none, from=2-1, to=3-3]
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; A_i)}}"{description}, from=3-1, to=3-3]
	\arrow["{\mu_{\underset{I}\oplaxbicolim \; A_i}}", from=3-3, to=4-3]
	\arrow["{T(\mu_{\underset{I}\oplaxbicolim \; A_i)})}"{description}, from=3-1, to=4-1]
	\arrow["{\rho_{\underset{I}\oplaxbicolim \; A_i} \atop \simeq}"{description}, draw=none, from=3-1, to=4-3]
	\arrow["{\mu_{T(\underset{I}\oplaxbicolim \; \eta_{A_i})} \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=1]
\end{tikzcd}\]
\end{itemize}






We will says that a morphism $ q: \mathscr{X}(0) \rightarrow C$ \emph{pseudocoequalizes} $ \mathbb{X}$ if it inserts an invertible 2-cell 
% https://q.uiver.app/?q=WzAsNCxbMCwwLCJcXG1hdGhzY3J7WH0oMSkiXSxbMSwwLCJcXG1hdGhzY3J7WH0oMCkiXSxbMSwxLCJDIl0sWzAsMSwiXFxtYXRoc2Nye1h9KDApIl0sWzAsMSwiXFxtYXRoc2Nye1h9KGRfMCkiXSxbMSwyLCJxIl0sWzAsMywiXFxtYXRoc2Nye1h9KGRfMSkiLDJdLFszLDIsInEiLDJdLFswLDIsIlxceGkgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}
	{\mathscr{X}(1)} & {\mathscr{X}(0)} \\
	{\mathscr{X}(0)} & C
	\arrow["{\mathscr{X}(d_0)}", from=1-1, to=1-2]
	\arrow["q", from=1-2, to=2-2]
	\arrow["{\mathscr{X}(d_1)}"', from=1-1, to=2-1]
	\arrow["q"', from=2-1, to=2-2]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=1-1, to=2-2]
\end{tikzcd}\]
satisfying moreover the following identities
% https://q.uiver.app/?q=WzAsNyxbMSwxLCJcXG1hdGhzY3J7WH0oMSkiXSxbMywxLCJcXG1hdGhzY3J7WH0oMCkiXSxbMywzLCJDIl0sWzEsMywiXFxtYXRoc2Nye1h9KDApIl0sWzAsMCwiXFxtYXRoc2Nye1h9KDIpIl0sWzIsMCwiXFxtYXRoc2Nye1h9KDEpIl0sWzAsMiwiXFxtYXRoc2Nye1h9KDEpIl0sWzAsMSwiXFxtYXRoc2Nye1h9KGRfMCkiLDFdLFsxLDIsInEiXSxbMCwzLCJcXG1hdGhzY3J7WH0oZF8xKSIsMV0sWzMsMiwicSIsMl0sWzAsMiwiXFx4aSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDBdLFs0LDUsIlxcbWF0aHNjcntYfShwXzApIl0sWzUsMSwiXFxtYXRoc2Nye1h9KGRfMCkiXSxbNCw2LCJcXG1hdGhzY3J7WH0ocF8yKSIsMl0sWzYsMywiXFxtYXRoc2Nye1h9KGRfMSkiLDJdLFswLDUsIlxcbWF0aHNjcntYfShcXHRoZXRhX3swMX0pIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsMCwiXFxtYXRoc2Nye1h9KFxcdGhldGFfezAxfSkgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}
	{\mathscr{X}(2)} && {\mathscr{X}(1)} \\
	& {\mathscr{X}(1)} && {\mathscr{X}(0)} \\
	{\mathscr{X}(1)} \\
	& {\mathscr{X}(0)} && C
	\arrow["{\mathscr{X}(d_0)}"{description}, from=2-2, to=2-4]
	\arrow["q", from=2-4, to=4-4]
	\arrow["{\mathscr{X}(d_1)}"{description}, from=2-2, to=4-2]
	\arrow["q"', from=4-2, to=4-4]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=2-2, to=4-4]
	\arrow[from=1-1, to=2-2]
	\arrow["{\mathscr{X}(p_0)}", from=1-1, to=1-3]
	\arrow["{\mathscr{X}(d_0)}", from=1-3, to=2-4]
	\arrow["{\mathscr{X}(p_2)}"', from=1-1, to=3-1]
	\arrow["{\mathscr{X}(d_1)}"', from=3-1, to=4-2]
	\arrow["{\mathscr{X}(\theta_{01}) \atop \simeq}"{description}, draw=none, from=2-2, to=1-3]
	\arrow["{\mathscr{X}(\theta_{01}) \atop \simeq}"{description}, draw=none, from=3-1, to=2-2]
\end{tikzcd}\]
% https://q.uiver.app/?q=WzAsNyxbMywxLCJcXG1hdGhzY3J7WH0oMCkiXSxbMywzLCJDIl0sWzEsMywiXFxtYXRoc2Nye1h9KDApIl0sWzAsMCwiXFxtYXRoc2Nye1h9KDIpIl0sWzIsMCwiXFxtYXRoc2Nye1h9KDEpIl0sWzAsMiwiXFxtYXRoc2Nye1h9KDEpIl0sWzIsMiwiXFxtYXRoc2Nye1h9KDApIl0sWzAsMSwicSJdLFsyLDEsInEiLDJdLFszLDQsIlxcbWF0aHNjcntYfShwXzApIl0sWzQsMCwiXFxtYXRoc2Nye1h9KGRfMCkiXSxbMyw1LCJcXG1hdGhzY3J7WH0ocF8yKSIsMl0sWzUsMiwiXFxtYXRoc2Nye1h9KGRfMSkiLDJdLFs1LDYsIlxcbWF0aHNjcntYfShkXzEpIiwxXSxbNCw2LCJcXG1hdGhzY3J7WH0oZF8wKSIsMV0sWzYsMSwicSIsMV0sWzMsNiwiXFxtYXRoc2Nye1h9KFxcdGhldGFfezAyfSkgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiwyLCJcXHhpIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsMCwiXFx4aSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	{\mathscr{X}(2)} && {\mathscr{X}(1)} \\
	&&& {\mathscr{X}(0)} \\
	{\mathscr{X}(1)} && {\mathscr{X}(0)} \\
	& {\mathscr{X}(0)} && C
	\arrow["q", from=2-4, to=4-4]
	\arrow["q"', from=4-2, to=4-4]
	\arrow["{\mathscr{X}(p_0)}", from=1-1, to=1-3]
	\arrow["{\mathscr{X}(d_0)}", from=1-3, to=2-4]
	\arrow["{\mathscr{X}(p_2)}"', from=1-1, to=3-1]
	\arrow["{\mathscr{X}(d_1)}"', from=3-1, to=4-2]
	\arrow["{\mathscr{X}(d_1)}"{description}, from=3-1, to=3-3]
	\arrow["{\mathscr{X}(d_0)}"{description}, from=1-3, to=3-3]
	\arrow["q"{description}, from=3-3, to=4-4]
	\arrow["{\mathscr{X}(\theta_{02}) \atop \simeq}"{description}, draw=none, from=1-1, to=3-3]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=3-3, to=4-2]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=3-3, to=2-4]
\end{tikzcd}\]
%Now take the weight $ \mathscr{J} : \mathbb{T} \rightarrow \Cat$ sending $ 0$ on the one object category $ *$, $1$ on the walking isomorphism $ * \simeq *$ and $ 2$ on the walking composable isomorphisms $ * \simeq * \simeq*$. A $\mathscr{J}$-weighted pseudocone \emph{pseudocoequalizes} a codescent object if it inserts a 2-cell $ \alpha $


A \emph{bicoequalizer} of a codescent object $ \mathscr{X}$ is the weighted bicolimit relative to the weight $ \mathscr{J} : \mathbb{X} \rightarrow \Cat$ sending 




\[\begin{tikzcd}[row sep=huge]
	{(T\underset{I}\oplaxcolim \; TTA_i, \mu_{\underset{I}\oplaxbicolim \; TTA_i},(\xi_{\underset{I}\oplaxbicolim \; TTA_i}, \rho_{\underset{I}\oplaxbicolim \; TTA_i}))} \\
	\\
	{(T\underset{I}\oplaxcolim \; TA_i, \mu_{\underset{I}\oplaxbicolim \; TA_i}, (\xi_{\underset{I}\oplaxbicolim \; TA_i},\rho_{\underset{I}\oplaxbicolim \; TA_i}))} \\
	\\
	{(T\underset{I}\oplaxcolim \; A_i, \mu_{\underset{I}\oplaxbicolim \; A_i}, (\xi_{\underset{I}\oplaxbicolim \; A_i},\rho_{\underset{I}\oplaxbicolim \; A_i}))}
	\arrow["{(\mu_{\underset{I}\oplaxcolim \; TA_i} Tt, \mu_{\underset{I}\oplaxbicolim \; T{A_i}}* \mu_{Tt}\rho_{\underset{I}\oplaxbicolim \; T{A_i}}*TTt)}"{description}, from=1-1, to=3-1]
	\arrow["{(T\underset{I}\oplaxcolim \; Ta_i,\mu_{\underset{I}\oplaxbicolim \; Ta_i})}"{description, pos=0.8}, shift left=50, from=1-1, to=3-1]
	\arrow["{\small{(T\underset{I}\oplaxcolim \; \mu_{A_i}, \mu_{\underset{I}\oplaxbicolim \; \mu_{A_i})}}}"{description, pos=0.2}, shift right=50,  from=1-1, to=3-1]
	\arrow["{(T\underset{I}\oplaxcolim \; \eta_{A_i},\mu_{\underset{I}\oplaxbicolim \; \eta_{A_i}})}"{description}, from=5-1, to=3-1]
	\arrow["{(T\underset{I}\oplaxcolim \; a_i,\mu_{\underset{I}\oplaxbicolim \; a_i})}"{description, pos=0.8}, shift left=40, from=3-1, to=5-1]
	\arrow["{(\mu_{\underset{I}\oplaxcolim \; A_i}T(s),\mu_{\underset{I}\oplaxbicolim \; A_i}*\mu_s\rho_{\underset{I}\oplaxbicolim \; A_i}*TTs)}"{description, pos=0.2}, shift right=40,  from=3-1, to=5-1]
\end{tikzcd}\]














Very complicated from of lemma 4.12 and co







Then we have at each $d$ in $\Sigma$ the following sequence of decompositions
% https://q.uiver.app/?q=WzAsNCxbNCwxLCJDIl0sWzIsMSwiXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBGICJdLFswLDAsIkYoXFxkb20oZCkpIl0sWzAsMiwiRihcXGNvZChkKSkiXSxbMSwwLCJxIiwxXSxbMiwzLCJGKGQpIiwyXSxbMywxLCJxX3tcXGNvZChkKX0iLDJdLFsyLDEsInFfe1xcZG9tKGQpfSJdLFs2LDcsInFfZCIsMCx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XV0=
\[\begin{tikzcd}
	{F(\dom(d))} \\
	&& {\underset{I}\oplaxbicolim \; F } && C \\
	{F(\cod(d))}
	\arrow["q"{description}, from=2-3, to=2-5]
	\arrow["{F(d)}"', from=1-1, to=3-1]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{q_{\cod(d)}}"', from=3-1, to=2-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{q_{\dom(d)}}", from=1-1, to=2-3]
	\arrow["{q_d}", shorten <=5pt, shorten >=5pt, Rightarrow, from=0, to=1]
\end{tikzcd}\]
% https://q.uiver.app/?q=WzAsNixbNCwxLCJDIl0sWzAsMCwiRihcXGRvbShkKSkiXSxbMCwyLCJGKFxcY29kKGQpKSJdLFsxLDEsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltIFxcOyBGIFxcZG9tIl0sWzIsMCwiXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBGICJdLFsyLDIsIlxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgRiAiXSxbMSwyLCJGKGQpIiwyXSxbMSwzLCJxXjJfZCIsMV0sWzQsMCwicSJdLFsxLDQsInFfe1xcZG9tKGQpfSJdLFszLDQsIlxcbGFuZ2xlIHFfe1xcY29kKGQpfSBGKGQpIFxccmFuZ2xlX3tkIFxcaW4gSV4yfSIsMV0sWzQsNSwiIiwxLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSwwLCJxIiwyXSxbMiw1XSxbMyw5LCJxX2QiLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzgsMTIsIj0iLDIseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMywxMywiXFx0aGV0YSdfZCBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[ = \begin{tikzcd}
	{F(\dom(d))} && {\underset{I}\oplaxbicolim \; F } \\
	& {\underset{\Sigma^2}\oplaxbicolim \; F \dom} &&& C \\
	{F(\cod(d))} && {\underset{I}\oplaxbicolim \; F }
	\arrow["{F(d)}"', from=1-1, to=3-1]
	\arrow["{q^2_d}"{description}, from=1-1, to=2-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "q", from=1-3, to=2-5]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{q_{\dom(d)}}", from=1-1, to=1-3]
	\arrow["{\langle q_{\cod(d)} F(d) \rangle_{d \in I^2}}"{description}, from=2-2, to=1-3]
	\arrow[Rightarrow, no head, from=1-3, to=3-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "q"', from=3-3, to=2-5]
	\arrow["q_{\cod(d)}"', ""{name=3, anchor=center, inner sep=0}, from=3-1, to=3-3]
	\arrow["{q_d}", shorten <=3pt, shorten >=3pt, Rightarrow, from=2-2, to=1]
	\arrow["{=}"', Rightarrow, draw=none, from=0, to=2]
	\arrow["{\theta'_d \atop \simeq}"{description}, Rightarrow, draw=none, from=2-2, to=3]
\end{tikzcd}\]


% https://q.uiver.app/?q=WzAsNyxbNCwxLCJDIl0sWzAsMCwiRihcXGRvbShkKSkiXSxbMCwyLCJGKFxcY29kKGQpKSJdLFsxLDEsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltIFxcOyBGIFxcZG9tIl0sWzIsMCwiXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBGICJdLFsyLDIsIlxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgRiAiXSxbMSwwLCJcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbSBcXDsgRiBcXGRvbSJdLFsxLDIsIkYoZCkiLDJdLFsxLDMsInFeMl9kIiwxXSxbNCwwLCJxIl0sWzEsNCwicV97XFxkb20oZCl9IiwwLHsiY3VydmUiOi00fV0sWzQsNSwiIiwxLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSwwLCJxIiwyXSxbMiw1XSxbMSw2LCJxXjJfZCIsMV0sWzYsNCwiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gSV4yfSIsMl0sWzMsNiwicV9kIiwwLHsibGV2ZWwiOjJ9XSxbMyw1LCJcXGxhbmdsZSBxX3tcXGNvZChkKX0gRihkKSBcXHJhbmdsZV97ZCBcXGluIEleMn0iLDFdLFs5LDEyLCI9IiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMsMTMsIlxcdGhldGEnX2QgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTAsNiwiXFx0aGV0YV9kIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[ = \begin{tikzcd}
	{F(\dom(d))} & {\underset{\Sigma^2}\oplaxbicolim \; F \dom} & {\underset{I}\oplaxbicolim \; F } \\
	& {\underset{\Sigma^2}\oplaxbicolim \; F \dom} &&& C \\
	{F(\cod(d))} && {\underset{I}\oplaxbicolim \; F }
	\arrow["{F(d)}"', from=1-1, to=3-1]
	\arrow["{q^2_d}"{description}, from=1-1, to=2-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "q", from=1-3, to=2-5]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{q_{\dom(d)}}", curve={height=-24pt}, from=1-1, to=1-3]
	\arrow[Rightarrow, no head, from=1-3, to=3-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "q"', from=3-3, to=2-5]
	\arrow[""{name=3, anchor=center, inner sep=0}, from=3-1, to=3-3]
	\arrow["{q^2_d}"{description}, from=1-1, to=1-2]
	\arrow["{\langle q_{\dom(d)} \rangle_{d \in I^2}}"', from=1-2, to=1-3]
	\arrow["{q_d}", Rightarrow, from=2-2, to=1-2]
	\arrow["{\langle q_{\cod(d)} F(d) \rangle_{d \in I^2}}"{description}, from=2-2, to=3-3]
	\arrow["{=}"', Rightarrow, draw=none, from=0, to=2]
	\arrow["{\theta'_d \atop \simeq}"{description}, Rightarrow, draw=none, from=2-2, to=3]
	\arrow["{\theta_d \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=1-2]
\end{tikzcd}\]


% https://q.uiver.app/?q=WzAsNixbNCwxLCJDIl0sWzAsMCwiRihcXGRvbShkKSkiXSxbMCwyLCJGKFxcY29kKGQpKSJdLFsxLDEsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltIFxcOyBGIFxcZG9tIl0sWzIsMCwiXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBGICJdLFsyLDIsIlxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgRiAiXSxbMSwyLCJGKGQpIiwyXSxbMSwzLCJxXjJfZCIsMV0sWzQsMCwicSJdLFsxLDQsInFfe1xcZG9tKGQpfSJdLFs1LDAsInEiLDJdLFsyLDVdLFszLDUsIlxcbGFuZ2xlIHFfe1xcY29kKGQpfSBGKGQpIFxccmFuZ2xlX3tkIFxcaW4gSV4yfSIsMV0sWzMsNCwiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gSV4yfSIsMV0sWzQsNSwiXFx4aSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszLDExLCJcXHRoZXRhJ19kIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzksMywiXFx0aGV0YV9kIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[ = \begin{tikzcd}
	{F(\dom(d))} && {\underset{I}\oplaxbicolim \; F } \\
	& {\underset{\Sigma^2}\oplaxbicolim \; F \dom} &&& C \\
	{F(\cod(d))} && {\underset{I}\oplaxbicolim \; F }
	\arrow["{F(d)}"', from=1-1, to=3-1]
	\arrow["{q^2_d}"{description}, from=1-1, to=2-2]
	\arrow["q", from=1-3, to=2-5]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{q_{\dom(d)}}", from=1-1, to=1-3]
	\arrow["q"', from=3-3, to=2-5]
	\arrow[""{name=1, anchor=center, inner sep=0}, from=3-1, to=3-3]
	\arrow["{\langle q_{\cod(d)} F(d) \rangle_{d \in I^2}}"{description}, from=2-2, to=3-3]
	\arrow["{\langle q_{\dom(d)} \rangle_{d \in I^2}}"{description}, from=2-2, to=1-3]
	\arrow["{\xi \atop \simeq}"{description}, draw=none, from=1-3, to=3-3]
	\arrow["{\theta'_d \atop \simeq}"{description}, Rightarrow, draw=none, from=2-2, to=1]
	\arrow["{\theta_d \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=2-2]
\end{tikzcd}\]
(where $ \theta_d$, $\theta_d'$ are the universal invertible 2-cells provided at the oplax cocone of \cref{Codescent data associated to a bicolimit: 1-dimensional data})

\textcolor{red}{Where the last move is due to ???????}\\
\textcolor{red}{also the condition on identity i had forgotten !}
\textcolor{red}{Compatibility conditions ? }\\











\begin{lemma}
The composite $ p_0\eta_C$ pseudocoequalizes the codescent diagram $ U_T\mathscr{X}$. 
\end{lemma}

\begin{proof}

We must first exhibit an invertible 2-cell $ \xi_0$ inserted by $ p_0\eta_C$. This can be chosen as the following pasting:
% https://q.uiver.app/?q=WzAsNyxbMCwyLCJDIl0sWzIsMCwiQyJdLFsxLDIsIlRDIl0sWzIsMiwiUF8wIl0sWzIsMSwiVEMiXSxbMCwwLCJCIl0sWzEsMSwiVEIiXSxbMCwyLCJcXGV0YV9DIiwyXSxbMSw0LCJcXGV0YV9DIl0sWzQsMywicF8wIl0sWzUsMCwidCIsMl0sWzUsMSwicyJdLFsyLDMsInBfMCIsMl0sWzUsNiwiXFxldGFfQiIsMV0sWzYsMiwiVHQiLDFdLFs2LDQsIlRzIiwxXSxbNiwzLCJcXHhpXzBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMSwxNSwiXFxldGFfcyBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMCwxNCwiXFxldGFfdCBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	B && C \\
	& TB & TC \\
	C & TC & {P_0}
	\arrow["{\eta_C}"', from=3-1, to=3-2]
	\arrow["{\eta_C}", from=1-3, to=2-3]
	\arrow["{p_0}", from=2-3, to=3-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "t"', from=1-1, to=3-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "s", from=1-1, to=1-3]
	\arrow["{p_0}"', from=3-2, to=3-3]
	\arrow["{\eta_B}"{description}, from=1-1, to=2-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, "Tt"{description}, from=2-2, to=3-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, "Ts"{description}, from=2-2, to=2-3]
	\arrow["{\xi_0\atop \simeq}"{description}, draw=none, from=2-2, to=3-3]
	\arrow["{\eta_s \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=3]
	\arrow["{\eta_t \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=2]
\end{tikzcd}\]
We must prove this pasting to satisfy the coherence condition of a pseudocoequalizer. This is done by combining pseudonaturality cubes of the units $ \eta$ over the canonical 2-cells $ \theta_{01},\theta_{12},\theta_{02}$ of the codescent diagram $ U_T\mathscr{X}$ together with the pseudocoequalizing property of $ \pi_0$ relative to the codescent diagram $ TU_T \mathscr{X}$
% https://q.uiver.app/?q=WzAsOSxbMCwwLCJBIl0sWzEsMCwiQiJdLFswLDEsIkIiXSxbMCwzLCJDIl0sWzMsMCwiQyJdLFsyLDMsIlRDIl0sWzMsMywiUF8wIl0sWzMsMiwiVEMiXSxbMSwxLCJCIl0sWzAsMiwiZiIsMl0sWzAsMSwiaCJdLFsyLDMsInQiLDJdLFsxLDQsInMiXSxbMyw1LCJcXGV0YV9DIiwyXSxbNCw3LCJcXGV0YV9DIl0sWzcsNl0sWzAsOCwiZyIsMV0sWzgsMywidCIsMV0sWzgsNCwicyIsMV0sWzUsNl0sWzIsOCwiXFx0aGV0YV97MTJ9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsOCwiXFx0aGV0YV97MDF9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsNiwiXFx4aV8wIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	A & B && C \\
	B & B \\
	&&& TC \\
	C && TC & {P_0}
	\arrow["f"', from=1-1, to=2-1]
	\arrow["h", from=1-1, to=1-2]
	\arrow["t"', from=2-1, to=4-1]
	\arrow["s", from=1-2, to=1-4]
	\arrow["{\eta_C}"', from=4-1, to=4-3]
	\arrow["{\eta_C}", from=1-4, to=3-4]
	\arrow["{p_0}", from=3-4, to=4-4]
	\arrow["g"{description}, from=1-1, to=2-2]
	\arrow["t"{description}, from=2-2, to=4-1]
	\arrow["s"{description}, from=2-2, to=1-4]
	\arrow["{p_0}"', from=4-3, to=4-4]
	\arrow["{\theta_{12} \atop \simeq}"{description}, draw=none, from=2-1, to=2-2]
	\arrow["{\theta_{01} \atop \simeq}"{description}, draw=none, from=1-2, to=2-2]
	\arrow["{\xi_0 \atop \simeq}"{description}, draw=none, from=2-2, to=4-4]
\end{tikzcd}
% https://q.uiver.app/?q=WzAsMTAsWzAsMCwiQSJdLFsxLDAsIkIiXSxbMCwxLCJCIl0sWzAsMywiQyJdLFszLDAsIkMiXSxbMiwzLCJUQyJdLFszLDMsIlBfMCJdLFszLDIsIlRDIl0sWzEsMSwiQiJdLFsyLDIsIlRCIl0sWzAsMiwiZiIsMl0sWzAsMSwiaCJdLFsyLDMsInQiLDJdLFsxLDQsInMiXSxbMyw1LCJcXGV0YV9DIiwyXSxbNCw3LCJcXGV0YV9DIl0sWzcsNl0sWzAsOCwiZyIsMV0sWzgsOSwiXFxldGFfQiIsMV0sWzksNSwiVHQiLDFdLFs5LDcsIlRzIiwxXSxbOCwzLCJ0IiwxXSxbOCw0LCJzIiwxXSxbOSw2LCJcXHBpXzAiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSw2XSxbMiw4LCJcXHRoZXRhX3sxMn0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMSw4LCJcXHRoZXRhX3swMX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMjEsMTksIlxcZXRhX3QgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMjIsMjAsIlxcZXRhX3MgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
=\begin{tikzcd}
	A & B && C \\
	B & B \\
	&& TB & TC \\
	C && TC & {P_0}
	\arrow["f"', from=1-1, to=2-1]
	\arrow["h", from=1-1, to=1-2]
	\arrow["t"', from=2-1, to=4-1]
	\arrow["s", from=1-2, to=1-4]
	\arrow["{\eta_C}"', from=4-1, to=4-3]
	\arrow["{\eta_C}", from=1-4, to=3-4]
	\arrow["{p_0}", from=3-4, to=4-4]
	\arrow["g"{description}, from=1-1, to=2-2]
	\arrow["{\eta_B}"{description}, from=2-2, to=3-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "Tt"{description}, from=3-3, to=4-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "Ts"{description}, from=3-3, to=3-4]
	\arrow[""{name=2, anchor=center, inner sep=0}, "t"{description}, from=2-2, to=4-1]
	\arrow[""{name=3, anchor=center, inner sep=0}, "s"{description}, from=2-2, to=1-4]
	\arrow["{\pi_0}"{description}, draw=none, from=3-3, to=4-4]
	\arrow["{p_0}"', from=4-3, to=4-4]
	\arrow["{\theta_{12} \atop \simeq}"{description}, draw=none, from=2-1, to=2-2]
	\arrow["{\theta_{01} \atop \simeq}"{description}, draw=none, from=1-2, to=2-2]
	\arrow["{\eta_t \atop \simeq}"{description}, Rightarrow, draw=none, from=2, to=0]
	\arrow["{\eta_s \atop \simeq}"{description}, Rightarrow, draw=none, from=3, to=1]
\end{tikzcd}\]
% https://q.uiver.app/?q=WzAsMTIsWzAsMCwiQSJdLFsxLDAsIkIiXSxbMCwxLCJCIl0sWzAsMywiQyJdLFszLDAsIkMiXSxbMiwzLCJUQyJdLFszLDMsIlBfMCJdLFszLDIsIlRDIl0sWzIsMSwiVEIiXSxbMSwyLCJUQiJdLFsxLDEsIlRBIl0sWzIsMiwiVEIiXSxbMCwyLCJmIiwyXSxbMCwxLCJoIl0sWzIsMywidCIsMl0sWzEsNCwicyJdLFszLDUsIlxcZXRhX0MiLDJdLFs0LDcsIlxcZXRhX0MiXSxbNyw2LCJwXzAiXSxbNSw2LCJwXzAiLDJdLFsxLDgsIlxcZXRhX0IiLDFdLFs4LDcsIlRzIiwxXSxbMiw5LCJcXGV0YV9CIiwxXSxbOSw1LCJUdCIsMV0sWzEwLDksIlRmIiwxXSxbMTAsOCwiVGgiLDFdLFswLDEwLCJcXGV0YV9BIiwxXSxbMTAsMTEsIlRnIiwxXSxbMTEsNV0sWzExLDddLFsxMSw2LCJcXHBpXzAgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCw0LCJcXGV0YV9zIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzksMywiXFxldGFfdCBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDExLCJUXFx0aGV0YV97MDF9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzksMTEsIlRcXHRoZXRhX3sxMn0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiwxMCwiXFxldGFfZiBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMCwxLCJcXGV0YV9oIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[=\begin{tikzcd}
	A & B && C \\
	B & TA & TB \\
	& TB & TB & TC \\
	C && TC & {P_0}
	\arrow["f"', from=1-1, to=2-1]
	\arrow["h", from=1-1, to=1-2]
	\arrow["t"', from=2-1, to=4-1]
	\arrow["s", from=1-2, to=1-4]
	\arrow["{\eta_C}"', from=4-1, to=4-3]
	\arrow["{\eta_C}", from=1-4, to=3-4]
	\arrow["{p_0}", from=3-4, to=4-4]
	\arrow["{p_0}"', from=4-3, to=4-4]
	\arrow["{\eta_B}"{description}, from=1-2, to=2-3]
	\arrow["Ts"{description}, from=2-3, to=3-4]
	\arrow["{\eta_B}"{description}, from=2-1, to=3-2]
	\arrow["Tt"{description}, from=3-2, to=4-3]
	\arrow["Tf"{description}, from=2-2, to=3-2]
	\arrow["Th"{description}, from=2-2, to=2-3]
	\arrow["{\eta_A}"{description}, from=1-1, to=2-2]
	\arrow["Tg"{description}, from=2-2, to=3-3]
	\arrow[from=3-3, to=4-3]
	\arrow[from=3-3, to=3-4]
	\arrow["{\pi_0 \atop \simeq}"{description}, draw=none, from=3-3, to=4-4]
	\arrow["{\eta_s \atop \simeq}"{description}, draw=none, from=2-3, to=1-4]
	\arrow["{\eta_t \atop \simeq}"{description}, draw=none, from=3-2, to=4-1]
	\arrow["{T\theta_{01} \atop \simeq}"{description}, draw=none, from=2-3, to=3-3]
	\arrow["{T\theta_{12} \atop \simeq}"{description}, draw=none, from=3-2, to=3-3]
	\arrow["{\eta_f \atop \simeq}"{description}, draw=none, from=2-1, to=2-2]
	\arrow["{\eta_h \atop \simeq}"{description}, draw=none, from=2-2, to=1-2]
\end{tikzcd}
% https://q.uiver.app/?q=WzAsMTIsWzAsMCwiQSJdLFsxLDAsIkIiXSxbMCwxLCJCIl0sWzAsMywiQyJdLFszLDAsIkMiXSxbMiwzLCJUQyJdLFszLDMsIlBfMCJdLFszLDIsIlRDIl0sWzIsMSwiVEIiXSxbMSwyLCJUQiJdLFsyLDIsIlRDIl0sWzEsMSwiVEEiXSxbMCwyLCJmIiwyXSxbMCwxLCJoIl0sWzIsMywidCIsMl0sWzEsNCwicyJdLFszLDUsIlxcZXRhX0MiLDJdLFs0LDcsIlxcZXRhX0MiXSxbNyw2LCJwXzAiXSxbNSw2LCJwXzAiLDJdLFsxLDgsIlxcZXRhX0IiLDFdLFs4LDcsIlRzIiwxXSxbMiw5LCJcXGV0YV9CIiwxXSxbOSw1LCJUdCIsMV0sWzgsNCwiXFxldGFfcyBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs5LDMsIlxcZXRhX3QgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOSwxMCwiVHQiLDFdLFs4LDEwLCJUcyIsMV0sWzEwLDZdLFsxMCw1LCJcXHBpXzAgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTAsNywiXFxwaV8wIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzExLDksIlRmIiwxXSxbMTEsOCwiVGgiLDFdLFswLDExLCJcXGV0YV9BIiwxXSxbMiwxMSwiXFxldGFfZiBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMSwxLCJcXGV0YV9oIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzExLDEwLCJUXFx0aGV0YV97MDJ9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
=\begin{tikzcd}
	A & B && C \\
	B & TA & TB \\
	& TB & TC & TC \\
	C && TC & {P_0}
	\arrow["f"', from=1-1, to=2-1]
	\arrow["h", from=1-1, to=1-2]
	\arrow["t"', from=2-1, to=4-1]
	\arrow["s", from=1-2, to=1-4]
	\arrow["{\eta_C}"', from=4-1, to=4-3]
	\arrow["{\eta_C}", from=1-4, to=3-4]
	\arrow["{p_0}", from=3-4, to=4-4]
	\arrow["{p_0}"', from=4-3, to=4-4]
	\arrow["{\eta_B}"{description}, from=1-2, to=2-3]
	\arrow["Ts"{description}, from=2-3, to=3-4]
	\arrow["{\eta_B}"{description}, from=2-1, to=3-2]
	\arrow["Tt"{description}, from=3-2, to=4-3]
	\arrow["{\eta_s \atop \simeq}"{description}, draw=none, from=2-3, to=1-4]
	\arrow["{\eta_t \atop \simeq}"{description}, draw=none, from=3-2, to=4-1]
	\arrow["Tt"{description}, from=3-2, to=3-3]
	\arrow["Ts"{description}, from=2-3, to=3-3]
	\arrow["p_0", from=3-3, to=4-4]
	\arrow["{\pi_0 \atop \simeq}"{description}, draw=none, from=3-3, to=4-3]
	\arrow["{\pi_0 \atop \simeq}"{description}, draw=none, from=3-3, to=3-4]
	\arrow["Tf"{description}, from=2-2, to=3-2]
	\arrow["Th"{description}, from=2-2, to=2-3]
	\arrow["{\eta_A}"{description}, from=1-1, to=2-2]
	\arrow["{\eta_f \atop \simeq}"{description}, draw=none, from=2-1, to=2-2]
	\arrow["{\eta_h \atop \simeq}"{description}, draw=none, from=2-2, to=1-2]
	\arrow["{T\theta_{02} \atop \simeq}"{description}, draw=none, from=2-2, to=3-3]
\end{tikzcd}\]
% https://q.uiver.app/?q=WzAsMTIsWzAsMCwiQSJdLFsxLDAsIkIiXSxbMCwxLCJCIl0sWzAsMywiQyJdLFszLDAsIkMiXSxbMiwzLCJUQyJdLFszLDMsIlBfMCJdLFszLDIsIlRDIl0sWzIsMSwiVEIiXSxbMSwyLCJUQiJdLFsyLDIsIlRDIl0sWzEsMSwiQyJdLFswLDIsImYiLDJdLFswLDEsImgiXSxbMiwzLCJ0IiwyXSxbMSw0LCJzIl0sWzMsNSwiXFxldGFfQyIsMl0sWzQsNywiXFxldGFfQyJdLFs3LDYsInBfMCJdLFs1LDYsInBfMCIsMl0sWzEsOCwiXFxldGFfQiIsMV0sWzgsNywiVHMiLDFdLFsyLDksIlxcZXRhX0IiLDFdLFs5LDUsIlR0IiwxXSxbOCw0LCJcXGV0YV9zIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzksMywiXFxldGFfdCBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs5LDEwLCJUdCIsMV0sWzgsMTAsIlRzIiwxXSxbMTAsNiwicF8wIiwxXSxbMTAsNSwiXFxwaV8wIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEwLDcsIlxccGlfMCBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMSwxMCwiXFxldGFfQyIsMV0sWzIsMTEsInQiLDFdLFsxLDExLCJzIiwxXSxbMCwxMSwiXFx0aGV0YV97MDJ9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzExLDgsIlxcZXRhX3MgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTEsOSwiXFxldGFfdCBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[=\begin{tikzcd}
	A & B && C \\
	B & C & TB \\
	& TB & TC & TC \\
	C && TC & {P_0}
	\arrow["f"', from=1-1, to=2-1]
	\arrow["h", from=1-1, to=1-2]
	\arrow["t"', from=2-1, to=4-1]
	\arrow["s", from=1-2, to=1-4]
	\arrow["{\eta_C}"', from=4-1, to=4-3]
	\arrow["{\eta_C}", from=1-4, to=3-4]
	\arrow["{p_0}", from=3-4, to=4-4]
	\arrow["{p_0}"', from=4-3, to=4-4]
	\arrow["{\eta_B}"{description}, from=1-2, to=2-3]
	\arrow["Ts"{description}, from=2-3, to=3-4]
	\arrow["{\eta_B}"{description}, from=2-1, to=3-2]
	\arrow["Tt"{description}, from=3-2, to=4-3]
	\arrow["{\eta_s \atop \simeq}"{description}, draw=none, from=2-3, to=1-4]
	\arrow["{\eta_t \atop \simeq}"{description}, draw=none, from=3-2, to=4-1]
	\arrow["Tt"{description}, from=3-2, to=3-3]
	\arrow["Ts"{description}, from=2-3, to=3-3]
	\arrow["{p_0}"{description}, from=3-3, to=4-4]
	\arrow["{\pi_0 \atop \simeq}"{description}, draw=none, from=3-3, to=4-3]
	\arrow["{\pi_0 \atop \simeq}"{description}, draw=none, from=3-3, to=3-4]
	\arrow["{\eta_C}"{description}, from=2-2, to=3-3]
	\arrow["t"{description}, from=2-1, to=2-2]
	\arrow["s"{description}, from=1-2, to=2-2]
	\arrow["{\theta_{02} \atop \simeq}"{description}, draw=none, from=1-1, to=2-2]
	\arrow["{\eta_s \atop \simeq}"{description}, draw=none, from=2-2, to=2-3]
	\arrow["{\eta_t \atop \simeq}"{description}, draw=none, from=2-2, to=3-2]
\end{tikzcd}
% https://q.uiver.app/?q=WzAsMTAsWzAsMCwiQSJdLFsxLDAsIkIiXSxbMCwxLCJCIl0sWzAsMywiQyJdLFszLDAsIkMiXSxbMiwzLCJUQyJdLFszLDMsIlBfMCJdLFszLDIsIlRDIl0sWzIsMiwiVEMiXSxbMSwxLCJDIl0sWzAsMiwiZiIsMl0sWzAsMSwiaCJdLFsyLDMsInQiLDJdLFsxLDQsInMiXSxbMyw1LCJcXGV0YV9DIiwyXSxbNCw3LCJcXGV0YV9DIl0sWzcsNiwicF8wIl0sWzUsNiwicF8wIiwyXSxbOCw2LCJwXzAiLDFdLFs5LDgsIlxcZXRhX0MiLDFdLFsyLDksInQiLDFdLFsxLDksInMiLDFdLFswLDksIlxcdGhldGFfezAyfSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszLDE5LCJcXHhpXzAgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCwxOSwiXFx4aV8wIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
=\begin{tikzcd}
	A & B && C \\
	B & C \\
	&& TC & TC \\
	C && TC & {P_0}
	\arrow["f"', from=1-1, to=2-1]
	\arrow["h", from=1-1, to=1-2]
	\arrow["t"', from=2-1, to=4-1]
	\arrow["s", from=1-2, to=1-4]
	\arrow["{\eta_C}"', from=4-1, to=4-3]
	\arrow["{\eta_C}", from=1-4, to=3-4]
	\arrow["{p_0}", from=3-4, to=4-4]
	\arrow["{p_0}"', from=4-3, to=4-4]
	\arrow["{p_0}"{description}, from=3-3, to=4-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\eta_C}"{description}, from=2-2, to=3-3]
	\arrow["t"{description}, from=2-1, to=2-2]
	\arrow["s"{description}, from=1-2, to=2-2]
	\arrow["{\theta_{02} \atop \simeq}"{description}, draw=none, from=1-1, to=2-2]
	\arrow["{\xi_0 \atop \simeq}"{description}, Rightarrow, draw=none, from=4-1, to=0]
	\arrow["{\xi_0 \atop \simeq}"{description}, Rightarrow, draw=none, from=1-4, to=0]
\end{tikzcd}\]

Proving the retraction identity is of the same vein and can be left as an exercise. 
\end{proof}




\begin{comment}
Both the composites $ \eta_{{\oplaxbicolim}_I \, T{A_i}} {\oplaxbicolim}_I \, \eta_{A_i} $ and $ T({\oplaxbicolim}_I \,; \eta_{A_i}) \eta_{{\oplaxbicolim}_I \, {A_i}}$ define a common pseudosection of $T{\oplaxbicolim}_I \, a_i$ and $ \mu_{{\oplaxbicolim}_I \, A_i} Ts$.

\end{comment}






\begin{comment}






On the other hand, the underlying morphisms of the corresponding free pseudomorphisms over the $k_i$ produce an oplax cocone $(Tk_i : TA_i \rightarrow TB)_{i \in I}$ inducing a universal factorization
% https://q.uiver.app/?q=WzAsMyxbMCwwLCJUQV9pIl0sWzIsMCwiVEQiXSxbMSwxLCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDEsIlRrX2kiXSxbMCwyLCJcXHdpZGV0aWxkZXtxfV9pIiwyXSxbMiwxLCJcXGxhbmdsZSBUa19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iLDJdLFszLDIsIlxcbnUnX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}
	{TA_i} && TB \\
	& {\underset{I}\oplaxbicolim \; A_i}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Tk_i}", from=1-1, to=1-3]
	\arrow["{q^{T}_i}"', from=1-1, to=2-2]
	\arrow["{\langle Tk_i \rangle_{i \in I}}"', from=2-2, to=1-3]
	\arrow["{\nu'_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=2-2]
\end{tikzcd}\]
Now, using again the oplax bicolimit property of $\oplaxbicolim_I a_i$ in $\ps[2,\mathcal{C}]$, we can extract a unique invertible 2-cell $ \kappa$ from the pasting below
% https://q.uiver.app/?q=WzAsNixbMCwxLCJUQV9pIl0sWzIsMSwiVEQiXSxbMSwwLCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMCwyLCJBX2kiXSxbMiwyLCJEX2kiXSxbMSwzLCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDEsIlRrX2kiLDFdLFswLDIsIlxcd2lkZXRpbGRle3F9X2kiXSxbMiwxLCJcXGxhbmdsZSBUa19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iXSxbMCwzLCJhX2kiLDJdLFszLDQsImtfaSIsMV0sWzEsNCwiZCJdLFszLDUsInFfaSIsMl0sWzUsNCwiXFxsYW5nbGUga19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iLDJdLFs2LDIsIlxcbnUnX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiwxMCwiXFxrYXBwYV9pIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEwLDUsIlxcbnVfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	& {\underset{I}\oplaxbicolim \; TA_i} \\
	{TA_i} && TB \\
	{A_i} && {B} \\
	& {\underset{I}\oplaxbicolim \; A_i}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Tk_i}"{description}, from=2-1, to=2-3]
	\arrow["{q^{T}_i}", from=2-1, to=1-2]
	\arrow["{\langle Tk_i \rangle_{i \in I}}", from=1-2, to=2-3]
	\arrow["{a_i}"', from=2-1, to=3-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{k_i}"{description}, from=3-1, to=3-3]
	\arrow["b", from=2-3, to=3-3]
	\arrow["{q_i}"', from=3-1, to=4-2]
	\arrow["{\langle k_i \rangle_{i \in I}}"', from=4-2, to=3-3]
	\arrow["{\nu'_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=1-2]
	\arrow["{\kappa_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=1]
	\arrow["{\nu_i \atop \simeq}"{description}, Rightarrow, draw=none, from=1, to=4-2]
\end{tikzcd}  =
% https://q.uiver.app/?q=WzAsNixbMCwxLCJUQV9pIl0sWzIsMSwiVEQiXSxbMSwwLCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IFRBX2kiXSxbMCwyLCJBX2kiXSxbMiwyLCJEX2kiXSxbMSwzLCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDIsIlxcd2lkZXRpbGRle3F9X2kiXSxbMiwxLCJcXGxhbmdsZSBUa19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iXSxbMCwzLCJhX2kiLDJdLFsxLDQsImQiXSxbMyw1LCJxX2kiLDJdLFs1LDQsIlxcbGFuZ2xlIGtfaSBcXHJhbmdsZV97aSBcXGluIEl9IiwyXSxbMiw1LCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSIsMV0sWzEyLDksIlxcb21lZ2FfaSBcXGF0b3AgXFxzaW1lcSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo3MCwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsMTIsIlxcdGhldGFfaSBcXGF0b3AgXFxzaW1lcSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjozMCwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\begin{tikzcd}
	& {\underset{I}\oplaxbicolim \; TA_i} \\
	{TA_i} && TB \\
	{A_i} && {B} \\
	& {\underset{I}\oplaxbicolim \; A_i}
	\arrow["{q^{T}_i}", from=2-1, to=1-2]
	\arrow["{\langle Tk_i \rangle_{i \in I}}", from=1-2, to=2-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{a_i}"', from=2-1, to=3-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "b", from=2-3, to=3-3]
	\arrow["{q_i}"', from=3-1, to=4-2]
	\arrow["{\langle k_i \rangle_{i \in I}}"', from=4-2, to=3-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\underset{I}\oplaxbicolim \; A_i}"{description}, from=1-2, to=4-2]
	\arrow["{\kappa \atop \simeq}"{description, pos=0.7}, Rightarrow, draw=none, from=2, to=1]
	\arrow["{\theta_i \atop \simeq}"{description, pos=0.3}, Rightarrow, draw=none, from=0, to=2]
\end{tikzcd}\]

The is a problem !!!



\textcolor{red}{Now we must prove that a certain pseudomorphism $(b T\langle k_i \rangle_{i \in I}, ??? )$ pseudocoequalizes the codescent diagram $ \mathscr{X}_{(A,a,(\alpha^t, \alpha^s))}$}. \\ 

We first prove that $b T\langle k_i \rangle_{i \in I}$ pseudocoequalizes the underlying codescent diagram in $\mathcal{C}$. To this end we first construct a certain auxiliary invertible 2-cell $ \nu = \langle T\nu_i \nu'_i \rangle_{i \in I} $ from the universal property of $\oplaxbicolim_I TA_i$ in the following pasting:
% https://q.uiver.app/?q=WzAsNCxbMSwwLCJUQV9pIl0sWzAsMSwiXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzIsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzEsMiwiVEQiXSxbMCwxLCJcXHdpZGV0aWxkZXtxfV9pIiwyXSxbMCwyLCJUcV9pIl0sWzEsMywiXFxsYW5nbGUgVGtfaSBcXHJhbmdsZV97aSBcXGluIEl9IiwyXSxbMiwzLCJUXFxsYW5nbGUga19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iXSxbMCwzLCJUa19pIiwxXSxbOCwxLCJcXG51X2knIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsMiwiVFxcbnVfaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}[column sep=tiny]
& {TA_i} \\
	{\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; A_i} \\
	& TB
	\arrow["{q^{T}_i}"', from=1-2, to=2-1]
	\arrow["{Tq_i}", from=1-2, to=2-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\langle Tk_i \rangle_{i \in I}}"', from=2-1, to=3-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{T\langle k_i \rangle_{i \in I}}", from=2-3, to=3-2]
	\arrow["{Tk_i}"{description, pos=0.6}, from=1-2, to=3-2]
	\arrow["{\nu_i' \atop \simeq}"{description, pos=0.6}, Rightarrow, draw=none, from=0, to=1-2]
	\arrow["{T\nu_i \atop \simeq}"{description, pos=0.4}, Rightarrow, draw=none, from=1-2, to=1]
\end{tikzcd}
% https://q.uiver.app/?q=WzAsNCxbMSwwLCJUQV9pIl0sWzAsMSwiXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzIsMSwiVFxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbSBcXDsgQV9pIl0sWzEsMiwiVEQiXSxbMCwxLCJcXHdpZGV0aWxkZXtxfV9pIiwyXSxbMCwyLCJUcV9pIl0sWzEsMywiXFxsYW5nbGUgVGtfaSBcXHJhbmdsZV97aSBcXGluIEl9IiwyXSxbMiwzLCJUXFxsYW5nbGUga19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iXSxbMSwyLCJzIiwxXSxbMCw4LCJcXHNpZ21hX2kgXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCwzLCJcXG51IFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
=\begin{tikzcd}[column sep=tiny]
	& {TA_i} \\
	{\underset{I}\oplaxbicolim \; TA_i} && {T\underset{I}\oplaxbicolim \; A_i} \\
	& TB
	\arrow["{q^{T}_i}"', from=1-2, to=2-1]
	\arrow["{Tq_i}", from=1-2, to=2-3]
	\arrow["{\langle Tk_i \rangle_{i \in I}}"', from=2-1, to=3-2]
	\arrow["{T\langle k_i \rangle_{i \in I}}", from=2-3, to=3-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "s"{description}, from=2-1, to=2-3]
	\arrow["{\sigma_i \atop \simeq}"{description}, Rightarrow, draw=none, from=1-2, to=0]
	\arrow["{\nu \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=3-2]
\end{tikzcd}\]
Now it suffices to take the following pasting as the inserted invertible 2-cell:
% https://q.uiver.app/?q=WzAsOCxbMSwwLCJUXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltIFxcOyBUQV9pIl0sWzAsMSwiVFRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFswLDIsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsxLDEsIlRURCJdLFsyLDAsIlRcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW0gXFw7IEFfaSJdLFsyLDEsIlREIl0sWzEsMiwiVEQiXSxbMiwyLCJEIl0sWzAsMSwiVChzKSIsMl0sWzEsMiwiXFxtdV9BIiwyXSxbMCwzLCJUXFxsYW5nbGUgVGtfaSBcXHJhbmdsZV97aSBcXGluIEl9Il0sWzEsMywiVFRcXGxhbmdsZSBrX2kgXFxyYW5nbGVfe2kgXFxpbiBJfSIsMl0sWzAsNCwiVGEiXSxbNCw1LCJUXFxsYW5nbGUga19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iXSxbMiw2LCJUXFxsYW5nbGUga19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iLDJdLFszLDYsIlxcbXVfRCJdLFszLDUsIlRkIiwxXSxbNiw3LCJkIiwyXSxbNSw3LCJkIl0sWzMsNywiXFxkZWx0YV5zIFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsNiwiXFxtdV97XFxsYW5nbGUga19pIFxccmFuZ2xlX3tpIFxcaW4gSX19IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsNSwiVFxca2FwcGEgXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCwzLCJUXFxudSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	& {T\underset{I}\oplaxbicolim \; TA_i} & {T\underset{I}\oplaxbicolim \; A_i} \\
	{TT\underset{I}\oplaxbicolim \; A_i} & TTB & TB \\
	{T\underset{I}\oplaxbicolim \; A_i} & TB & B
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Ts}"', from=1-2, to=2-1]
	\arrow["{\mu_{A}}"', from=2-1, to=3-1]
	\arrow["{T\langle Tk_i \rangle_{i \in I}}", from=1-2, to=2-2]
	\arrow["{TT\langle k_i \rangle_{i \in I}}"', from=2-1, to=2-2]
	\arrow["Ta", from=1-2, to=1-3]
	\arrow["{T\langle k_i \rangle_{i \in I}}", from=1-3, to=2-3]
	\arrow["{T\langle k_i \rangle_{i \in I}}"', from=3-1, to=3-2]
	\arrow["{\mu_D}", from=2-2, to=3-2]
	\arrow["Td"{description}, from=2-2, to=2-3]
	\arrow["b"', from=3-2, to=3-3]
	\arrow["b", from=2-3, to=3-3]
	\arrow["{\beta^s \atop \simeq}"{description}, draw=none, from=2-2, to=3-3]
	\arrow["{\mu_{\langle k_i \rangle_{i \in I}} \atop \simeq}"{description}, draw=none, from=2-1, to=3-2]
	\arrow["{T\kappa \atop \simeq}"{description}, draw=none, from=1-2, to=2-3]
	\arrow["{T\nu \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=2-2]
\end{tikzcd}\]

\textcolor{red}{The pseudomorphism structure ; this defines a transformation of pseudomorphism}\\

\textcolor{red}{The higher coherence conditions}



Then the composite $ (b T \langle k_i \rangle_{i \in I}, ...)$ pseudocoequalizes $ \mathscr{X}_\mathbb{A}$: this induces a canonical factorization throuhg some $ (g,\psi)$ ...
% https://q.uiver.app/?q=WzAsNixbMCwwLCIoVChBX2kpLFxcbXVfe0FfaX0sIChcXHhpX3tBX2l9LCBcXHJob197QV9pfSkgKSJdLFsyLDAsIihUKFxcdW5kZXJzZXR7SX17XFxvcGxheGJpY29saW19IFxcOyBBX2kpLCBcXG11X3tBfSwgKFxceGlfe0F9LCBcXHJob197QX0pIl0sWzAsMSwiKEFfaSwgYV9pLChcXGFscGhhXnRfaSwgXFxhbHBoYV5zX2kpKSJdLFsxLDIsIihCLGIsIChcXGJldGFedCxcXGJldGFecykpIl0sWzIsMSwiKEMsYywgKFxcZ2FtbWFedCxcXGdhbW1hXnMpKSJdLFsxLDEsIihUKEJfaSksXFxtdV97Ql9pfSwgKFxceGlfe0JfaX0sIFxccmhvX3tCX2l9KSApIl0sWzAsMSwiKFQocV9pKSwgXFxtdV97cV9pfSkiXSxbMCwyLCIoYV9pLFxcYWxwaGFfaV5zKSIsMl0sWzIsMywiKGtfaSwgXFxrYXBwYV9pKSIsMl0sWzEsNCwiKHAsIFxccGkpIl0sWzQsMywiKGcsXFxwc2kpIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzAsNSwiKFRrX2ksIFxcbXVfe2tfaX0pIiwxXSxbNSwzLCIoYi4uLiA/KSJdLFsxLDUsIihUXFxsYW5nbGUga19pIFxccmFuZ2xlX3tpIFxcaW4gSX0sLi4uKSIsMV0sWzEzLDEwLCI/IiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsNSwiPyIsMCx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMSw4LCI/IiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{(TA_i,\mu_{A_i}, (\xi_{A_i}, \rho_{A_i}) )} && {(T\underset{I}{\oplaxbicolim} \; A_i, \mu_{A}, (\xi_{A}, \rho_{A}))} \\
	{(A_i, a_i,(\alpha^t_i, \alpha^s_i))} & {(TB_i,\mu_{B_i}, (\xi_{B_i}, \rho_{B_i}) )} & {(C,c, (\gamma^t,\gamma^s))} \\
	& {(B,b, (\beta^t,\beta^s))}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{(Tq_i, \mu_{q_i})}", from=1-1, to=1-3]
	\arrow["{(a_i,\alpha_i^s)}"', from=1-1, to=2-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{(k_i, \kappa_i)}"', from=2-1, to=3-2]
	\arrow["{(p, \pi)}", from=1-3, to=2-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{(g,\psi)}", dashed, from=2-3, to=3-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{(Tk_i, \mu_{k_i})}"{description}, from=1-1, to=2-2]
	\arrow["{(b... ?)}", from=2-2, to=3-2]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{(T\langle k_i \rangle_{i \in I},...)}"{description}, from=1-3, to=2-2]
	\arrow["{?}"{description}, Rightarrow, draw=none, from=4, to=2]
	\arrow["{?}", Rightarrow, draw=none, from=0, to=2-2]
	\arrow["{?}"{description}, Rightarrow, draw=none, from=3, to=1]
\end{tikzcd}\]

\textcolor{red}{
Is the upper triangle a 2-cell in the 2-category $ [\mathbb{X}, T\hy\psAlg]$ ? If so, for the verticla map are each time the corresponding bicoequalizers, and the vertical face the 2-cell induced by the universal property of the bicoequalizers at those morphisms, the lower triangle is the 2-cell induced by the $ \bicoeq(-)$ 2-functor applied to those codescent diagrams. }

% https://q.uiver.app/?q=WzAsNSxbMCwwLCIoVChBX2kpLFxcbXVfe0FfaX0sIChcXHhpX3tBX2l9LCBcXHJob197QV9pfSkgKSJdLFsyLDAsIihUKFxcdW5kZXJzZXR7SX17XFxvcGxheGJpY29saW19IFxcOyBBX2kpLCBcXG11X3tcXHVuZGVyc2V0e0l9e1xcb3BsYXhiaWNvbGltfSBcXDsgQV9pfSwgKFxceGlfe1xcdW5kZXJzZXR7SX17XFxvcGxheGJpY29saW19IFxcOyBBX2l9LCBcXHJob197XFx1bmRlcnNldHtJfXtcXG9wbGF4Ymljb2xpbX0gXFw7IEFfaX0pIl0sWzAsMSwiKEFfaSwgYV9pLChcXGFscGhhXnRfaSwgXFxhbHBoYV5zX2kpKSJdLFsxLDIsIihCLGIsIChcXGJldGFedCxcXGJldGFecykpIl0sWzIsMSwiKEMsYywgKFxcZ2FtbWFedCxcXGdhbW1hXnMpKSJdLFswLDEsIihUKHFfaSksIFxcbXVfe3FfaX0pIl0sWzAsMiwiKGFfaSxcXGFscGhhX2lecykiLDJdLFsyLDMsIihrX2ksIFxca2FwcGFfaSkiLDJdLFsxLDQsIihwLCBcXHBpKSJdLFs0LDMsIj8iLDFdLFsyLDQsIihsX2ksXFxsYW1iZGFfaSkiLDFdLFs1LDEwLCJcXGNoaV9pIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMsMTAsIj8iLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}
	{(TA_i,\mu_{A_i}, (\xi_{A_i}, \rho_{A_i}) )} && {(T\underset{I}{\oplaxbicolim} \; A_i, \mu_{\underset{I}{\oplaxbicolim} \; A_i}, (\xi_{A}, \rho_{A}))} \\
	{(A_i, a_i,(\alpha^t_i, \alpha^s_i))} && {(C,c, (\gamma^t,\gamma^s))} \\
	& {(B,b, (\beta^t,\beta^s))}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{(Tq_i, \mu_{q_i})}", from=1-1, to=1-3]
	\arrow["{(a_i,\alpha_i^s)}"', from=1-1, to=2-1]
	\arrow["{(k_i, \kappa_i)}"', from=2-1, to=3-2]
	\arrow["{(p, \pi)}", from=1-3, to=2-3]
	\arrow["{?}"{description}, from=2-3, to=3-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{(l_i,\lambda_i)}"{description}, from=2-1, to=2-3]
	\arrow["{\chi_i \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=1]
	\arrow["{?}"{description}, Rightarrow, draw=none, from=3-2, to=1]
\end{tikzcd}\]
\end{comment}



























---------------------------------------------


























Now, from the functoriality in the way the universal 2-cells $ \theta_d'$ are induced, we have the following decomposition: 



% https://q.uiver.app/?q=WzAsOSxbMSwzLCJcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbVxcOyAgRlxcZG9tIl0sWzEsMiwiXFx1bmRlcnNldHtcXFNpZ21hXjJ9XFxvcGxheGJpY29saW1cXDsgIEZcXGRvbSJdLFszLDIsIkMiXSxbMywxLCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW1cXDsgIEYiXSxbMiwzLCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW1cXDsgIEYiXSxbMCwyLCJGXFxkb21cXCwgcF8wIFxccGhpIl0sWzAsMSwiRlxcY29kXFwscF8wXFxwaGkgPSBGIFxcZG9tIFxcLCBwXzFcXHBoaSJdLFsxLDAsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb20iXSxbMSwxLCJGXFxjb2RcXCxwXzFcXHBoaSAiXSxbMywyLCJcXGxhbmdsZSBxJ19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iXSxbMSwzLCJcXGxhbmdsZSBxX3tcXGRvbShkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9IiwxXSxbMCwzLCJcXGxhbmdsZSBxX3tcXGNvZChkKUYoZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzAsNCwiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMl0sWzQsMiwiXFxsYW5nbGUgcSdfaSBcXHJhbmdsZV97aSBcXGluIEl9IiwyLHsiY3VydmUiOjJ9XSxbNSwwLCJxXntcXGRvbX1fe3BfMFxccGhpfSIsMix7ImN1cnZlIjoyfV0sWzUsNiwiRnBfMFxccGhpIl0sWzYsMSwicV57XFxkb219X3twXzFcXHBoaX0iLDJdLFs2LDcsInFee1xcZG9tfV97cF8xXFxwaGl9IiwwLHsiY3VydmUiOi0yfV0sWzcsMywiXFxsYW5nbGUgcV97XFxjb2QoZClGKGQpfSBcXHJhbmdsZV97ZCBcXGluIFxcU2lnbWFeMn0iLDAseyJjdXJ2ZSI6LTJ9XSxbNiw4LCJGcF8xXFxwaGkiXSxbOCwzLCJxX3tcXGNvZCBcXCxwXzFcXHBoaX0iXSxbOCw3LCJcXHRoZXRhJ197cF8xXFxwaGl9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsMSwiIiwyLHsibGV2ZWwiOjJ9XSxbMSwwLCIiLDIseyJsZXZlbCI6Mn1dLFsxMSwyLCJcXGxhbmdsZSBcXHRoZXRhJ19kIHFfZCBcXHRoZXRhX2R7LTF9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSBcXGF0b3AgXFxzaW1lcSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo2MCwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	& {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} \\
	{F\cod\,p_0\phi = F \dom \, p_1\phi} & {F\cod\,p_1\phi } && {\underset{I}\oplaxbicolim\;  F} \\
	{F\dom\, p_0 \phi} & {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} && C \\
	& {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} & {\underset{I}\oplaxbicolim\;  F}
	\arrow["{\langle q'_i \rangle_{i \in I}}", from=2-4, to=3-4]
	\arrow["{\langle q_{\dom(d)} \rangle_{d \in \Sigma^2}}"{description}, from=3-2, to=2-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}"{description}, from=4-2, to=2-4]
	\arrow["{\langle q_{\dom(d)} \rangle_{d \in \Sigma^2}}"', from=4-2, to=4-3]
	\arrow["{\langle q'_i \rangle_{i \in I}}"', curve={height=12pt}, from=4-3, to=3-4]
	\arrow["{q^{\dom}_{p_0\phi}}"', curve={height=12pt}, from=3-1, to=4-2]
	\arrow["{Fp_0\phi}", from=3-1, to=2-1]
	\arrow["{q^{\dom}_{p_1\phi}}"', from=2-1, to=3-2]
	\arrow["{q^{\dom}_{p_1\phi}}", curve={height=-12pt}, from=2-1, to=1-2]
	\arrow["{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}", curve={height=-12pt}, from=1-2, to=2-4]
	\arrow["{Fp_1\phi}", from=2-1, to=2-2]
	\arrow["{q_{\cod \,p_1\phi}}", from=2-2, to=2-4]
	\arrow["{\theta'_{p_1\phi} \atop \simeq}"{description}, draw=none, from=2-2, to=1-2]
	\arrow[Rightarrow, from=2-2, to=3-2]
	\arrow[Rightarrow, from=3-2, to=4-2]
	\arrow["{\langle \theta'_d q_d \theta_d{-1} \rangle_{d \in \Sigma^2} \atop \simeq}"{description, pos=0.6}, Rightarrow, draw=none, from=0, to=3-4]
\end{tikzcd}\]






% https://q.uiver.app/?q=WzAsOSxbMSw0LCJcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbVxcOyAgRlxcZG9tIl0sWzEsMiwiXFx1bmRlcnNldHtcXFNpZ21hXjJ9XFxvcGxheGJpY29saW1cXDsgIEZcXGRvbSJdLFszLDMsIkMiXSxbMywyLCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW1cXDsgIEYiXSxbMiw0LCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW1cXDsgIEYiXSxbMCwzLCJGXFxkb21cXCwgcF8wIFxccGhpIl0sWzAsMiwiRlxcY29kXFwscF8wXFxwaGkgPSBGIFxcZG9tIFxcLCBwXzFcXHBoaSJdLFsxLDAsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb20iXSxbMSwxLCJGXFxjb2RcXCxwXzFcXHBoaSAiXSxbMywyLCJcXGxhbmdsZSBxJ19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iXSxbMSwzLCJcXGxhbmdsZSBxX3tcXGRvbShkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9IiwxXSxbMCwzLCJcXGxhbmdsZSBxX3tcXGNvZChkKUYoZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzAsNCwiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMl0sWzQsMiwiXFxsYW5nbGUgcSdfaSBcXHJhbmdsZV97aSBcXGluIEl9IiwyLHsiY3VydmUiOjJ9XSxbNSwwLCJxXntcXGRvbX1fe3BfMFxccGhpfSIsMix7ImN1cnZlIjoyfV0sWzUsNiwiRnBfMFxccGhpIl0sWzYsMSwicV57XFxkb219X3twXzFcXHBoaX0iLDJdLFs2LDcsInFee1xcZG9tfV97cF8xXFxwaGl9IiwwLHsiY3VydmUiOi0yfV0sWzcsMywiXFxsYW5nbGUgcV97XFxjb2QoZClGKGQpfSBcXHJhbmdsZV97ZCBcXGluIFxcU2lnbWFeMn0iLDAseyJjdXJ2ZSI6LTJ9XSxbNiw4LCJGcF8xXFxwaGkiXSxbOCwzLCJxX3tcXGNvZCBcXCxwXzFcXHBoaX0iLDAseyJvZmZzZXQiOi0xLCJjdXJ2ZSI6LTF9XSxbOCw3LCJcXHRoZXRhJ197cF8xXFxwaGl9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsMywicV97XFxkb20gXFwscF8xXFxwaGl9IiwyLHsiY3VydmUiOjN9XSxbNiwzLCJxX3tcXGRvbSBcXCxwXzFcXHBoaX0iLDEseyJjdXJ2ZSI6LTJ9XSxbMTEsMiwiXFxsYW5nbGUgXFx0aGV0YSdfZCBxX2QgXFx0aGV0YV9key0xfSBcXHJhbmdsZV97ZCBcXGluIFxcU2lnbWFeMn0gXFxhdG9wIFxcc2ltZXEiLDEseyJsYWJlbF9wb3NpdGlvbiI6NjAsInNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxLDIyLCJcXHRoZXRhX3twXzFcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDAseyJsYWJlbF9wb3NpdGlvbiI6ODAsInNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxNCwyMiwiXFx0aGV0YSdfe3BfMFxccGhpfSBcXGF0b3AgXFxzaW1lcSIsMCx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDIzLCJxX3twXzFcXHBoaX0iLDAseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9fV0sWzIzLDEwLCJcXHRoZXRhX3twXzFcXHBoaX1eey0xfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	& {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} \\
	& {F\cod\,p_1\phi } \\
	{F\cod\,p_0\phi = F \dom \, p_1\phi} & {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} && {\underset{I}\oplaxbicolim\;  F} \\
	{F\dom\, p_0 \phi} &&& C \\
	& {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} & {\underset{I}\oplaxbicolim\;  F}
	\arrow["{\langle q'_i \rangle_{i \in I}}", from=3-4, to=4-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\langle q_{\dom(d)} \rangle_{d \in \Sigma^2}}"{description}, from=3-2, to=3-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}"{description}, from=5-2, to=3-4]
	\arrow["{\langle q_{\dom(d)} \rangle_{d \in \Sigma^2}}"', from=5-2, to=5-3]
	\arrow["{\langle q'_i \rangle_{i \in I}}"', curve={height=12pt}, from=5-3, to=4-4]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{q^{\dom}_{p_0\phi}}"', curve={height=12pt}, from=4-1, to=5-2]
	\arrow["{Fp_0\phi}", from=4-1, to=3-1]
	\arrow["{q^{\dom}_{p_1\phi}}"', from=3-1, to=3-2]
	\arrow["{q^{\dom}_{p_1\phi}}", curve={height=-12pt}, from=3-1, to=1-2]
	\arrow["{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}", curve={height=-12pt}, from=1-2, to=3-4]
	\arrow["{Fp_1\phi}", from=3-1, to=2-2]
	\arrow["{q_{\cod \,p_1\phi}}", shift left=1, curve={height=-6pt}, from=2-2, to=3-4]
	\arrow["{\theta'_{p_1\phi} \atop \simeq}"{description}, draw=none, from=2-2, to=1-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{q_{\dom \,p_1\phi}}"', curve={height=18pt}, from=3-1, to=3-4]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{q_{\dom \,p_1\phi}}"{description}, curve={height=-12pt}, from=3-1, to=3-4]
	\arrow["{\langle \theta'_d q_d \theta_d{-1} \rangle_{d \in \Sigma^2} \atop \simeq}"{description, pos=0.6}, Rightarrow, draw=none, from=1, to=4-4]
	\arrow["{\theta_{p_1\phi} \atop \simeq}"{pos=0.8}, Rightarrow, draw=none, from=3-2, to=3]
	\arrow["{\theta'_{p_0\phi} \atop \simeq}", Rightarrow, draw=none, from=2, to=3]
	\arrow["{q_{p_1\phi}}", shorten >=4pt, Rightarrow, from=2-2, to=4]
	\arrow["{\theta_{p_1\phi}^{-1} \atop \simeq}"{description}, Rightarrow, draw=none, from=4, to=0]
\end{tikzcd}\]




% https://q.uiver.app/?q=WzAsNSxbMCwxLCJGXFxkb21cXCxwXzBcXHBoaSA9IEZcXGRvbVxcLHBfMlxccGhpIl0sWzIsMSwiRlxcY29kXFwscF8yXFxwaGkgPSBGXFxjb2RcXCxwXzFcXHBoaSJdLFsxLDMsIntcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW1cXDsgIEZ9Il0sWzAsMiwie1xcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb219Il0sWzEsMCwiRlxcY29kXFwscF8wXFxwaGkgPSBGXFxkb21cXCxwXzFcXHBoaSJdLFswLDEsIkZwXzJcXHBoaSIsMV0sWzEsMiwicV97XFxjb2QgXFwsIHBfMlxccGhpfSJdLFswLDMsInFee1xcZG9tfV97cF8yfSIsMl0sWzMsMiwiXFxsYW5nbGUgcV97XFxjb2QoZClGKGQpfSBcXHJhbmdsZV97ZCBcXGluIFxcU2lnbWFeMn0iLDJdLFswLDQsIkZwXzBcXHBoaSJdLFs0LDEsIkZwXzFcXHBoaSJdLFs1LDIsInFfe3BfMFxccGhpfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDUsIkZcXHBoaSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	& {F\cod\,p_0\phi = F\dom\,p_1\phi} \\
	{F\dom\,p_0\phi = F\dom\,p_2\phi} && {F\cod\,p_2\phi = F\cod\,p_1\phi} \\
	{{\underset{\Sigma^2}\oplaxbicolim\;  F\dom}} \\
	& {{\underset{I}\oplaxbicolim\;  F}}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{Fp_2\phi}"{description}, from=2-1, to=2-3]
	\arrow["{q_{\cod \, p_2\phi}}", from=2-3, to=4-2]
	\arrow["{q^{\dom}_{p_2}}"', from=2-1, to=3-1]
	\arrow["{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}"', from=3-1, to=4-2]
	\arrow["{Fp_0\phi}", from=2-1, to=1-2]
	\arrow["{Fp_1\phi}", from=1-2, to=2-3]
	\arrow["{q_{p_0\phi} \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=4-2]
	\arrow["{F\phi \atop \simeq}"{description}, Rightarrow, draw=none, from=1-2, to=0]
\end{tikzcd}\]
% https://q.uiver.app/?q=WzAsNixbMCwxLCJGXFxkb21cXCxwXzBcXHBoaSA9IEZcXGRvbVxcLHBfMlxccGhpIl0sWzIsMSwiRlxcY29kXFwscF8yXFxwaGkgPSBGXFxjb2RcXCxwXzFcXHBoaSJdLFsxLDQsIntcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW1cXDsgIEZ9Il0sWzAsMywie1xcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb219Il0sWzEsMCwiRlxcY29kXFwscF8wXFxwaGkgPSBGXFxkb21cXCxwXzFcXHBoaSJdLFsxLDIsIntcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbVxcOyAgRlxcZG9tfSJdLFsxLDIsInFfe1xcY29kIFxcLCBwXzJcXHBoaX0gPSBxX3tcXGNvZCBcXCwgcF8xXFxwaGl9Il0sWzAsMywicV57XFxkb219X3twXzJ9IiwyXSxbMywyLCJcXGxhbmdsZSBxX3tcXGNvZChkKUYoZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMl0sWzAsNCwiRnBfMFxccGhpIl0sWzQsMSwiRnBfMVxccGhpIl0sWzUsMiwiXFxsYW5nbGUgcV97XFxjb2QoZClGKGQpfSBcXHJhbmdsZV97ZCBcXGluIFxcU2lnbWFeMn0iLDFdLFswLDUsInFee1xcZG9tfV97cF8wXFxwaGl9IiwxXSxbMCwyLCJcXHRoZXRhX3twXzBcXHBoaX0gXFx0aGV0YV57LTF9X3twXzJcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSw0LCJcXHRoZXRhJ197RnBfMVxccGhpIEZwXzBcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[=\begin{tikzcd}
	& {F\cod\,p_0\phi = F\dom\,p_1\phi} \\
	{F\dom\,p_0\phi = F\dom\,p_2\phi} && {F\cod\,p_2\phi = F\cod\,p_1\phi} \\
	& {{\underset{\Sigma^2}\oplaxbicolim\;  F\dom}} \\
	{{\underset{\Sigma^2}\oplaxbicolim\;  F\dom}} \\
	& {{\underset{I}\oplaxbicolim\;  F}}
	\arrow["{q_{\cod \, p_2\phi} = q_{\cod \, p_1\phi}}", from=2-3, to=5-2]
	\arrow["{q^{\dom}_{p_2}}"', from=2-1, to=4-1]
	\arrow["{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}"', from=4-1, to=5-2]
	\arrow["{Fp_0\phi}", from=2-1, to=1-2]
	\arrow["{Fp_1\phi}", from=1-2, to=2-3]
	\arrow["{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}"{description}, from=3-2, to=5-2]
	\arrow["{q^{\dom}_{p_0\phi}}"{description}, from=2-1, to=3-2]
	\arrow["{\theta_{p_0\phi} \theta^{-1}_{p_2\phi} \atop \simeq}"{description}, draw=none, from=2-1, to=5-2]
	\arrow["{\theta'_{Fp_1\phi Fp_0\phi} \atop \simeq}"{description}, draw=none, from=3-2, to=1-2]
\end{tikzcd}\]

Then we can perform the corresponding substitution in the diagram above to get the following:

% https://q.uiver.app/?q=WzAsOSxbMSwwLCJGXFxkb21cXCwgcF8wIFxccGhpID0gRlxcZG9tIFxcLCBwXzIgXFxwaGkiXSxbMywwLCJGXFxjb2RcXCxwXzBcXHBoaSA9IEYgXFxkb20gXFwsIHBfMVxccGhpIl0sWzEsMiwiXFx1bmRlcnNldHtcXFNpZ21hXjJ9XFxvcGxheGJpY29saW1cXDsgIEZcXGRvbSJdLFs0LDIsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb20iXSxbMiw0LCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW1cXDsgIEYiXSxbMywyLCJGXFxjb2QgXFwsIHBfMiBcXHBoaSA9IEZcXGNvZCBcXCwgcF8xIFxccGhpIl0sWzAsMiwiXFx1bmRlcnNldHtcXFNpZ21hXjJ9XFxvcGxheGJpY29saW1cXDsgIEZcXGRvbSJdLFsyLDUsIkMiXSxbMiwyLCJcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbVxcOyAgRlxcZG9tIl0sWzAsMSwiRnBfMFxccGhpIl0sWzAsMiwicV57XFxkb219X3twXzJcXHBoaX0iLDJdLFsxLDMsInFee1xcZG9tfV97cF8xXFxwaGl9Il0sWzMsNCwiXFxsYW5nbGUgcV97XFxjb2QoZClGKGQpfSBcXHJhbmdsZV97ZCBcXGluIFxcU2lnbWFeMn0iXSxbMCw1LCJGcF8yXFxwaGkiLDFdLFsxLDUsIkZwXzFcXHBoaSIsMV0sWzUsNCwicV97XFxjb2QgXFwsIHBfMiBcXHBoaSB9PSBxX3tcXGNvZCBcXCwgcF8xIFxccGhpfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MH1dLFswLDYsInFee1xcZG9tfV97cF8wXFxwaGl9IiwyXSxbNCw3LCJcXGxhbmdsZSBxJ19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iXSxbMCw4LCJxXntcXGRvbX1fe3BfMlxccGhpfSAiLDEseyJsYWJlbF9wb3NpdGlvbiI6ODB9XSxbOCw0LCJcXGxhbmdsZSBxX3tcXGNvZChkKUYoZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzIsNCwiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzYsNCwiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMl0sWzksNSwiRlxccGhpIFxcYXRvcCBcXHNpbWVxIiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE0LDMsIlxcdGhldGEnX3twXzFcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJsZXZlbCI6MSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE2LDIsIlxcdGhldGFfe3BfMFxccGhpfSBcXHRoZXRhXnstMX1fe3BfMlxccGhpfSBcXGF0b3AgXFxzaW1lcSIsMSx7ImxldmVsIjoxLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMTgsIlxcdGhldGEnX3twXzJcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiwxOCwiXFx0aGV0YSdfe3BfMlxccGhpfXFee1xcZG9tfV97cF8yXFxwaGl9XFx0aGV0YV57LTF9X3twXzJcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=


% https://q.uiver.app/?q=WzAsMTAsWzAsMywiRlxcZG9tXFwsIHBfMCBcXHBoaSA9IEZcXGRvbSBcXCwgcF8yIFxccGhpIl0sWzAsMSwiRlxcY29kXFwscF8wXFxwaGkgPSBGIFxcZG9tIFxcLCBwXzFcXHBoaSJdLFsyLDQsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb20iXSxbNCwzLCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW1cXDsgIEYiXSxbMiwxLCJGXFxjb2QgXFwsIHBfMiBcXHBoaSA9IEZcXGNvZCBcXCwgcF8xIFxccGhpIl0sWzIsNSwiXFx1bmRlcnNldHtcXFNpZ21hXjJ9XFxvcGxheGJpY29saW1cXDsgIEZcXGRvbSJdLFs1LDMsIkMiXSxbMiwzLCJcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbVxcOyAgRlxcZG9tIl0sWzIsMiwiXFx1bmRlcnNldHtcXFNpZ21hXjJ9XFxvcGxheGJpY29saW1cXDsgIEZcXGRvbSJdLFsyLDAsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb20iXSxbMCwxLCJGcF8wXFxwaGkiXSxbMCwyLCJxXntcXGRvbX1fe3BfMlxccGhpfSIsMl0sWzEsNCwiRnBfMVxccGhpIiwyXSxbNCwzLCJxX3tcXGNvZCBcXCwgcF8yIFxccGhpIH09IHFfe1xcY29kIFxcLCBwXzEgXFxwaGl9IiwxLHsibGFiZWxfcG9zaXRpb24iOjQwfV0sWzAsNSwicV57XFxkb219X3twXzBcXHBoaX0iLDJdLFszLDYsIlxcbGFuZ2xlIHEnX2kgXFxyYW5nbGVfe2kgXFxpbiBJfSJdLFswLDcsInFee1xcZG9tfV97cF8yXFxwaGl9ICIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo4MH1dLFs3LDMsIlxcbGFuZ2xlIHFfe1xcY29kKGQpRihkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9Il0sWzIsMywiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzUsMywiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMix7Im9mZnNldCI6MSwiY3VydmUiOjJ9XSxbMCw4LCJxXlxcZG9tX3twXzBcXHBoaX0iLDFdLFs4LDMsIlxcbGFuZ2xlIHFfe1xcY29kKGQpRihkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9IiwxXSxbMSw5LCJxXntcXGRvbX1fe3BfMVxccGhpfSJdLFs5LDMsIlxcbGFuZ2xlIHFfe1xcY29kKGQpRihkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9IiwwLHsib2Zmc2V0IjotMSwiY3VydmUiOi0yfV0sWzcsOCwiXFx0aGV0YSdfe3BfMFxccGhpfSBcXHRoZXRhJ157LTF9X3twXzJcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiw3LCJcXHRoZXRhJ197cF8yXFxwaGl9cV57XFxkb219X3twXzJcXHBoaX1cXHRoZXRhXnstMX1fe3BfMlxccGhpfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSwyLCJcXHRoZXRhX3twXzBcXHBoaX0gXFx0aGV0YV57LTF9X3twXzJcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw5LCJcXHRoZXRhJ197cF8xXFxwaGl9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIwLDEsIlxcdGhldGFfe3BfMFxccGhpfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==


% https://q.uiver.app/?q=WzAsMTAsWzAsMywiRlxcZG9tXFwsIHBfMCBcXHBoaSA9IEZcXGRvbSBcXCwgcF8yIFxccGhpIl0sWzAsMSwiRlxcY29kXFwscF8wXFxwaGkgPSBGIFxcZG9tIFxcLCBwXzFcXHBoaSJdLFsyLDQsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb20iXSxbNCwzLCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW1cXDsgIEYiXSxbMiwxLCJGXFxjb2QgXFwsIHBfMiBcXHBoaSA9IEZcXGNvZCBcXCwgcF8xIFxccGhpIl0sWzIsNSwiXFx1bmRlcnNldHtcXFNpZ21hXjJ9XFxvcGxheGJpY29saW1cXDsgIEZcXGRvbSJdLFs1LDMsIkMiXSxbMiwzLCJcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbVxcOyAgRlxcZG9tIl0sWzIsMCwiXFx1bmRlcnNldHtcXFNpZ21hXjJ9XFxvcGxheGJpY29saW1cXDsgIEZcXGRvbSJdLFsyLDIsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb20iXSxbMCwxLCJGcF8wXFxwaGkiXSxbMCwyLCJxXntcXGRvbX1fe3BfMlxccGhpfSIsMl0sWzEsNCwiRnBfMVxccGhpIiwyXSxbNCwzLCJxX3tcXGNvZCBcXCwgcF8yIFxccGhpIH09IHFfe1xcY29kIFxcLCBwXzEgXFxwaGl9IiwxLHsibGFiZWxfcG9zaXRpb24iOjQwfV0sWzAsNSwicV57XFxkb219X3twXzBcXHBoaX0iLDIseyJjdXJ2ZSI6Mn1dLFszLDYsIlxcbGFuZ2xlIHEnX2kgXFxyYW5nbGVfe2kgXFxpbiBJfSJdLFswLDcsInFee1xcZG9tfV97cF8yXFxwaGl9ICIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo4MH1dLFs3LDMsIlxcbGFuZ2xlIHFfe1xcY29kKGQpRihkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9Il0sWzIsMywiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzUsMywiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMix7Im9mZnNldCI6MSwiY3VydmUiOjJ9XSxbMSw4LCJxXntcXGRvbX1fe3BfMVxccGhpfSIsMCx7ImN1cnZlIjotMn1dLFs4LDMsIlxcbGFuZ2xlIHFfe1xcY29kKGQpRihkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9IiwwLHsib2Zmc2V0IjotMSwiY3VydmUiOi0zfV0sWzIsNywiXFx0aGV0YSdfe3BfMlxccGhpfXFee1xcZG9tfV97cF8yXFxwaGl9XFx0aGV0YV57LTF9X3twXzJcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDAseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJsZXZlbCI6Mn1dLFs1LDIsIlxcdGhldGFfe3BfMFxccGhpfSBcXHRoZXRhXnstMX1fe3BfMlxccGhpfSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDksInFeXFxkb21fe3BfMFxccGhpfSIsMV0sWzksMywiXFxsYW5nbGUgcV97XFxjb2QoZClGKGQpfSBcXHJhbmdsZV97ZCBcXGluIFxcU2lnbWFeMn0iLDFdLFs3LDksIlxcdGhldGEnX3twXzBcXHBoaX0gXFx0aGV0YSdeey0xfV97cF8yXFxwaGl9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzQsOCwiXFx0aGV0YSdfe3BfMVxccGhpfSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyNCwxLCJcXHRoZXRhX3twXzBcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}
	&& {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} \\
	{F\cod\,p_0\phi = F \dom \, p_1\phi} && {F\cod \, p_2 \phi = F\cod \, p_1 \phi} \\
	&& {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} \\
	{F\dom\, p_0 \phi = F\dom \, p_2 \phi} && {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} && {\underset{I}\oplaxbicolim\;  F} & C \\
	&& {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} \\
	&& {\underset{\Sigma^2}\oplaxbicolim\;  F\dom}
	\arrow["{Fp_0\phi}", from=4-1, to=2-1]
	\arrow["{q^{\dom}_{p_2\phi}}"', from=4-1, to=5-3]
	\arrow["{Fp_1\phi}"', from=2-1, to=2-3]
	\arrow["{q_{\cod \, p_2 \phi }= q_{\cod \, p_1 \phi}}"{description, pos=0.4}, from=2-3, to=4-5]
	\arrow["{q^{\dom}_{p_0\phi}}"', curve={height=12pt}, from=4-1, to=6-3]
	\arrow["{\langle q'_i \rangle_{i \in I}}", from=4-5, to=4-6]
	\arrow["{q^{\dom}_{p_2\phi} }"{description, pos=0.8}, from=4-1, to=4-3]
	\arrow["{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}", from=4-3, to=4-5]
	\arrow["{\langle q_{\dom(d)} \rangle_{d \in \Sigma^2}}"{description}, from=5-3, to=4-5]
	\arrow["{\langle q_{\dom(d)} \rangle_{d \in \Sigma^2}}"', shift right=1, curve={height=12pt}, from=6-3, to=4-5]
	\arrow["{q^{\dom}_{p_1\phi}}", curve={height=-12pt}, from=2-1, to=1-3]
	\arrow["{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}", shift left=1, curve={height=-18pt}, from=1-3, to=4-5]
	\arrow["{\theta'_{p_2\phi}q^{\dom}_{p_2\phi}\theta^{-1}_{p_2\phi} \atop \simeq}", shorten >=2pt, Rightarrow, from=5-3, to=4-3]
	\arrow["{\theta_{p_0\phi} \theta^{-1}_{p_2\phi} \atop \simeq}"{description}, draw=none, from=6-3, to=5-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{q^\dom_{p_0\phi}}"{description}, from=4-1, to=3-3]
	\arrow["{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}"{description}, from=3-3, to=4-5]
	\arrow["{\theta'_{p_0\phi} \theta'^{-1}_{p_2\phi} \atop \simeq}"{description}, draw=none, from=4-3, to=3-3]
	\arrow["{\theta'_{p_1\phi} \atop \simeq}"{description}, draw=none, from=2-3, to=1-3]
	\arrow["{\theta_{p_0\phi} \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=2-1]
\end{tikzcd}\]

Now we can paste the 

% https://q.uiver.app/?q=WzAsOSxbMiwwLCJGXFxkb21cXCwgcF8wIFxccGhpID0gRlxcZG9tIFxcLCBwXzIgXFxwaGkiXSxbMywwLCJGXFxjb2RcXCxwXzBcXHBoaSA9IEYgXFxkb20gXFwsIHBfMVxccGhpIl0sWzEsMiwiXFx1bmRlcnNldHtcXFNpZ21hXjJ9XFxvcGxheGJpY29saW1cXDsgIEZcXGRvbSJdLFszLDQsIlxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbVxcOyAgRiJdLFs0LDEsIkZcXGNvZCBcXCwgcF8yIFxccGhpID0gRlxcY29kIFxcLCBwXzEgXFxwaGkiXSxbMCwyLCJcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbVxcOyAgRlxcZG9tIl0sWzMsNSwiQyJdLFsyLDIsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb20iXSxbMywyLCJcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbVxcOyAgRlxcZG9tIl0sWzAsMSwiRnBfMFxccGhpIl0sWzAsMiwicV57XFxkb219X3twXzJcXHBoaX0iLDJdLFsxLDQsIkZwXzFcXHBoaSIsMl0sWzQsMywicV97XFxjb2QgXFwsIHBfMiBcXHBoaSB9PSBxX3tcXGNvZCBcXCwgcF8xIFxccGhpfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MH1dLFswLDUsInFee1xcZG9tfV97cF8wXFxwaGl9IiwyXSxbMyw2LCJcXGxhbmdsZSBxJ19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iXSxbMCw3LCJxXntcXGRvbX1fe3BfMlxccGhpfSAiLDEseyJsYWJlbF9wb3NpdGlvbiI6ODB9XSxbNywzLCJcXGxhbmdsZSBxX3tcXGNvZChkKUYoZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzIsMywiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzUsMywiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMl0sWzAsOCwicV5cXGRvbV97cF8wXFxwaGl9IiwxXSxbOCwzLCJcXGxhbmdsZSBxX3tcXGNvZChkKUYoZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzEzLDIsIlxcdGhldGFfe3BfMFxccGhpfSBcXHRoZXRhXnstMX1fe3BfMlxccGhpfSBcXGF0b3AgXFxzaW1lcSIsMSx7ImxldmVsIjoxLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiwxNSwiXFx0aGV0YSdfe3BfMlxccGhpfXFee1xcZG9tfV97cF8yXFxwaGl9XFx0aGV0YV57LTF9X3twXzJcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InRhcmdldCI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNywxOSwiXFx0aGV0YSdfe3BfMFxccGhpfSBcXHRoZXRhJ157LTF9X3twXzJcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJsZXZlbCI6MSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE5LDEsIlxcdGhldGFfe3BfMFxccGhpfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==




% https://q.uiver.app/?q=WzAsOCxbMSwwLCJGXFxkb21cXCwgcF8wIFxccGhpIl0sWzIsMCwiRlxcY29kXFwscF8wXFxwaGkgPSBGIFxcZG9tIFxcLCBwXzFcXHBoaSJdLFsxLDEsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb20iXSxbMywxLCJcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbVxcOyAgRlxcZG9tIl0sWzEsMywiQyJdLFszLDIsIlxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbVxcOyAgRiJdLFswLDEsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb20iXSxbMSwyLCJcXHVuZGVyc2V0e0l9XFxvcGxheGJpY29saW1cXDsgIEYiXSxbMCwxLCJGcF8wXFxwaGkiXSxbMCwyLCJxXntcXGRvbX1fe3BfMFxccGhpfSJdLFsxLDMsInFee1xcZG9tfV97cF8xXFxwaGl9Il0sWzMsNSwiXFxsYW5nbGUgcV97XFxjb2QoZClGKGQpfSBcXHJhbmdsZV97ZCBcXGluIFxcU2lnbWFeMn0iXSxbNSw0LCJcXGxhbmdsZSBxJ19pIFxccmFuZ2xlX3tpIFxcaW4gSX0iLDFdLFswLDYsInFee1xcZG9tfV97cF8wXFxwaGl9IiwyXSxbNiw3LCJcXGxhbmdsZSBxX3tcXGRvbShkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9IiwyXSxbMiw3LCJcXGxhbmdsZSBxX3tcXGNvZChkKUYoZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzEsNywicV97XFxkb21cXCwgcF8xfSIsMV0sWzMsNywiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzcsNCwiXFxsYW5nbGUgcSdfaSBcXHJhbmdsZV97aSBcXGluIEl9IiwyXSxbMTYsMywiXFx0aGV0YV97cF8xfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyLDE2LCJcXHRoZXRhJ197cF8wfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==












% https://q.uiver.app/?q=WzAsOCxbMCwyLCJGXFxkb21cXCwgcF8wIFxccGhpIl0sWzAsMSwiRlxcY29kXFwscF8wXFxwaGkgPSBGIFxcZG9tIFxcLCBwXzFcXHBoaSJdLFsxLDQsIlxcdW5kZXJzZXR7XFxTaWdtYV4yfVxcb3BsYXhiaWNvbGltXFw7ICBGXFxkb20iXSxbMSwwLCJcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbVxcOyAgRlxcZG9tIl0sWzQsMiwiQyJdLFszLDAsIlxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbVxcOyAgRiJdLFsyLDIsIlxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbVxcOyAgRiJdLFszLDQsIlxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbVxcOyAgRiJdLFswLDEsIkZwXzBcXHBoaSJdLFswLDIsInFee1xcZG9tfV97cF8wXFxwaGl9IiwyXSxbMSwzLCJxXntcXGRvbX1fe3BfMVxccGhpfSJdLFszLDUsIlxcbGFuZ2xlIHFfe1xcY29kKGQpRihkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9Il0sWzUsNCwiXFxsYW5nbGUgcSdfaSBcXHJhbmdsZV97aSBcXGluIEl9Il0sWzYsNCwiXFxsYW5nbGUgcSdfaSBcXHJhbmdsZV97aSBcXGluIEl9IiwyXSxbMyw2LCJcXGxhbmdsZSBxX3tcXGRvbShkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9IiwxXSxbMSw2LCJxX3tcXGRvbVxcLCBwXzF9IiwxXSxbMiw2LCJcXGxhbmdsZSBxX3tcXGNvZChkKUYoZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMV0sWzIsNywiXFxsYW5nbGUgcV97XFxkb20oZCl9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSIsMl0sWzcsNCwiXFxsYW5nbGUgcSdfaSBcXHJhbmdsZV97aSBcXGluIEl9IiwyXSxbNSw2LCJcXGxhbmdsZSBcXHRoZXRhJ19kIHFfZCBcXHRoZXRhX2R7LTF9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiw3LCJcXGxhbmdsZSBcXHRoZXRhJ19kIHFfZCBcXHRoZXRhX2R7LTF9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTUsMywiXFx0aGV0YV97cF8xfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyLDE1LCJcXHRoZXRhJ197cF8wfSBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==


% https://q.uiver.app/?q=WzAsOCxbMCwyLCJGXFxkb21cXCwgcF8wIFxccGhpID0gRlxcZG9tIFxcLCBwXzIgXFxwaGkiXSxbMCwxLCJGXFxjb2RcXCxwXzBcXHBoaSA9IEYgXFxkb20gXFwsIHBfMVxccGhpIl0sWzQsMSwiXFx1bmRlcnNldHtJfVxcb3BsYXhiaWNvbGltXFw7ICBGIl0sWzIsMSwiRlxcY29kIFxcLCBwXzIgXFxwaGkgPSBGXFxjb2QgXFwsIHBfMSBcXHBoaSJdLFs1LDMsIkMiXSxbMiwwLCJcXHVuZGVyc2V0e1xcU2lnbWFeMn1cXG9wbGF4Ymljb2xpbVxcOyAgRlxcZG9tIl0sWzIsMywiXFx1bmRlcnNldHtcXFNpZ21hXjJ9XFxvcGxheGJpY29saW1cXDsgIEZcXGRvbSJdLFs0LDMsIlxcdW5kZXJzZXR7SX1cXG9wbGF4Ymljb2xpbVxcOyAgRiJdLFswLDEsIkZwXzBcXHBoaSJdLFsxLDMsIkZwXzFcXHBoaSIsMV0sWzMsMiwicV97XFxjb2QgXFwsIHBfMiBcXHBoaSB9PSBxX3tcXGNvZCBcXCwgcF8xIFxccGhpfSIsMCx7ImxhYmVsX3Bvc2l0aW9uIjo0MH1dLFsyLDQsIlxcbGFuZ2xlIHEnX2kgXFxyYW5nbGVfe2kgXFxpbiBJfSIsMCx7ImN1cnZlIjotMX1dLFsxLDUsInFee1xcZG9tfV97cF8xXFxwaGl9IiwwLHsiY3VydmUiOi0yfV0sWzUsMiwiXFxsYW5nbGUgcV97XFxjb2QoZClGKGQpfSBcXHJhbmdsZV97ZCBcXGluIFxcU2lnbWFeMn0iLDAseyJvZmZzZXQiOi0xLCJjdXJ2ZSI6LTF9XSxbMCw2LCJxXlxcZG9tX3twXzBcXHBoaX0iLDEseyJjdXJ2ZSI6Mn1dLFs2LDIsIlxcbGFuZ2xlIHFfe1xcY29kKGQpRihkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9IiwxXSxbMyw1LCJcXHRoZXRhJ197cF8xXFxwaGl9IFxcYXRvcCBcXHNpbWVxIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzcsNCwiXFxsYW5nbGUgcSdfaSBcXHJhbmdsZV97aSBcXGluIEl9IiwyXSxbNiw3LCJcXGxhbmdsZSBxX3tcXGRvbShkKX0gXFxyYW5nbGVfe2QgXFxpbiBcXFNpZ21hXjJ9IiwyXSxbMiw3LCJcXGxhbmdsZSBcXHRoZXRhJ19kIHFfZCBcXHRoZXRhX2R7LTF9IFxccmFuZ2xlX3tkIFxcaW4gXFxTaWdtYV4yfSBcXGF0b3AgXFxzaW1lcSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxNCwzLCJcXHRoZXRhX3twXzBcXHBoaX0gXFxhdG9wIFxcc2ltZXEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}
	&& {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} \\
	{F\cod\,p_0\phi = F \dom \, p_1\phi} && {F\cod \, p_2 \phi = F\cod \, p_1 \phi} && {\underset{I}\oplaxbicolim\;  F} \\
	{F\dom\, p_0 \phi = F\dom \, p_2 \phi} \\
	&& {\underset{\Sigma^2}\oplaxbicolim\;  F\dom} && {\underset{I}\oplaxbicolim\;  F} & C
	\arrow["{Fp_0\phi}", from=3-1, to=2-1]
	\arrow["{Fp_1\phi}"{description}, from=2-1, to=2-3]
	\arrow["{q_{\cod \, p_2 \phi }= q_{\cod \, p_1 \phi}}"{pos=0.4}, from=2-3, to=2-5]
	\arrow["{\langle q'_i \rangle_{i \in I}}", curve={height=-6pt}, from=2-5, to=4-6]
	\arrow["{q^{\dom}_{p_1\phi}}", curve={height=-12pt}, from=2-1, to=1-3]
	\arrow["{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}", shift left=1, curve={height=-6pt}, from=1-3, to=2-5]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{q^\dom_{p_0\phi}}"{description}, curve={height=12pt}, from=3-1, to=4-3]
	\arrow["{\langle q_{\cod(d)F(d)} \rangle_{d \in \Sigma^2}}"{description}, from=4-3, to=2-5]
	\arrow["{\theta'_{p_1\phi} \atop \simeq}"{description}, draw=none, from=2-3, to=1-3]
	\arrow["{\langle q'_i \rangle_{i \in I}}"', from=4-5, to=4-6]
	\arrow["{\langle q_{\dom(d)} \rangle_{d \in \Sigma^2}}"', from=4-3, to=4-5]
	\arrow["{\langle \theta'_d q_d \theta_d{-1} \rangle_{d \in \Sigma^2} \atop \simeq}"{description}, draw=none, from=2-5, to=4-5]
	\arrow["{\theta_{p_0\phi} \atop \simeq}"{description}, Rightarrow, draw=none, from=0, to=2-3]
\end{tikzcd}\]





